Trackable Island-model Genetic Algorithms at Wafer Scale

Emerging ML/AI hardware accelerators, like the 850,000 processor Cerebras Wafer-Scale Engine (WSE), hold great promise to scale up the capabilities of evolutionary computation. However, challenges remain in maintaining visibility into underlying evolutionary processes while efficiently utilizing these platforms' large processor counts. Here, we focus on the problem of extracting phylogenetic information from digital evolution on the WSE platform. We present a tracking-enabled asynchronous island-based genetic algorithm (GA) framework for WSE hardware. Emulated and on-hardware GA benchmarks with a simple tracking-enabled agent model clock upwards of 1 million generations a minute for population sizes reaching 16 million. This pace enables quadrillions of evaluations a day. We validate phylogenetic reconstructions from these trials and demonstrate their suitability for inference of underlying evolutionary conditions. In particular, we demonstrate extraction of clear phylometric signals that differentiate wafer-scale runs with adaptive dynamics enabled versus disabled. Together, these benchmark and validation trials reflect strong potential for highly scalable evolutionary computation that is both efficient and observable. Kernel code implementing the island-model GA supports drop-in customization to support any fixed-length genome content and fitness criteria, allowing it to be leveraged to advance research interests across the community.

==> Dockerfile <==
FROM mmore500/docker-texlive-full:sha-ea45eb5

COPY . /opt/wse-sketches/tex

SHELL ["/bin/bash", "-c"]

# Define default working directory.
WORKDIR /opt/wse-sketches/tex

# Prevent interactive time zone config.
# adapted from https://askubuntu.com/a/1013396
ENV DEBIAN_FRONTEND=noninteractive

RUN \
  echo 'Acquire::http::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::ftp::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::Retries "100";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo "buffed apt-get resiliency"

RUN \
  find /etc/apt -type f -name '*.list' -exec sed -i 's/\(^deb.*-backports.*\)/#\1/; s/\(^deb.*-updates.*\)/#\1/; s/\(^deb.*-proposed.*\)/#\1/; s/\(^deb.*-security.*\)/#\1/' {} + \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "removed -backports, -updates, -proposed, -security repositories"

# magic to fix java installation conflict in subsequent apt install
# see https://github.com/geerlingguy/ansible-role-java/issues/64
RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    man \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  mkdir /usr/share/man/man1/

RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    bibtool \
    git \
    make \
    moreutils \
    nodejs \
    pcregrep \
    pdftk \
    && \
  rm -rf /var/lib/apt/lists/*

CMD ["bash"]


==> Makefile <==
SHELL=/bin/bash

# get the basename of the containing directory
# this will be used to name othe output document
BUILD_DIR := $(shell basename $(abspath $(dir $(lastword $(MAKEFILE_LIST)))/..))

DRAFT_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}-draft.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

RELEASE_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

all: ${BUILD_DIR}-draft.pdf

draft: ${BUILD_DIR}-draft.pdf ${BUILD_DIR}-manuscript-draft.pdf ${BUILD_DIR}-supplement-draft.pdf ${BUILD_DIR}-draft.tex

release: ${BUILD_DIR}.pdf ${BUILD_DIR}-manuscript.pdf ${BUILD_DIR}-supplement.pdf ${BUILD_DIR}.tex

${BUILD_DIR}.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR} \
    -pdflatex="pdflatex -interaction=nonstopmode" main.tex

${BUILD_DIR}.tex: main.tex
	./script/latexpand.pl main.tex > ${BUILD_DIR}.tex

${BUILD_DIR}-manuscript.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat 1-$$(( $(RELEASE_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript.pdf

${BUILD_DIR}-supplement.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat $(RELEASE_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement.pdf

${BUILD_DIR}-draft.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR}-draft \
    -pdflatex="pdflatex -interaction=nonstopmode" draft.tex

${BUILD_DIR}-draft.tex: main.tex
	./script/latexpand.pl draft.tex > ${BUILD_DIR}-draft.tex

${BUILD_DIR}-manuscript-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat 1-$$(( $(DRAFT_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript-draft.pdf

${BUILD_DIR}-supplement-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat $(DRAFT_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement-draft.pdf

fresh: cleaner all

clean:
	rm -f ${BUILD_DIR}.pdf
	rm -f ${BUILD_DIR}.tex
	rm -f ${BUILD_DIR}-draft.pdf
	rm -f ${BUILD_DIR}-draft.tex
	rm -f ${BUILD_DIR}-manuscript.pdf
	rm -f ${BUILD_DIR}-manuscript-draft.pdf
	rm -f ${BUILD_DIR}-supplement.pdf
	rm -f ${BUILD_DIR}-supplement-draft.pdf

sview:
	xdg-open ${BUILD_DIR}-draft.pdf 2>/dev/null

cleaner: clean
	latexmk -CA
	# remove auxillary files, excepting .tex and .bib files
	find . -type f -name ${BUILD_DIR}"*" ! -name '*.tex' ! -name '*.bib' -delete
	rm -rf *.bbl *.blg *.aux

.PHONY: draft release clean sview cleaner fresh


==> binder-wafer-scale/tex/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> binder-wafer-scale/tex/fig/async-ga-schematic.tex <==
\begin{figure}
  \centering
\includegraphics[width=0.8\linewidth]{binder-wse-sketches/tex-access-proposal/img/async-ga-schematic}
  \caption{%
  \textbf{Island model GA implementation for WSE.}
  Neighboring PEs exchange agent genomes (``migration''') via asynchronous send/receive operations from dedicated buffers, with on-completion callbacks seting ``ready'' flags.
  }
  \label{fig:async-ga-schematic}
  \vspace{-0.2in}
\end{figure}


==> binder-wafer-scale/tex/fig/benchmarking.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{binder-wafer-scale/binder/teeplots/all=false+hue=implementation+orient=h+row=language+score=nanoseconds-per-op+viz=peckplot+x=nanoseconds-per-op+y=policy+y-group=outer+ext=}

\vspace{-2.5ex}

  \caption{%
    \textbf{Hereditary stratigraphy algorithm benchmarks.}
    \footnotesize
    Comparison of per-generation operation time for column- and surface-based steady and tilted retention policies, lower is better.
  Top and bottom panels show Python and Zig implementations, respectively.
    Trivial is a simple harcoded retention decision, provided as a baseline control.
    Background hatching indicates significant outcome (Mann-Whitney U test; $n=20$).
  }
  \label{fig:benchmarking}
  \vspace{-0.2in}
\end{figure*}


==> binder-wafer-scale/tex/fig/col-vs-surf.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{binder-reconstruction-quality/binder/surf-vs-col/outplots/surf-vs-col-table}
  \caption{%
   \textbf{Comparison of reconstruction accuracies from column- and surface-based annotations.}
   \footnotesize
    Color coding represents non-parametric difference between accuracy measures, with red indicating superior surface performance and blue indicating superior column performance.
    Left column shows tilted retention policies, and right column shows steady retention policies.
    For heatmap charts, +'s indicate small, medium, and large effect sizes using the Cliff's delta statistic and *'s indicate statistical significance at $\alpha = 0.05$ via Mann-Whitney U test.
  }
  \label{fig:col-vs-surf}
  \vspace{-0.2in}
\end{figure*}


==> binder-wafer-scale/tex/fig/genome-layout.tex <==
% Define lighter colors
\definecolor{LighterBlue}{rgb}{0.84, 0.92, 0.95}
\definecolor{LighterSalmon}{rgb}{1.0, 0.81, 0.76}
\definecolor{LighterPastelGreenYellow}{rgb}{0.88, 0.96, 0.90}

% Define thick vertical lines for section dividers
\newcolumntype{q}{!{\color{white} \vrule width 2pt}}

\begin{figure*}
    \centering
\begin{minipage}[t]{\textwidth}
\centering
\footnotesize
\begin{tabular}{
c
>{\columncolor{LighterBlue}}c
>{\columncolor{LighterBlue}}c
>{\columncolor{LighterSalmon}}c
>{\columncolor{LighterSalmon}}c
q % Thick divider
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
q % Thick divider
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
}
& \multicolumn{4}{cq}{\cellcolor{white}Word 0} & \multicolumn{4}{cq}{\cellcolor{white}Word 1} & \multicolumn{4}{c}{\cellcolor{white}Word 2} \\
\cmidrule(l{1.5pt}r{1.5pt}){2-5}
\cmidrule(l{1.5pt}r{1.5pt}){6-9}
\cmidrule(l{1.5pt}r{1.5pt}){10-13}
Byte & {\cellcolor{white}0} & {\cellcolor{white}1} & {\cellcolor{white}2} & {\cellcolor{white}3} & {\cellcolor{white}4} & {\cellcolor{white}5} & {\cellcolor{white}6} & {\cellcolor{white}7} & {\cellcolor{white}8} & {\cellcolor{white}9} & {\cellcolor{white}10} & {\cellcolor{white}11} \\
\cmidrule(l{1.5pt}r{1.5pt}){2-2}
\cmidrule(l{1.5pt}r{1.5pt}){3-3}
\cmidrule(l{1.5pt}r{1.5pt}){4-4}
\cmidrule(l{1.5pt}r{1.5pt}){5-5}
\cmidrule(l{1.5pt}r{1.5pt}){6-6}
\cmidrule(l{1.5pt}r{1.5pt}){7-7}
\cmidrule(l{1.5pt}r{1.5pt}){8-8}
\cmidrule(l{1.5pt}r{1.5pt}){9-9}
\cmidrule(l{1.5pt}r{1.5pt}){10-10}
\cmidrule(l{1.5pt}r{1.5pt}){11-11}
\cmidrule(l{1.5pt}r{1.5pt}){12-12}
\cmidrule(l{1.5pt}r{1.5pt}){13-13}
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 0} & \texttt{F9} & \texttt{02} & \texttt{79} & \texttt{00} & \texttt{8D} & \texttt{22} & \texttt{4F} & \texttt{F3} & \texttt{D2} & \texttt{78} & \texttt{AD} & \texttt{C7} \\
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 1} & \texttt{F9} & \texttt{02} & \texttt{75} & \texttt{00} & \texttt{8D} & \texttt{A1} & \texttt{CB} & \texttt{F2} & \texttt{D1} & \texttt{5B} & \texttt{CC} & \texttt{D4} \\
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 2} & \texttt{61} & \texttt{B6} & \texttt{65} & \texttt{00} & \texttt{66} & \texttt{29} & \texttt{B4} & \texttt{F0} & \texttt{62} & \texttt{99} & \texttt{5A} & \texttt{61} \\
{\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} &
{\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} \\
\end{tabular}
\end{minipage}

\begin{minipage}[t]{\textwidth}
\caption{%
\textbf{Example genomes sampled after validation experiment completion.}
  In validation testing, genomes were composed of three 32-bit words.
  The first two bytes (blue) are fixed random markers generated at simulation start-up, indicating independent lineage originations.
  The next two bytes (salmon) are a generation counter.
  Bits within the final eight bytes are lineage checkpoint values to facilitate phylogenetic reconstruction, arranged according to a tilted hereditary stratigraphic algorithm.
  Note that this genome does not include any content affecting agent traits or fitness --- neutral selection was used for this validation experiment.
}
\label{fig:genome-layout}
\end{minipage}
\end{figure*}


==> binder-wafer-scale/tex/fig/on-device.tex <==
\begin{figure}

\begin{subfigure}[c]{\linewidth}
    \includegraphics[width=\linewidth]{binder-wse-sketches/binder/teeplots/col=metric+hue=regime+kind=swarm+post=teed-set-titles-col-name+viz=catplot+x=num-pes-10k+y=value+ext=}
 \caption{\footnotesize adaptive vs. purifying phylometric structure}
  \label{fig:on-device-phylometrics}
\end{subfigure}

\vspace{0.2ex}

\begin{subfigure}[c]{0.5\linewidth}
  \centering
  \includegraphics[width=0.7\linewidth,trim={0 11.05in 7.2in 0in},clip]{binder-wse-sketches/binder/outplots/linear/genomeFlavor=genome_purifyingplus+globalSeed=1.0+nCycle=1000000.0+popSize=562500+replicate=0d82d64b-991d-455b-84d8-cdf9edaad99d+ext=}

  \vspace{-2ex}
  \includegraphics[width=0.7\linewidth,trim={0 11.05in 7.2in 0in},clip]{binder-wse-sketches/binder/outplots/log/genomeFlavor=genome_purifyingplus+globalSeed=1.0+nCycle=1000000.0+popSize=562500+replicate=0d82d64b-991d-455b-84d8-cdf9edaad99d+ext=}

  \vspace{-2ex}
  \footnotesize
 \caption{\footnotesize adaptive regime}
  \label{fig:on-device-adaptive}
\end{subfigure}%
\begin{subfigure}[c]{0.5\linewidth}
  \centering
  \includegraphics[width=0.7\linewidth,trim={0 11.05in 7.2in 0in},clip]{binder-wse-sketches/binder/outplots/linear/genomeFlavor=genome_purifyingonly+globalSeed=1.0+nCycle=1000000.0+popSize=562500+replicate=ce2a0bf2-e132-4a61-95ec-c6ca54213949+ext=}

  \vspace{-2ex}
  \includegraphics[width=0.7\linewidth,trim={0 11.05in 7.2in 0in},clip]{binder-wse-sketches/binder/outplots/log/genomeFlavor=genome_purifyingonly+globalSeed=1.0+nCycle=1000000.0+popSize=562500+replicate=ce2a0bf2-e132-4a61-95ec-c6ca54213949+ext=}

  \vspace{-2ex}
  \footnotesize
 \caption{\footnotesize purifying regime}
  \label{fig:on-device-purifying}
\end{subfigure}

\vspace{-1.5ex}

\caption{%
\textbf{On-hardware Trial.}
\footnotesize
Results from phylogenetic reconstruction of 1 million generation simulations with 10k ($100\times100$), 250k ($500\times500$) and 562.5k ($750\times750$) PE arrays.
Panel \ref{fig:on-device-phylometrics} compares phylometric readings from purifying-only and adaptation-enabled configurations, 4 replicates each.
Panels \labelcref{fig:on-device-adaptive,fig:on-device-purifying} juxtapose example $750\times750$ PE simulation phylogenies under each configuration regime.
Example phylogenies reconstructed from runs of increasing duration on grid of nine hardware-simulated PEs.
Phylometrics were calculated from reconstructions with 10k sampled end-state agents.
For legibility, phylogeny visualizations were further subsampled to 1k end-state agents.
Top phylogenies are linear-scaled.
Bottom phylogenies are log-scaled with ultrametric correction to better show topology.
}
\label{fig:on-device}
\vspace{-0.2in}
\end{figure}


==> binder-wafer-scale/tex/fig/schematic.tex <==
\begin{figure}
  \vspace{2ex}
    \centering
  \includegraphics[width=0.8\linewidth]{binder-wse-sketches/tex-access-proposal/img/runtime-posthoc-schematic}
  \vspace{-1.5ex}
    \caption{\textbf{Strategy for trackable distributed evolution simulation.}
    \footnotesize %
    Hstrat markers attached to agent support post hoc estimation of relatedness between lineages, enabling approximate phylogenetic reconstruction.
    }
    \label{fig:runtime-posthoc-schematic}
\vspace{-0.2in}
\end{figure}


==> binder-wafer-scale/tex/fig/surf-algorithms.tex <==
\begin{figure*}
  \centering
\begin{subfigure}[b]{0.43\linewidth}
\centering
\textbf{steady retention policy}
\end{subfigure}
\begin{subfigure}[b]{0.43\linewidth}
\centering
\textbf{tilted retention policy}
\end{subfigure}

\vspace{-1.5ex}

  \begin{subfigure}[b]{0.5\linewidth}
    \centering
  \includegraphics[width=0.88\linewidth,trim={0 0 2.4cm 0},clip]{binder-surface-concept/teeplots/10/cnorm=log+num-generations=4096+surface-size=256+viz=site-deposition-depth-by-rank-heatmap+ynorm=linear+ext=}

    % \vspace{-1.5ex}

    % \caption{\footnotesize 256 bit steady surface site age plot}
    % \label{fig:steady-age-plot}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
  \includegraphics[width=0.88\linewidth, trim={2.4cm 0 0 0},clip]{binder-surface-concept/teeplots/21/cnorm=log+num-generations=4096+surface-size=256+viz=site-deposition-depth-by-rank-heatmap+ynorm=linear+ext=}

  % \vspace{-1.5ex}

  %   \caption{\footnotesize 256 bit tilted surface site age plot}
    % \label{fig:tilted-age-plot}
  \end{subfigure}

\vspace{-1ex}

\begin{subfigure}[b]{0.5\linewidth}
  \flushleft
\includegraphics[height=0.85in, trim={0 0 0 0},clip]{binder-surface-concept/teeplots/10/num-generations=262144+surface-size=64+viz=stratum-persistence-dripplot+ext=}

  % \centering
  % \vspace{-1.5ex}

  % \caption{\footnotesize 64 bit steady surface time retention plot}
  \label{fig:steady-retention-plot}
\end{subfigure}%
\begin{subfigure}[b]{0.5\linewidth}
  \centering
\includegraphics[height=0.85in, trim={1.65cm 0 0 0},clip]{binder-surface-concept/teeplots/21/num-generations=262144+surface-size=64+viz=stratum-persistence-dripplot+ext=}

  % \centering
  % \vspace{-1.5ex}

  % \caption{\footnotesize 64 bit tilted surface time retention plot}
  % \label{fig:tilted-retention-plot}
\end{subfigure}

\vspace{-2.5ex}

\caption{%
  \textbf{Surface-based hereditary stratigraphy implementations.}
  \footnotesize
  Visualizations of steady (left) and tilted (right) surface site selection policies.
  Top row heatmaps shows evolution of time-since-last-deposition for each site on a 256 bit field over the course of 4,096 depositions.
  Bottom row shows retention spans for 3,000 ingested time points.
  Vertical lines span durations between ingestion and elimination for differentia appended at successive time points.
  Time points previously eliminated are marked in red.
  Time elapses from bottom to top in both visualizations.
  }
\label{fig:surf-algorithms}
\vspace{-0.2in}

\end{figure*}


==> binder-wafer-scale/tex/fig/surf-vs-column-schematic.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{img/surf-vs-column-schematic}

  \vspace{-1.5ex}

  \caption{
  \textbf{Column vs. surface-based hereditary stratigraphy.}
  \footnotesize
  Contrast of existing sorted-order ``column''-based stratum retention framework with proposed explicitly addressed ``surface''-based approach.}
  \label{fig:surf-vs-column-schematic}
  \vspace{-0.2in}
\end{figure}


==> binder-wafer-scale/tex/fig/tagged.tex <==
\begin{figure}

\begin{subfigure}[c]{\linewidth} \centering
\begin{minipage}[c]{0.08\linewidth} \flushright
    \caption{\rotatebox[origin=c]{90}{25 cycles}}
    \label{fig:tagged_25}
  \end{minipage}%
  \begin{minipage}[c]{0.92\linewidth}
    \includegraphics[width=\textwidth,height=0.6in,trim={0 0.81cm 0 0},clip]{binder-wse-sketches/binder/teeplots/genome=hsurftiltedsticky_tagged+replicate=e4ea2071-8228-42de-af8c-879cedff9ba7+viz=draw-biopython-tree+ext=}
  \end{minipage}%
\end{subfigure}

\vspace{-1ex}

\begin{subfigure}[c]{\linewidth} \centering
\begin{minipage}[c]{0.08\linewidth} \flushright
    \caption{\rotatebox[origin=c]{90}{50 cycles}}
    \label{fig:tagged_50}
  \end{minipage}%
  \begin{minipage}[c]{0.92\linewidth}
    \includegraphics[width=\textwidth,height=0.6in,trim={0 0.81cm 0 0},clip]{binder-wse-sketches/binder/teeplots/genome=hsurftiltedsticky_tagged+replicate=3d55af5f-7714-45da-9276-e860f46b4d94+viz=draw-biopython-tree+ext=}
  \end{minipage}%
\end{subfigure}

\vspace{-1ex}

\begin{subfigure}[c]{\linewidth} \centering
  \begin{minipage}[c]{0.08\linewidth} \flushright
    \caption{\rotatebox[origin=c]{90}{100 cycles}}
    \label{fig:tagged_100}
  \end{minipage}%
  \begin{minipage}[c]{0.92\linewidth}
    \includegraphics[width=\textwidth,height=0.6in,trim={0 0.81cm 0 0},clip]{binder-wse-sketches/binder/teeplots/genome=hsurftiltedsticky_tagged+replicate=932aa302-becb-47e8-9712-7f550b02364c+viz=draw-biopython-tree+ext=}
  \end{minipage}%
\end{subfigure}

\vspace{-1ex}

\begin{subfigure}[c]{\linewidth} \centering
  \begin{minipage}[c]{0.08\linewidth} \flushright
    \caption{\rotatebox[origin=c]{90}{250 cycles}}
    \label{fig:tagged_250}
  \end{minipage}%
  \begin{minipage}[c]{0.92\linewidth}
    \includegraphics[width=\textwidth,height=0.8in]{binder-wse-sketches/binder/teeplots/genome=hsurftiltedsticky_tagged+replicate=42dbcbb3-b803-41a4-9285-4a450bfad6ed+viz=draw-biopython-tree+ext=}
  \end{minipage}%
\end{subfigure}

\vspace{-1.5ex}

\caption{%
\textbf{Clade Reconstruction Trial.}
\footnotesize
Example phylogenies reconstructed from runs of increasing duration on virtual grid of nine hardware-simulated PEs.
Founding genomes were tagged with random 16-byte identifier values, which were held constant over the course of simulation (Supplementary Figure \ref{fig:genome-layout}).
Color-coding indicates each sampled taxon's founding ancestor according to this identifier value.
Simulation performed under drift conditions.
}
\label{fig:tagged}
\vspace{-0.2in}
\end{figure}


==> binder-wafer-scale/tex/fig/wse-phylogenies.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{\textwidth}
    \centering
    Generations Ago (approx.)
  \end{minipage}
  \begin{minipage}{\textwidth}
    \hspace{0.02\linewidth}
    \rotatebox{30}{\makebox[0.1\linewidth][c]{200,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{50,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{10,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{2,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{30}}
    \rotatebox{90}{\makebox[0.04\linewidth][c]{0}}
  \end{minipage}
  \begin{subfigure}[t]{\linewidth}
    \centering
  \includegraphics[width=\linewidth,height=0.3\linewidth]{bindertex-evolutionary-inference/img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=22/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=22+_generation=262144+_index=22+scale=log+ext=}
    \caption{%
    Tournament size 2.
    STAND-IN IMAGE.
    }
    \label{fig:wse-phylogenies-tsize2}
  \end{subfigure}

  \begin{subfigure}[t]{\linewidth}
    \centering
\includegraphics[width=\linewidth,height=0.3\linewidth]{bindertex-evolutionary-inference/img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=6/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=6+_generation=262144+_index=6+scale=log+ext=}
    \caption{%
      Tournament size 8.
      STAND-IN IMAGE.
    }
    \label{fig:wse-phylogenies-tsize8}
  \end{subfigure}

\caption{%
\textbf{Phylogenies from on-hardware experiment.}
\footnotesize
Subfigures \ref{fig:wse-phylogenies-tsize2} and \ref{fig:wse-phylogenies-tsize8} contrast phylogenies from experiments with lower and higher selection pressure, respectively.
Note the recognizable decrease in phylogenetic richness under high selection pressure.
Each phylogeny subsampled to 131,072 taxa.
}
\label{fig:wse-phylogenies}

\end{figure*}


==> binder-wafer-scale/tex/text/acknowledgement.tex <==
\section*{Acknowledgement}
{\footnotesize
This research was supported by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research, through hardware access and training provided by the ByteBoost program under the National Science Foundation Cybertraining awards 2320990/2320991/2320992, and is based upon work supported by the Eric and Wendy Schmidt AI in Science Postdoctoral Fellowship, a Schmidt Futures program.
This research was supported in part by funding from the NSF (DEB 1813069).
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.
Thank you also to Mathias Jacquelin, Udai Mody, and Leighton Wilson at Cerebras Systems for guidance on technical aspects of this project.
}


==> binder-wafer-scale/tex/text/body.tex <==
\input{text/body/abstract.tex}

\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> binder-wafer-scale/tex/text/body/abstract.tex <==
\begin{abstract}
\vspace{-2ex}
Continuing improvements in computing hardware are poised to transform capabilities for \textit{in silico} modeling of cross-scale phenomena underlying major open questions in evolutionary biology and artificial life, such as transitions in individuality, eco-evolutionary dynamics, and rare evolutionary events.
Emerging ML/AI-oriented hardware accelerators, like the 850,000 processor Cerebras Wafer Scale Engine (WSE), hold particular promise.
However, many practical challenges remain in conducting informative evolution experiments that efficiently utilize these platforms' large processor counts.
Here, we focus on the problem of extracting phylogenetic information from agent-based evolution on the WSE platform.
This goal drove significant refinements to decentralized \textit{in silico} phylogenetic tracking, reported here.
These improvements yield order-of-magnitude performance improvements.
We also present an asynchronous island-based genetic algorithm (GA) framework for WSE hardware.
Emulated and on-hardware GA benchmarks with a simple tracking-enabled agent model clock upwards of 1 million generations a minute for population sizes reaching 16 million agents.
This pace enables quadrillions of agent replication events a day.
We validate phylogenetic reconstructions from these trials and demonstrate their suitability for inference of underlying evolutionary conditions.
In particular, we demonstrate extraction, from wafer-scale simulation, of clear phylometric signals that differentiate runs with adaptive dynamics enabled versus disabled.
Together, these benchmark and validation trials reflect strong potential for highly scalable agent-based evolution simulation that is both efficient and observable.
Developed capabilities will bring entirely new classes of previously intractable research questions within reach, benefiting further explorations within the evolutionary biology and artificial life communities across a variety of emerging high-performance computing platforms.
\end{abstract}


==> binder-wafer-scale/tex/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

Computing hardware with transformative capabilities is coming to market right now.
% and some of it --- like the Cerebras wafer scale engine \citep{lauterbach2021path} --- is built explicitly for decentralized, asynchronous computation.
This fact presents an immediate opportunity to bring orders-of-magnitude greater simulation scale to bear on grand challenges in artificial life.
It is not unreasonable to anticipate possibility that with such resources some aspects of these open questions will be revealed to harbor more-is-different dispositions, in which larger scales demonstrate qualitativey different dynamics \citep{anderson1972more}.
Riding the coattails of AI-workload driven hardware development, itself largely driven by profound more-is-different payoffs in deep learning, provides perhaps the most immediate means toward this possibility.

Such an endeavor is a community-level challenge that will require extensive collaborative effort and pursuit of outside resources.
 % a community-scale challenge that will require and pursuing collaborations and resources beyond the present comfort zone.
% And
% But just like other science domains have united to acquire resources for paradigm-changing resources we need to do the same thing.
Work presented here is an early step in methods and wide-ranging infrastructure development necessary to scale up what's possible in digital evolution research.
We have demonstrated new algorithms and software for phylogeny-enabled agent-based evolution on a next-generation HPC accelerator hardware platform.
With respect to instrumentative simulation components, microbenchmarking results show that proposed algorithms achieve several-fold improvement in computational efficiency.
Related work has found that the new algorithms can improve reconstruction quality in some cases, too \citep{moreno2024guide}.
Early emulated integrative benchmarking suggests that, for simple agent models, on the order of quintillions of replication cycles per day may be possible at full wafer scale on CS-2 hardware.

% However, in the wide-ranging .
% that will be necessary to achieve rich simulation at scales with potential to reveal
Special characteristics set agent-based digital evolution apart from many other HPC application domains and position it as a potentially valuable testbed for innovation and leadership.
Among these factors are challenging workload heterogeneity (varying within a population and over evolutionary time), resiliency of global state to local perturbations, and perhaps unparalleled freedom to recompose underlying simulation semantics to accommodate hardware capabilities.
Indeed, artificial life and digital evolution have played host to notable boundary-pushing approaches to computing at the frontiers of computing modalities such as best-effort computing, reservoir computing, globe-spanning time-available computing, and modular tile-based computing in addition to more traditional cluster and GPU-oriented approaches \citep{moreno2021conduit,ackley2020best,ackley2023robust,heinemann2008artificial,miikkulainen2024evolving}.
Work done to scale up digital evolution simulation should be done with an eye for contributions back to broader HPC constituencies.
% As noted earlier, the unique character of artificial life simulation suits it to serve at the tip of the spear in HPC evolution.
% Effort to establish artificial life simulation as a flagship HPC application could be of mutual benefit.

% There is reason to expect a highly synergistic, reciprocal relationship between digital evolution and the broader HPC enterprise.
% Work proposed here steps in this direction, seeking to blaze new territory that opens new possibilities to benefit broader constituencies of ABM/HPC practitioners.
% exciting --- and fairly uncharted, with applications outside deep learning workloads still in early days
% Researchers using agent-based evolution recognize HPC as critical to the future of the field \citep{ackley2016indefinite}.

% due to emerging architectures being built to support deep learning, if only we can developm methods necessary to operate within their framings.
% It is easy to do experiments on your laptop or on traditional HPC resources you can access without having to ask for money.
% Given ubiquity of deep net training and stencil-based numerical solvers in applications (CITE), programming for agent-based simulation can be of interest insofar as it flexes harware capabilities in unimagined ways.

In this vein, presented ``surface'' indexing algorithms stand to benefit larger classes of stream curation problems, situations in which a rolling feed of sequenced observations must be dynamically downsampled to ensure retention of elements representative across observed history \citep{moreno2024algorithms}.
% Potential extensions of this work include repurposing of HStrat's rolling cross-temporal sampling algorithms to facilitate efficient downsampled observability in additional application domains.
In particular, to further benefit observable agent-based modeling, we are interested in exploring applications that sample time-series activity at simulation sites or distill coarsened agent histories (e.g., position over time).

The immediate goal of our presented work, however, is to build means for progress toward existing research agendas held across the realms of digital evolution and artificial life.
To this end, our work has prioritized production of reusable CSL and Python software tools ready to be harnessed by the broader research community.
In particular, CSL code implementing the presented island-model GA is defined in a modularized and extensible manner to support drop-in customization to instantiate any fixed-length genome content and fitness criteria corresponding to research interests within the community.
We look forward to collaboration in broader, tandem efforts to harness the Cerebras platform, and other emerging hardware, in follow-on work.

% These new HStrat methods, and extensive development targeting the Cerebras CSL using the SDK hardware simulator, position our project
% to hit the ground running.


% Within ABM, our proposed work focuses in particular on the topic of evolutionary computation.
% Our project design emphasizes explicit steps to demonstrate and evaluate novel components of underlying implementation in order to form technical foundations for ongoing work in this vein.



% The diversity of HPC strategies for evolutionary simulation stems in large part from unique properties largely distinct from other HPC application domains.
% Given its inherent underlying stochastic nature and the stabilizing influence of adaptive selection, evolutionary simulation can often tolerate significant arbitrary asynchronicity or even entirely lost simulation components (e.g., dropped messages, crashed nodes, etc.).
% Likewise, digital evolution is typically amenable to locality restrictions of computation due to the inherent spatial structure of natural systems we are seeking to model.
% % In particular, massively-distributed, spatial computing being directly highlighted to be of particular interest \citep{ackley}.
% Because agent behavior evolves over time, the influence of population-level drift and adaptive change can inject extreme heterogeneity into the computational workload profile of evolutionary simulation over time and simulation space.
% Finally, emerging research questions have introduced challenging communication-intensive requirements to support rich interactions between evolving agents.
% The largely decoupled nature of classic approaches within evolutionary computation like island models or controller/worker schemes  \citep{bennett1999building,cantu2001master} no longer suffice to realize the dynamic, communication-intensive interaction characteristic of major transitions in individuality (e.g., multicellularity) and ecological communities \citep{moreno2022engineering}.

% Proposed work lays foundations to harness wafer-scale computing for agent-based modeling.
% Orders-of-magnitude scale-up will bring entirely new classes of cross-scale dynamics within reach across many ABM application areas.
% To advance on this front, we explore a fundamental re-frame of simulation that shifts from a paradigm of complete, perfect data observability to dynamic, approximate observability akin to estimation approaches traditionally used to study physical systems.

% We will harness cutting-edge \textit{hereditary stratigraphy} (HStrat) approaches to distributed phylogenetic tracking to investigate fundamental questions about the relationship between phylogenetic structure, population scale, and time scale.

% Within the domain of evolution modeling, we anticipate building from work proposed here to conduct cross-scale evo-epidemiological research into how pathogen trait evolution confronts fitness trade-offs related to within-host infection dynamics and between-host transmissibility.


==> binder-wafer-scale/tex/text/body/introduction.tex <==
\section{Introduction}

\input{fig/schematic}

% defining? fundamental?
A quintessential characteristic of computational artificial life experiments is the near total malleability of the simulacrum \citep{pattee1989simulations}.
Indeed, ability to explore arbitrary possibilities as-they-could-be is the core of artificial life's role as a tool for inquiry \citep{langton1997artificial}.
Such near-limitless freedom to realize arbitrary system configurations, however, can obscure an intrinsic limitation of most computational artificial life work: scale.

% Often, although not always, computational alife systems are designed for evaluation on a single CPU.
Take, for instance, the Avida platform, which instantiates populations of self-replicating computer programs for evolution experiments.
When running on a single CPU, this system can support about 20,000 generations per day, or about two hundred million individual replication cycles daily \citep{ofria2009artificial}.
By way of comparison, \textit{E. coli} populations within individual flasks of the Lenski Long-Term Evolution Experiment undergo only six doublings per day, meaning their generations take orders of magnitude longer than Avidians \citep{good2017dynamics}.
(In continuous culture, though, the rate can be c. 72 generations per day.)
Indeed, such capability for fast generational turnover has been a key motivation for using artificial life systems to study evolution.
However, the effective population size of flasks in the Long-Term Evolution Experiment is orders of magnitude larger than Avida's: 30 million vs. 10,000.
Consequently, these systems actually exhibit a similar number of replication events per day.
%With an effective population size of 30 million and around 6 doublings per day, about 180 million replication events elapse per day within each flask \citep{good2017dynamics}.
This pattern of dramatically faster generation times than those observed in nature and dramatically smaller populations largely generalizes across artificial life systems.
%Although Alife systems can typically observe generational cycles at orders-of-magnitude faster rates than their biological counterparts, population sizes are often limited and,
Of course, any such comparisons should also note profound discrepancies between the genetic, phenotypic, and environmental richness of biological organisms and alife models.
% Of course, such a comparison neglects profound incommensurabilities between Avidians and bacteria or yeast.
% Natural organisms have vastly more genetic content and phenotypic state, as well as more and more diverse interactions with the environment and with other cells.

% Adversely? Crucially? Conversely? Formidabbly? Aversely? Cumbrously?
Crucially, however, the scale of population size can greatly impact subjects of artificial life research, like transitions in individuality, ecological dynamics, and rare evolutionary innovations \citep{taylor2016open,dolson2021digital,taylor2019evolutionary}.
% Indeed, there is some evidence that limitations in scale are holding back \citep{CITEGEB}.
Cross-scale dynamics are also crucial to many key real-world challenges.
For example, in evolutionary epidemiology, interactions between within-host infection dynamics and population-level epidemiological patterns determine the evolutionary trajectory of the population \citep{schreiber2021cross}.
However, because capabilities of current silicon-based processors are not expected to improve markedly in the forseeable future \citep{sutter2005free}, scale-up necessary to progress on these key frontiers will demand many-processor computation.
Application of parallel and distributed computation, however, imposes compromises with respect to the convienence, flexibility, observability, interpretability, total reliability, and perfect replicability enjoyed under classical centralized, serial models of computation.
Encouragingly, these challenges are already implicit to much of biology; the productivity of research involving natrual organisms evidences that they are surmountable and even hints at strategies that can be used to solve them.
Here, we explore alignment of digital evolution to HPC accelerator hardware at the extreme cutting-edge of massively distributed computation, and use techniques inspired by those applied to natural organisms to mitigate limitations of distributed computation with respect to tracking phylogenies.

\subsection{Progress toward Scale-up in Artificial Life}

% effort
Achieving highly-scalable artificial life and digital evolution systems involves two distinct engineering considerations.
First, as with any high-performance scientific computing, careful design is required to appropriately divvy computation and communication workloads across available hardware.
% flexible/pliable/creative/abstract/representational/invites
% formulation
Second, given the exceptionally discretionary nature of artificial life modeling, we can intentionally tailor simulation semantics to suit underlying hardware capabilities.
% dichotomy
Ackley's ongoing work with the T2 Tile Project and ULAM exemplifies a strong synthesis of this engineering duality \citep{ackley2016ulam}.
At the level of simulation semantics, Ackley formulates update procedures in terms of local interactions between discrete, spatially situated particles.
This design provides for an efficient one-to-one mapping between simulation space and hardware components, minimizing requirements for intra-hardware connectivity and preventing global impacts from on-the-fly augmentations or reductions of available hardware.
The ULAM framework then ties into implementation-level infrastructure necessary to accomplish performant, best-effort lock/release of spatial event windows spanning bordering hardwares \citep{ackley2013movable}.
The Santa Fe Board project provided analogous infrastructure foundations for earlier work, coordinating efficient packet-framed, non-blocking communication between hardware tile elements \citep{livingcomputationSFBSanta}.
Ackley's work is distinguished, in fact, in dipping to a yet-lower level of abstraction and tackling design of bespoke, modular distributed processing hardware \citep{ackley2011homeostatic,ackley2023robust}.
% to engineer computational artificial life systems for scalability
% This work joins/builds on a longstanding chorus of interest in scale-up of artificial life, and already some exciting work in that domain.
% Of particular note is ADVOCACY/ARGUMENTATION Ackley has bespoke hardware \citep{ILLUMINAXMACHINA,ackley2023robust}.

% parallel and distributed
Several additional digital evolution projects have made notable headway in synthesizing artificial life models with sophisticated, scalable technical backing, achieving rich interactions among numerous parallelized simulation components.
Harding demonstrated large-scale cellular automota-based artificial development systems, achieved through GPU-parallelized instantiations of a genetic program  \citep{harding2007fast_ieee}.
Early work by Ray with Network Tierra used an island model to distribute digital organisms across federated servers, with migration handled according to the real-time latencies and topology of the underlying network \citep{ray1995proposal}.
More recently, Heinemann's continuation of the ALIEN project has leveraged GPU acceleration to achieve spectacularly elaborate simulations with rich interactions between numerous spatially-situated soft body agents \citep{heinemann2008artificial}.
Likewise, the Distributed Hierarchical Transitions in Individuality (DISHTINY) project has incorporated event-driven agent-agent interaction schemes amenable to best-effort, asynchronous interlocution \citep{moreno2022exploring,moreno2021conduit}.
GPU-first agent-based modeling (ABM) packages like Flame GPU also tackle this problem of hardware-simulacrum matching, albeit framed at a higher level of abstraction \citep{richmond2010high}.
Beyond alife, broader realms of application-oriented evolutionary computation have folded in with many-processor computation, most commonly through island-model and director-worker evaluation paradigms \citep{abdelhafez2019performance,cantu2001master}.

\subsection{Untapped Emerging Hardware}

In retrospect, connectionist artificial intelligence turns out to have been profoundly scale-dependent.
The utility and ubiquity of ANNs have exploded in tandem with torrential growth in training set sizes, parameter counts, and training FLOPs \citep{marcus2018deep}.
Recruitment of multi-GPU training for image classification, requisite particular accomodating adjustments to the underlying deep learning architecture, is commonly identified as the watershed moment to this transformation
 \citep{krizhevsky2012imagenet}.
Commerical investment in AI capabilies then set in motion a virtuous cycle of further-and-further-enabling hardware advances \citep{jouppi2017datacenter}.
Indeed, the scaling relationship between deep learning and training resources has itself become a major area of active study, with expectation for this virtuous cycle to continue through the forseeable future \citep{kaplan2020scaling}.

% The relationship between artificial life and scaling can be argued similar to that of connectionist artificial intelligence and scaling.
% except that artificial intelligence is a lot further along in this regard.
% % In important regards, the question of scale within artificial life parallels that within artificial intelligence,
% However, .
% The development of
% AlexNet united methodological innovations from the field (e.g., big data, dropout, ReLU) with GPU computing that enabled training of orders-of-magnitude-larger networks.
% In fact, .

% Spectacular advances achieved with artificial neural networks over the last decade illuminate one conceivable progression of events.
% As with digital evolution, artificial neural networks (ANNs) were traditionally understood as a versatile but auxiliary methodology --- both techniques have been described as ``the second best way to do almost anything'' \citep{miaoulis2008intelligent,eiben2015introduction}.

A major upshot of the deep learning race is emergence of a constellation of spectacularly capable next-generation compute accelerators \citep{zhang2016cambricon,emani2021accelerating,jia2019dissecting,medina2020habana}.
Although tailored expressly to deep learning workloads, these hardware platforms represent an exceptional opportunity to leapfrog progress on grand challenges in artificial life.
The emerging class of fabric-based accelerators, led by the 850,000 core Cerebras CS-2 Wafer Scale Engine (WSE) \citep{lauterbach2021path,lie2022cerebras}, holds particular promise as a vehicle for artificial life models.
This architecture interfaces multitudinous processor elements (PEs) in a physical lattice, with PEs executing independently with private on-chip memory and interacting locally through a network-like interface.

Our work here explores how such hardware might be recruited for large-scale digital evolution, demonstrating a genetic algorithm implementation tailored to the asynchronous, dataflow-oriented computing model of the CS-2 platform.
Indeed, rapid advances in the capability of accelerator devices, driven in particular by market demand for deep learning operations, is anticipated to play a key role in future advances in agent-based model capabilities \citep{perumalla2022computer}.
The very recent CS-3 chip announcement is fitting in this respect; among other spec enhancemments, it boosts clustering support to potentiallly thousands of constituent accelerators \citep{moore2024cerebras}.

% This will require changes and impose limitations to what is possible, artificial life.
% This is not an entirely unreasonable notion of a possible future of artificial life.

\subsection{Maintaining Observability}

% more is different More is different \citep{anderson1972more}.
% Likewise, progress of artificial life systems along a path, in the most ambitious framing, to indefinite scalability seems likely to unfold through incremental investments spurred by progressive scientific achievements.
% In tandem with more farsighted efforts, progress will also require prosaic leverage of existing, commercially-available parallel and distributed compute resources at circumstantially-feasible scales.
Orthogonalities between the fundamental structure and objectives of AI and artificial life methods will complicate any effort to requisition AI hardware for artificial life purposes.
In common use, deep learning operates as a black box medium \citep{loyola2019black} (but not always \citep{mahendran2015understanding}).
This paradigm de-emphasizes accessibility of inner state.
In contrast, artificial life more often functions as a tool for inquiry.
This goal emphasizes capability to observe and interpret underlying simulation state \citep{moreno2023toward,horgan1995complexity}.
(A similar argument holds for alife work driven by artistic objectives, as well.)
% Observability is even useful in goal-oriented evolutionary computation, where it can benefit diagnostics required to tune configuration to achieve good solution quality \citep{hernandez2022can}.

Unfortunately, scale complicates simulation observability.
% Scale transforms simulation into relentless data streams with
It is not uncommon for volume and velocity of data streams from contemporary simulation to outstrip hardware bandwidth and storage capacity \citep{osti_1770192}.
Intentional engineering effort will be required to ensure large-scale simulation retains utility in pursuing rigorous hypothesis-driven objectives.
% , and this problem is ubiquitous across simulation, observational, and experimental sciences
% Observability  and interpretability \citep{} will be key concerns, as will .

% To serve as a useful experimental platform, digital evolution simulations must be observable.
Here, we confront just a single aspect of simulation observability within distributed evolutionary simulation: phylogenetic history (i.e., evolutionary ancestry relationships).
Phylogenetic history plays a critical role in many evolution studies, across study domains and \textit{in vivo} and \textit{in silico} model systems alike \citep{faithConservationEvaluationPhylogenetic1992, STAMATAKIS2005phylogenetics,frenchHostPhylogenyShapes2023,kim2006discovery,lewinsohnStatedependentEvolutionaryModels2023a,lenski2003evolutionary}.
Phylogenetic analysis can trace the history of notable evolutionary events (e.g., extinctions, evolutionary innovations), but also characterize more general questions about the underlying mode and tempo of evolution \citep{moreno2023toward,hernandez2022can,shahbandegan2022untangling,lewinsohnStatedependentEvolutionaryModels2023a}.
Particularly notable, recent work has used comparison of observed phylogenies against those produced under differing simulation conditions to test hypotheses describing underlying dynamics within real-life evo-epidemiological systems \citep{giardina2017inference,voznica2022deep}.
Additionally, \textit{in silico}, phylogenetic information can even serve as a mechanism to guide evolution in application-oriented domains \citep{lalejini2024phylogeny,lalejini2024runtime,murphy2008simple,burke2003increased}.

\subsection{Decentralized Phylogenetic Tracking}

% Unfortunately, existing approaches to recording phylogenetic history from digital evolution simulations do not scale robustly.
In order to analyze the phylogenetic history of an evolving system, we must first collect it.
In existing artificial life work, a typical approach uses centralized tracking to maintain an exact, complete record comprising all parent-offspring relationships that have existed over the course of a simulation \citep{ray1992evolution,bohm2017mabe,de2012deap,garwood2019revosim,godin2019apoget,dolson2024phylotrackpy}.
Often, records of extinct lineages are pruned to prevent memory bloat \citep{moreno2024analysis}.
Although the direct-tracking approach is well suited to serial simulation or centralized controller-worker schemes, extreme sensitivity to missing data and runtime communication overheads impede scaling to highly distributed systems --- particularly those with lean memory capacity like the Cerebras WSE \citep{moreno2024analysis}.
To overcome this limitation, we have developed reconstruction-based approaches to phylogenetic tracking \textit{in silico} \citep{moreno2022hereditary}.
These approaches require no centralized data collection during simulation runtime; instead, they use \textit{post hoc} comparisons among end-state agent genomes to deduce approximate phylogenetic history --- akin to how DNA-based analyses tell how lineages of contemporary organisms relate in natural history.
Figure \ref{fig:runtime-posthoc-schematic} summarizes this reconstruction-based strategy.

Although analogous work with natural biosequences is notoriously challenging, uncertain, biased, and data-intensive \citep{neyman1971molecular,lemmon2013high},
recent development of hereditary stratigraphy algorithms provides a genetic annotation architecture explicitly designed for fast, accurate reconstruction requiring only small amounts of data.
% Work reported here uses just 96 bits of tracking information per agent genome.
Designed for attachment to underlying replicators as a neutral annotation (akin to noncoding DNA), it is a general-purpose technique potentially applicable across study domains \citep{liben2008tracing,cohen1987computer,friggeri2014rumor}.
In a stroke of convergent thinking, Ackley's recent work reports use of ``bar code'' annotations on his self replicators to achieve a measure of coarse-grained lineage tracing \citep{ackley2023robust}.
% Details on this methodology and our proposed approach to translate it to the WSE context is provided in Section \ref{sec:methods}.

\subsection{Contributions}

In this paper, we report new software and algorithms that harness the Cerebras Wafer Scale Engine to enable radically scaled-up agent-based evolution while retaining key aspects of observability necessary to support hypothesis-driven computational experiments.
Implementation comprises two primary aspects:
\begin{enumerate}
  \item an asynchronous island-based genetic algorithm (GA) suited to the memory-scarce, highly-distributed, data-oriented WSE architecture, and
  \item a fundamental reformulation of hereditary stratigraphy's core storage and update procedures to achieve fast, simple, resource-lean annotations compatible with unconventional, resource-constrained accelerator and embedded hardware like the WSE.
\end{enumerate}

Both are implemented in Cerebras Software Language (CSL) and validated using Cerebras' SDK hardware emulator.
We use benchmark experiments to evaluate the runtime performance characteristics of the new hereditary stratigraphy algorithms in isolation and in the integrated context providing tracking-enabled support for the island-model GA.
In conjunction, we report emulated and on-device trials that validate phylogenetic reconstructions and demonstrate their suitability for inference of underlying evolutionary conditions.

Results from both experiments are promising.
We find that new surface-based algorithms greatly improve runtime performance.
Scaled-down emulator benchmarks and early on-hardware trials suggest potential for simple agent models --- with phylogenetic tracking enabled --- to achieve on the order of quadrillions of agent replication events a day at full wafer scale, with support for population sizes potentially reaching hundreds of millions.
Further, using proposed techniques, phylogenetic analyses of simulations spanning hundreds of thousands of PEs succeed in detecting differences in adaptive dynamics between alternate simulation conditions.

% \item WANT TO DO: we ran the async GA at full wafer scale on hardware with high/low selection pressure (tournament size 2 vs 8 ) and extracted  phylogenetic information; this phylogenetic information was sufficient to detect the difference in selection dynamics between the two runs.
% \end{itemize}

% Since the field's inception, artificial life has ridden a steady current of microprocessor innovation.
% As improvements in serial processing dried up around the turn of the century \citep{sutter2005free}, parallel and distributed became ascendant.
% As a result, it has become routine to dispatch independent instantiations of simulation runs across hardware units.
% In scientific contexts, this practice yields replicate datasets that provide statistical power to answer research questions \citep{dolson2017spatial}.
% In applied contexts, this practice yields many converged populations that can be scavenged for the best solutions overall \citep{hornby2006automated}.
% Another established practice is to use ``island models'' where individuals are transplanted between populations residing across distributed hardware \citep{gorges1990explicit}.
% Notably, asynchronous approaches are common and effective in these models \citep{abdelhafez2019performance}.

% Koza and collaborators’ genetic programming work with a 1,000-CPU Beowulf cluster typifies the island model approach \citep{bennett1999building}.
% In recent years, Sentient Technologies spearheaded evolutionary computation projects on an unprecedented computational scale, comprising over a million CPUs and capable of a peak performance of 9 petaflops \citep{miikkulainen2019evolving}.
% According to its proponents, the scale and scalability of this ``DarkCycle'' system was a key aspect of its conceptualization \citep{gilbert2015artificial}.
% Much of the assembled infrastructure was pieced together from heterogeneous providers and employed on a time-available basis \citep{blondeau2009distributed}.
% Unlike typical island models where selection occurs entirely independently on each CPU, this scheme transferred evaluation criteria between computational instances in addition to individual genomes \citep{hodjat2013distributed}.
% Sentient Technologies also notably exploited a large pool of hardware accelerators (e.g., 100 GPUs) in work evolving neural network architectures by performing each candidate architecture's costly model training and evaluation process \citep{miikkulainen2019evolving}.

% Existing parallel and distributed digital evolution systems typically minimize interaction between simulation components on disjoint hardware.
% Such independence facilitates simple and efficient implementation.
% This approach typically involves independent evaluation of sub-populations (i.e., island models) or individuals (i.e., primary-subordinate or controller-responder parallelism \citep{cantu2001master}).
% Cases where evaluation of a single individual are parallelized often involve data-parallel evaluation over a set of independent test cases, which are subsequently consolidated into a single fitness profile \citep{harding2007fast_springer, langdon2019continuous}.


% \section{Paths Forward}

% Implicit among much of the field, it seems, is an anticipation that order-of-magnitude changes in artificial life systems may unlock a qualitative sea change in simulation outcomes.
% This is not an entirely unreasonable notion of a possible future of artificial life.

% Spectacular advances achieved with artificial neural networks over the last decade illuminate one conceivable progression of events.
% As with digital evolution, artificial neural networks (ANNs) were traditionally understood as a versatile but auxiliary methodology --- both techniques have been described as ``the second best way to do almost anything'' \citep{miaoulis2008intelligent,eiben2015introduction}.
% However, the utility and ubiquity of ANNs has since increased dramatically \citep{marcus2018deep}.
% The development of AlexNet is widely considered pivotal to this transformation.
% AlexNet united methodological innovations from the field (such as big datasets, dropout, and ReLU) with GPU computing that enabled training of orders-of-magnitude-larger networks.
% In fact, some aspects of their deep learning architecture were expressly modified to accommodate multi-GPU training \citep{krizhevsky2012imagenet}.
% By adapting existing methodology to exploit commercially available hardware, AlexNet spurred the greater availability of compute resources to the research domain and eventually the introduction of custom hardware to expressly support deep learning \citep{jouppi2017datacenter}.

% Likewise, progress of artificial life systems along a path, in the most ambitious framing, to indefinite scalability seems likely to unfold through incremental investments spurred by progressive scientific achievements.
% To that end, observability \citep{moreno2023toward} and interpretability \citep{horgan1995complexity} will be key concerns, as will intentionally focuusing engineering effort to support hypothesis-driven objectives.
% In tandem with more farsighted efforts, progress will also require prosaic leverage of existing, commercially-available parallel and distributed compute resources at circumstantially-feasible scales.

% Such work should be made with an eye for contribution back to HPC.
% As noted earlier, the unique character of artificial life simulation suits it to serve at the tip of the spear in HPC evolution.
% High-performance computing hardware with transformative capabilities is coming to market right now, and some of it --- like the Cerebras wafer scale engine \citep{lauterbach2021path} --- is built explicitly for decentralized, asynchronous computation.
% Given ubiquity of deep net training and stencil-based numerical solvers in applications (CITE), programming for agent-based simulation can be of interest insofar as it flexes harware capabilities in unimagined ways.
% Effort to establish artificial life simulation as a flagship HPC application could be of mutual benefit.


% \section{Introduction} \label{sec:introduction}

% Agent-Based Modeling (ABM) has gained increasing adoption as a method to answer basic science questions and inform policy decisions.
% Despite a wide berth of application domains --- spanning sectors like spanning transportation infrastructure, public health, telecommunications, materials science and more --- much ABM work is unified by a common theme of interest in cross-scale dynamics.
% To provide such insight, ABM require sufficient scale to capture systems' emergent behaviors.
% Advances in high-performance computing (HPC) have already yielded paradigm-shifting improvements to the capabilities of ABM.
% However, across domains key questions still remain out of computational reach.

% Significant untapped potential for ABM scale-up has been identified in hardware-accelerator-enabled computation.
% Rapid advances in the capability of accelerator devices, driven in particular by market demand for deep learning operations, is anticipated to play a key role in future advances in ABM capabilities \citep{perumalla2022computer}.
% Within this category, the emerging class of fabric-based accelerators, most notably the recently-introduced 850,000 core Cerebras CS-2 Wafer Scale Engine (WSE) \citep{lauterbach2021path,lie2022cerebras}, is a particularly exciting --- and fairly uncharted, with applications to HPC workloads still in early days.
% This paradigm interfaces multitudinous processor elements (PEs) in a physical lattice, with PEs executing independently using individual on-chip memory and local PEs interacting through a network-like interface.

% \subsection{Objectives}

% This proposal establishes foundation for next-generation accelerator-enabled ABM computation by decentralized, approximate data export agent-based evolutionary simulation.
% In particular, we will evaluate asynchronous approaches for ABM migration/interaction on the WSE architecture to power agent-based evolution simulations, incorporating cutting-edge methods for distributed approximate phylogenetic (i.e., ancestry tree) tracking.

% Proposed work advances two technical objectives:
% \begin{enumerate}
% \item to evaluate and demonstrate new approaches for phylogenetic tracking in a massively-distributed, resource-constrained setting,
% \item to test the scalability of desynchronized agent migration procedures on WSE hardware,
% \end{enumerate}

% These technical capabilities will unlock capability to investigate a broad array of science questions.
% In this proposal, we focus on one science objective:
% \begin{enumerate}
% \item to evaluate how phylogenetic structure scales across orders-of-magnitude population sizes, and the extent to which commonly used phylogeny structure metrics are scale-invariant or scale-sensitive.
% \end{enumerate}

% Proposed work falls within the domain of agent-based evolution modeling, and uses it to explores phylogenetics-related inquiry by leveraging Cerebras WSE hardware.
% Our dual technical objectives constitute significant advancement of methodological capabilities within digital evolution, and our project will directly address fundamental open questions within the domain of phylogenetic theory.
% However, findings and methodologies will also generalize to other ABM domains beyond evolutionary simulation and to broader classes of highly-distributed HPC architectures.

% \subsection{Agent-based Evolution Simulation}

% Evolutionary processes do not confine to matters of natural history.
% Rather, evolutionary processes pervade our contemporary, everyday world.
% Key societal challenges root in evolving systems: antibiotic resistance, epidemiology, conservation biology, and oncology among others.  % citations?
% Evolutionary biology provides the fundamental foothold to efforts to address these problems \citep{aktipis2013evolutionary}.

% Mathematical and computational modeling complements natural history field work and benchtop evolution experiments as a crucial third leg to stand evolutionary inquiry.
% Simulation-based approaches provide key capabilities complementary to work with natural systems: complete observability, arbitrary manipulability, and rapid generational turnover.
% Within this context, agent-based simulation plays an important connective role between natural systems and abstracted, aggregate-based mathematical and numerical models.
% Agent-based approaches instantiate \textit{bona fide} evolutionary processes that track populations of virtual genomes subject to mutation, heredity, and selection \citep{pennock2007models}.
% This characteristic incorporates some of the critical complications and subtleties characteristic of natural systems --- e.g., arbitrary agent behavior, sophisticated agent-agent interactions, complex genotype-phenotype maps, albeit at significantly reduced scope and sophistication.

% Indeed, agent-based evolution approaches have provided means for fruitful investigation of wide-ranging hypotheses, including evolution of evolvability \citep{wilke2001evolution}, host-parasite co-evolution \citep{zaman2014coevolution}, evolution of complex traits \citep{lenski2003evolutionary}.

% Ambitious work advancing the field increasingly targets large cross-scale questions, including major transitions in evolution (e.g., multicellularity and symbiosis) \citep{goldsby2020major,vostinar2021symbiosis} and open-ended evolution (e.g., long-term trajectories of complex ecosystems with strong biotic selection) \citep{stanley2019open,taylor2016open}.
% Progress on these fronts demands computational substrate for orders-of-magnitude larger simulation scale than tractable today \citep{moreno2022exploring,channon2019maximum}.

% %as well as scenarios where replicating entities like cultural artifacts or computer viruses.
% % At the frontiers of evolutionary computation, there is in particular growing interest in the question of ``open-ended evolution'' \citep{}.
% % This refers to the problem of the inability to recreate the ongoing generation of novelty, complexity, and adaptation within the natural world.

% \subsection{HPC and Agent-based Evolution}
% % opportunity


% % Evolutionary questions often explicitly span scopes, with key areas of inquiry including ecologies of interacting populations and assembly of individuals into multicellular organisms and eusocial colonies \citep{morenoDISHTINYDOTO, citephageDOTO}.
% Researchers using agent-based evolution recognize HPC as critical to the future of the field \citep{ackley2016indefinite}.
% Indeed, the field has played host to notable boundary-pushing approaches to computing at the frontiers of computing hardware and modalities such as best-effort computing, reservoir computing, global-scale time-available computing, and modular tile-based computing in addition to more traditional cluster and GPU-oriented approaches \citep{moreno2021conduit,ackley2020best,ackley2023robust,heinemann2008artificial,miikkulainen2024evolving}.
% The diversity and, in cases, novelty of HPC within evolutionary simulation stems in large part from unique properties largely distinct from other HPC application domains.

% Given its inherent underlying stochastic nature and the stabilizing influence of adaptive selection, evolutionary simulation can often tolerate significant arbitrary asynchronicity or even entirely lost simulation components (e.g., dropped messages, crashed nodes, etc.).
% Likewise, digital evolution is typically amenable to locality restrictions of computation due to the inherent spatial structure of natural systems we are seeking to model.
% % In particular, massively-distributed, spatial computing being directly highlighted to be of particular interest \citep{ackleyDOTO}.
% Because agent behavior evolves over time, the influence of population-level drift and adaptive change can inject extreme heterogeneity to the computational workload profile of evolutionary simulation over time and simulation space.
% Finally, emerging directions have begun to tilt implementation towards more challenging communication-intensive qualities.
% The largely-decoupled nature of classic approaches within evolutionary computation like island models or controller/worker schemes  \citep{bennett1999building,cantu2001master} no longer suffice to realize the dynamic, communication-intensive interaction characteristic of major transitions and open-ended evolution \citep{moreno2022engineering}.

% These distinctive properties, position agent-based evolution as a potentially valuable testbed for HPC innovation and leadership.
% There is reason to expect a highly synergistic, reciprocal relationship between digital evolution and the broader HPC enterprise.
% Work proposed here steps in this direction, seeking to blaze new territory that opens new possibilities to benefit broader constituencies of ABM/HPC practitioners.

% However, despite the strong motivation for large-scale simulation, the algorithmic pliability of evolutionary simulation, and the increasing availability of highly-capable parallel, distributed, and accelerator-driven hardware platforms, significant methodological limitations currently hold back progress achieving widespread scale-up the field of digital evolution.
% Through work proposed here, we will take significant steps to resolving this knot and thereby position the field to benefit significantly from this emerging class of hardware accelerators.

% \subsection{Phylogenetic Tracking Methods}

% To serve as a useful experimental platform, digital evolution simulations must be observable.
% In addition to end-state information (i.e., evolved traits), scientific questions demand information sufficient to characterize underlying mode and tempo of evolution.
% Additionally, it is often useful to be able to trace the history of notable evolutionary events (e.g., extinctions, evolutionary innovations)
% Observability counts, too, in application-oriented aspects of evolutionary computation, where such data serves as a critical diagnostic to tune configuration for good performance \citep{hernandez2022can}.

% In evolutionary biology, phylogenetic history is a valuable tool to triangulating the context of notable evolutionary events, as well as characterizing the underlying mode and tempo of evolution.
% The same holds true in evolutionary simulation.
% % https://github.com/mmore500/phylotrack-algorithm-analysis/blob/fe16d2b2d7df99faade09c01b72f681160749f51/tex/text/body/introduction.tex
% In addition to addressing questions of natural history, access to the phylogenetic record of biological life has proven informative to conservation biology, epidemiology, medicine, and biochemistry among other domains \citep{faithConservationEvaluationPhylogenetic1992, STAMATAKIS2005phylogenetics, frenchHostPhylogenyShapes2023,kim2006discovery}.
% Nonetheless, existing analyses of phylogenetic structure within digital systems have already proven valuable, enabling diagnosis of underlying evolutionary dynamics \citep{moreno2023toward,hernandez2022can,shahbandegan2022untangling, lewinsohnStatedependentEvolutionaryModels2023a} and even serving as mechanism to guide evolution in application-oriented domains \citep{lalejini2024phylogeny,lalejini2024runtime,murphy2008simple,burke2003increased}.
% Further, comparison of observed phylogenies against simulation phylogenies can be used to evaluate hypotheses for underlying dynamics within real-life evolutionary/epidemiological systems \citep{giardina2017inference,voznica2022deep}.

% Unfortunately, existing approaches to recording phylogenetic history from digital evolution simulations do not scale robustly.
% Simulation phylogenies have typically been collected using a centralized record-keeping approach where every reproduction event is stitched together in a tree data structure to produce a complete record.
% Record-keeping often involves pruning the records of extinct lineages to prevent memory bloat \citep{dolson2023phylotrack}.
% Although the direct-tracking approach is well suited to serial simulation substantial limitations and runtime overhead make scaling this up to highly parallel/distributed systems --- particularly those with low memory capacity like the Cerebras WSE --- essentially untenable \citep{moreno2024analysis}.

% To overcome this limitation to phylogenetic analysis within many-processor HPC contexts, we have proposed a new class of reconstruction-based approaches to phylogenetic tracking in silico \citep{moreno2022hereditary}.
% These approaches require no centralized data collection during simulation runtime; instead, they use post hoc comparisons between end-state agent genomes to deduce approximate phylogenetic history --- akin to how DNA-based analyses tell how lineages of contemporary organisms relate in natural history.
% Figure \ref{fig:runtime-posthoc-schematic} depicts our reconstruction-based strategy.

% To achieve efficient, tractable phylogenetic reconstructions in practice, some careful consideration is required.
% DNA-based is notoriously data-hungry, typically requiring on the order of thousands of genome sites, and can be significantly biased by physical/functional traits of the underlying genetic information.
% These concerns motivated our recent development of HStrat, a genetic architecture explicitly designed for fast, accurate reconstruction requiring only small amounts of data.
% HStrat data is designed to be attached to the underlying genomes within particular digital evolution systems as a neutral annotation.
% Benchmarking experiments to evaluate HStrat performance have achieved high-quality reconstruction of phylogenetic histories for tens of thousands of fully-distributed agents using just 96 bits of tracking information per agent genome.
% Details on this methodology and our proposed approach to translate it to the WSE context is provided in Section \ref{sec:methods}.


==> binder-wafer-scale/tex/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

This section details the algorithm and implementation design used in this work.
After briefly recounting the core mechanics of hereditary stratigraphy methods for phylogenetic tracking, we motivate and describe new lightweight ``surface'' data structures used to annotate agent genomes in this work.
Then, we describe the asynchronous compute-communicate implementation strategy behind the testbed WSE-oriented island-based genetic algorithm used for validation and benchmarking experiments.

\subsection{Distributed Phylogenetic Tracking}

Natural history of biological life operates under no extrinsic provision for interpretable record-keeping, yet efforts to study it have proved immensely fruitful.
This fact bodes well that scaled-up simulation studies can succeed as a platform for rich hypothesis-driven experiments despite potential sacrifices to aspects of observability currently enjoyed with centralized, storage-rich processing.
Indeed, observational and analytical strategies already developed to confront limitations in biological data can solve, or at least guide, work with massively distributed evolution simulations.

In biology, mutational drift encodes ancestry information in DNA genomes.
Our proposed methods are analogous, with ancestry information contained within genomes themselves rather than in any external tracking mechanism.
Phylogenetic history can then be estimated after the fact, as depicted in Figure \ref{fig:runtime-posthoc-schematic}.
This process ensures low runtime communication overhead, as well as near-total resiliency to germane modes of data loss (e.g., dropped messages, hardware crash-out).

Recent work introducing \textit{hereditary stratigraphy} (hstrat) methodology has explored how best to organize genetic material to maximize reconstruction quality and minimize memory footprint \citep{moreno2022hstrat, moreno2022hereditary}.
Hstrat material can be bundled with agent genomes in a manner akin to non-coding DNA, entirely neutral with respect to agent traits and fitness.

The hereditary stratigraphy algorithm associates each generation along individual lineages with an identifying ``fingerprint'' value, referred to as a differentia.
On birth, offspring recieve a new differentia value and append it to an inherited chronological record of past values, each corresponding to a generation along that lineage.
Under this scheme, mismatching differentiae can be used to delimit the extent of common ancestry.
This semantic streamlines \textit{post hoc} phylogenetic reconstruction to a simple trie-building procedure
\citep{moreno2024analysis}.

To save space, differentia may be pruned away.
However, care must be taken to ensure retention of checkpoint generations that maximize coverage across evolutionary history.
Reducing the number of bits per differentia can also provide many-fold memory space savings.
This savings can be re-invested to increase the quantity of differentia retained, improving the density of record coverage across elapsed generations.
The cost of this shift is an increased probability of spurious differentia value collisions, which can make two lineages appear more closely related than they actually are.
We anticipate that most use cases will call for differentia sized on the order of a single bit or a byte.
Indeed, single-bit differentiae have been shown to yield good quality phylogenies using only 96 bits per genome \citep{moreno2024guide}.

Small differentia size intensifies need for a lean data structure to back differentia record management.
Shrinking differentia to a single bit would be absurd if each is accompanied by a 32-bit generational timestamp.
To safely drop timestamps, though, we need means to recalculate them on demand.
As such, all described algorithms include means to deduce timestamps of retained differentia solely from their storage index and the count of the record's elapsed generations.

Lastly, design of hstrat annotations must also consider how available storage space should be allocated across the span of history.
In one possible strategy, retained time points would be distributed evenly across history.
In another, more recent time points would be preferred.
We term these as ``steady'' and ``tilted'' policies, respectively \citep{han2005stream,zhao2005generalized}.
Note that prior hereditary stratigraphy work refers to them instead as ``depth-proportional'' and ``recency-proportional resolution'' \citep{moreno2022hereditary}.
Comparisons of reconstruction quality have shown that tilted policy gives higher quality reconstructions from the same amount of reconstruction space in most --- but not all --- circumstances \citep{moreno2024guide}.
This pattern follows an intuition that high absolute precision is more useful to resolving recent events than more ancient ones.
In practice, it may be desirable to use a hybrid approach that allocates half of available annotation space to each strategy \citep{moreno2024guide}.
Figure \ref{fig:surf-algorithms} includes retention drip plots that contrast behavior of steady and tilted algorithms.

\subsection{Surface-based Hereditary Stratigraphy Algorithms}

% Although designed with efficiency in mind, existing ``column''-based  have several properties that make them a poor fit with a resource-constrained environment like the the Cerebras WSE:
At the outset of this project, several problematic aspects of porting existing hereditary stratigraphy algorithms to the WSE became apparent.
Issues stemmed, in part, from a fundamental feature of these algorithms: organization of retained strata in contiguous, sorted order.
Forthwith, we refer to algorithms following this convention as ``column''-based.
The column design, and attendant implementation details, impose various drawbacks:
\begin{itemize}
\item \textbf{wasted space}: an annotation size cap can be guaranteed, but a percentage of available space typically goes unused;
\item \textbf{high-level feature dependencies:} in places, existing column code uses complex data structures with dynamically allocated memory to perform operations like set subtraction,
\item \textbf{annotation size scaling:} procedures to maintain sorted order among differentia can take time linearly proportional to annotation size.
% \item \textbf{expensive operations:} in places, slow divide and modulo operations. heavy use
\end{itemize}

\input{fig/surf-vs-column-schematic}

Addressing these concerns required fundamental reformulation of hereditary stratigraphy conventions.
To this end, we introduce a constant-time indexing scheme that maps each lineage's fingerprint stream directly onto a fixed-width memory buffer.
Differentia pruning occurs implicitly, as a result of resident differentia being overwritten by new placements.
As before, care is taken to guarantee temporally-representative collections of resident differentiae within the memory buffer over elapsed time.
We refer to this new approach as ``surface''-based, as opposed to ``column''-based.
Figure \ref{fig:surf-vs-column-schematic} contrasts the two.
% to distinguish it from earlier conventions


% New approach uses a constant-time indexing scheme that maps each lineage's fingerprint stream onto a fixed-width memory buffer such that eviction of existing fingerprint values by new placements maintains a temporally-representative sampling over elapsed time .
% We call this approach ``surface''-based to distinguish it from earlier hereditary stratigraphy methods.
% As before, time stamps can be positionally inferred and thus do not need to be stored --- a several-fold savings that enables fingerprint values to be shrunk down and packed together.


\input{fig/surf-algorithms}

In the course of this work, we developed both steady- and tilted-policy surface-based hereditary stratigraphy algorithms.
Figure \ref{fig:surf-algorithms} depicts implementation behaviors, with the top panels tracking how placements are sequenced over time in buffer space and the bottom panels showing the resulting distributions of retained time points across history.
We leave formal descriptions of underlying indexing algorithms to future work.
However, reference Python implementations can be found in provided software materials.
For this work, we also translated the tilted algorithm to the general-purpose Zig programming language and then to the Zig-like Cerebras Software Language for use on the WSE.

These algorithms are notable in providing a novel and highly efficient solution the more general problem of curating dynamic temporal cross-samples from a data stream, and may lend themselves to a broad set of applications outside the scope of phylogeny tracking \citep{moreno2024algorithms}.

% async microthread to send from sendBuf to neighbor
% fn dispatchSend_S() void {
%   @fmovs(sendDsd_S, sendBufDsd_S,
%     .{
%       .async = true,
%       .activate = sendFinalizeTaskID_S

% const recvDsd_N = @get_dsd(fabin_dsd, .{
%   .fabric_color = recvColor_N,
%   .extent = recvBufSize,
%   .input_queue = @get_input_queue(q_in_N)
% });
% // open an async microthread to recv from neighbor into recvBuf
% fn dispatchRecv_N() void {
%   @fmovs(recvBufDsd_N, recvDsd_N,
%     .{
%       .async = true,

% color swapping

\subsection{WSE Architecture and Programming Model}

The Cerebras Wafer Scale Engine comprises a networked grid of independently executing compute cores (Processing Elements or PEs).
Each PE contains special message-handling infrastructure, which routes tagged 32-bit packets (``wavelets'') to neighboring PEs and/or to be processed locally, according to a programmed rule set.
Each Processor Element is equipped with 48kb of private on-chip memory, which can be accessed within a single clock cycle;
communication to neighboring PEs, too, incurs low latency \citep{buitrago2021neocortex}.
Processor Elements provide faculties for standard arithmetic and flow-control operations, as well as vectorized 32- and 16-bit integer and floating-point operations.

The WSE device is programmed by providing ``kernel'' code, written in the Cerebras Software Language (CSL), to be executed on each PE.
This language's programming model purposefully reflects underlying capabilities and particularities of the WSE architecture.
CSL organizes code within an event-driven framework, with the programmer defining tasks to be triggered in response to wavelet activation signals exchanged between --- and within --- PEs.
Scheduling of active tasks occurs via hardware-level microthreading, which allows for some level of concurrency.
Special faculties are provided for asynchronous send-receive operations that exchange contiguous, or strided, buffer data between PEs.

For further detail, we refer readers to extensive developer documentation made available by Cerebras through their SDK program.
Access can be requested, currently free of charge, via their website.
For this initial work, we evaluated some CSL code on a virtualized $3\times3$ PE array emulated with conventional CPU hardware, while other experiments used a physical CS-2 device.
(Scale-down to $3\times3$ was necessary to accommodate significant emulation-layer slowdown.)

\subsection{Asynchronous Island-model Genetic Algorithm}

\input{fig/async-ga-schematic}

We apply an island-model genetic algorithm, common in applications of parallel and distributed computing to evolutionary computation, to instantiate a wafer-scale evolutionary process spanning PEs \citep{bennett1999building}.
Under this model, PEs host independent populations that interact through migration (i.e., genome exchange) between neighbors.

Our implementation unfolds according to a generational update cycle, schematized in Figure \ref{fig:async-ga-schematic}.

Migration, depicted as blue-red arrows in Figure \ref{fig:async-ga-schematic}, is handled first.
% fully-asynchronous approach to migration between neighboring PEs.
% Evolutionary processes tend to occur in asynchronous manner with arbitrary factors influencing things, so this is a reasonable relaxation to make.
Each PE maintains independent immigration buffers and emigration buffers dedicated to each cardinal neighbor, depicted by Figure \ref{fig:async-ga-schematic} in solid blue and red, respectively.
On simulation startup, asynchronous receive operations are opened to accept genomes from each neighboring PE into its corresponding immigration buffer.
At startup, additionally, each emigration buffer is populated with genomes copied from the population and an asynchronous send request is opened for each. %to dispatch wavelets containing genome data from the emigration buffer to the neighbor.
Asynchronous operations are registered to on-completion callbacks that set a per-buffer ``send complete'' or ``receive complete'' flag variable.
In this work, we arbitrarily size send buffers to hold one genome and receive buffers to hold four genomes.
The main population buffer was sized to 32 genomes.

Subsequently, the main update loop tests all ``send complete'' and ``receive complete'' flags.
For each immigration flag that is set, buffered genomes are copied into the main population buffer, replacing randomly chosen population members.
Then, the flag is reset and a new receive request is initiated.
Likewise, for each emigration flag set, corresponding send buffers are re-populated with randomly sampled genomes from the main population buffer.
Corresponding flags are then reset and new send requests are initiated.
The bottom right corner of Figure \ref{fig:async-ga-schematic} summarizes the interplay between send/receive requests, callbacks, flags and buffers.

The remainder of the main update loop handles evolutionary operations within the scope of the executing PE.
Each genome within the population is evaluated to produce a floating point fitness value.
For this initial work, we use a trivial fitness function that explicitly models additive accumulation of beneficial/deleterious mutations as a floating point value within each genome.
% However, modular implementation ensures evaluation criteria can be chosen appropriate for underlying experimental objectives.

After evaluation, tournament selection is applied. % with, in our experiments, tournament size 5.
Each slot in the next generation is populated with a genome exhibiting maximal fitness among $n=5$ randomly sampled individuals, ties broken randomly.

Finally, a mutational operator is applied across all genomes in the next population.
% As with evaluation criteria, modular implementation allows mutation operations to be defined based on experimental objectives.
Experiments used a simple Gaussian mutation on each genome's stored fitness value, with sign restrictions used to manipulate the character of selection in some treatments.
At this point, hereditary stratigraphy annotations --- discussed next --- are updated to reflect an elapsed generation.

The process then repeats, with a self-activating wavelet dispatched to execute the next cycle of the main generation loop, until a generation count halting condition is met.

\subsection{Genome Model}

% Kernel source code implementing described procedures can be viewed at \url{https://hopth.ru/cl}.
% Our implementation is defined modularity with respect to genome size, layout, mutational operator, and fitness evaluation criteria, allowing for direct re-use of produced software for follow-on evolution experiments on WSE hardware.
At implementation level, genomes were handled as fixed-length segments of raw memory.
We used a 96-bit genome layout for clade reconstruction experiments, shown in Supplementary Figure \ref{fig:genome-layout} \citep{moreno2024supplement}.
The first sixteen bits were used to identify genomes descending from the same founding ancestor.
At the outset of simulation, founding population members were each assigned a randomized tag value, and the value was inherited without mutation over the course of simulation.
The next 80 bits were used for hereditary stratigraph annotation, 16 bits for a generation counter and the remaining 64 as a field for single-bit differentia managed according to a tilted surface policy.
For other experiments, a 128-bit genome layout was used instead, with the first 32 bits used for a floating point ``fitness'' value and the generation counter upgraded from 16 to 32 bits.
% A key question will be the extent to which intentionally desynchronizing affects performance, stability, and computation quality.

\subsection{Software and Data Availability}

Software, configuration files, and executable notebooks for this work are available via Zenodo at \url{https://doi.org/10.5281/zenodo.10974998}.
Data and supplemental materials are available via the Open Science Framework at \url{https://osf.io/bfm2z/} \citep{foster2017open}.

Hereditary stratigraphy utilities are published in the \texttt{hstrat} Python package \citep{moreno2022hstrat}.
This project uses data formats and tools associated with the ALife Data Standards project \citep{lalejini2019data} and benefited from many pieces of open-source scientific software \citep{huerta2016ete,2020SciPy-NMeth,harris2020array,reback2020pandas,mckinney-proc-scipy-2010,cock2009biopython,waskom2021seaborn,hunter2007matplotlib,moreno2024apc,moreno2024pecking,moreno2024hsurf,moreno2024wse,dolson2024phylotrackpy}.

WSE experiments reported in this work used the CSL compiler and CS-2 hardware emulator bundled with the Cerebras SDK v1.0.0 \citep{selig2022cerebras}, available via request form on the Cerebras website.
SDK utilities can be run from any Linux desktop environment, regardless of access to Cerebras hardware.
On-hardware trials used computational time on the PSC Neocortex installation \citep{buitrago2021neocortex}.

% Cerebras currently makes SDK materials available upon request, which can be .
% In preparation for proposed work, we joined the Cerebras SDK program \citep{selig2022cerebras} and assembled Cerebras Software Language (CSL) software implementations that will be necessary to conduct experiments with WSE hardware.
% Access to the SDK can be requested, currently free of charge, via their website.
% For the time being, we have used Cerebras' hardware emulator to test our software implementations.


==> binder-wafer-scale/tex/text/body/results-and-discussion.tex <==
\section{Results and Discussion} \label{sec:results}

Here, we report a series of benchmarks that evaluate the viability of our proposed approaches to harness the CS-2 accelerator for digital evolution simulations and extract phylogenetic records from said simulations.
First, we compare the performance characteristics of new surface-oriented hereditary stratigraphy methods against preceding column-based implementation to determine the extent to which they succeed in streamlining runtime operation.
%For assessment of  we refer the reader to related work CITE.
Then, we benchmark phylogeny-tracked WSE genetic algorithm implementations.
To assess the runtime overhead of surface-based tracking, we compare against benchmarking results with phylogenetic tracking disabled.
Finally, we validate the credibility of the presented end-to-end annotation-to-reconstruction pipeline by reviewing clade structure and phylometric properties from emulated and on-hardware runs.
% Finally, we show example phylogenies generated from on-hardware simulations under different selection pressure conditions and test the capability of inference from extracted phylogenetic information to detect differing selection pressure conditions.

\subsection{Surface Algorithm Benchmark on Conventional CPU}

\input{fig/benchmarking}

We performed microbenchmark experiments to test computational efficiency gains from new surface-based algorithms.
Trials measured the per-generation execution time of repeated sequential updates to one annotation with capacity for 64 differentia. % TODO check this
Benchmarks were conducted both using Python, for comparability with existing column algorithm implementations, and Zig, to assess performance in absolute terms under compiler optimization.
Figure \ref{fig:benchmarking} overviews results.

% Due to limited completed implementations of compiled-language algorithms, we performed the bulk of benchmarking using the Python implementations.
% However, in the process of porting the tilted surface algorithm over to Cerebras Software Language, we did create an implementation of that algorithm in Zig which is a compiled language and is capable of compiler optimizations.
% We augment the Python with a benchmark of this algorithm.

% https://github.com/mmore500/hstrat-surface-concept/blob/51d636d768d474fc5148b9fcaa199c1b7776e915/benchmark.ipynb
Python implementations of the surface tilted and steady algorithms both took around 4.2 microseconds per operation (SEM approx. 50; $n=20$).
For context, this speed was about $4\times$ the measured time for a surface placement using a trivial calculation (SEM approx. 0.05; $n=20$).
As expected, column implementations of steady and tilted fared much worse, taking about $7\times$ and $34\times$ the execution time per operation compared to the surface operations.
In both cases, surface implementations significantly outperformed their column counterparts (Mann-Whitney U test, $\alpha = 0.05$).
It should be noted that these results reflect an intrinsic performance penalty due to interpreter overhead of Python evaluation.
However, comparisons among these Python implementations are nonetheless informative because all are on equal footing in this regard.
% While Python is an interpreted language and the Python-implemented algorithms weren't specifically implemented to maximize performance and suffer an intrinsic performance penalty due to that, the algorithms were all on the same footing and
% We use the ``optimize''' flag to strip superfluous safety checks.

% https://github.com/mmore500/wse-sketches/blob/d4ab0155f63ff5809f8eeca1169ad9b272c30a68/binder/benchmark.ipynb
Zig microbenchmarks clock tilted surface annotation updates at 233 ns per operation (SEM 0.9; $n=20$).
For context, this time is a little more than twice that required for a main memory access in contemporary computing hardware \citep{markus2022memory}.
Our results measure the operation at $47\times$ the measured time for a trivial placement calculation (SEM 0.2; $n=20$).
Steady results are not included in this comparison due to a Zig implementation not yet being completed.

Low-hanging speedups and optimizations exist to further improve the per-operation surface update performance achieved in practice.
Half of update operations on surfaces with single-bit differentia can be skipped entirely, owing to 50\% probability that randomization fails to change a stored differentia value.
Further, simulations with synchronous or near-synchronous generations can cache calculated surface-placement indices, meaning they would only need to be computed once for an entire subpopulation.
Another possibility is to coarsen temporal resolution, only updating annotations at intervals every $n$th generation.

\subsection{WSE Island-model GA Benchmark}

Next, we used an emulator to characterize the expected performance of our island model genetic algorithm on WSE hardware and estimate the magnitude of simulation that might be achieved with on-device execution.
We used the emulator's per-PE clock cycle counters to measure the amount of real time elapsed over the course of a 40 generation-cycle simulation.
We tested using a $3\times3$ PE collective with the tagged 3-word genome and a per-PE population size of 32, applying a tilted hereditary stratigraphy every generation.
PEs completed a mean of 24,138 generation-cycles per second (SEM 99; $n=9$).
As an indicator of inter-PE exchange throughput, each PE immigrated a mean of 118 genomes (SEM 11; $n=9$) over 40 elapsed generation-cycles.

% https://osf.io/tf89g
What scale of simulation does this performance imply at full scale on CS-2 hardware?
Across eight on-device, tracking-enabled trials of 1 million generations (described in the following section), we measured a mean simulation rate of 17,688 generations per second for 562,500 PEs ($750\times750$ rectangle) with runtimes slightly below one minute.
As a point of comparison, eight trials trials conducted with 1,600 PEs ($40\times40$) yielded a similar mean generation rate of 17,734 hz.

Multiplied out to a full day, a 17 generations per second turnover rate would elapse around 1.5 billion generations.
With 32 individuals hosted per each of 850,000 PEs, the net population size would sit around 27 million at full CS-2 wafer scale.
(Note, though, that available on-chip memory could support thousands of our very simple agents per PE, raising the potential for a net population size on the order of a billion agents.)
% 24,000 * 850,000 * 60 * 60 * 24 * 32 ---> ?? quadrillion
A naive extrapolation estimates on the order of a quadrillion agent replications could be achieved hourly at full wafer scale for such a very simple model.
We look forward to conducting more thorough benchmarking and scaling experiments in future work.
%The barebones simplicity of the model should also be noted.

Recall that these figures are inclusive of phylogenetic tracking.
How fast does simulation run without hereditary stratigraphy instrumentation?
Using the hardware emulator, we repeated our benchmark using one-word genomes stripped of all instrumentation.
Under these conditions, PEs completed a mean of 47,175 generations per second (SEM 220; $n=20$)
As before, over the course of simulation, each PE immigrated on average 118 genomes (SEM 12; $n=12$).

These timings indicate cost of phylogeny tracking as approximately equivalent to that of the other aspects of simulation, combined.
Given the highly minimalistic nature of the agent model and selection process, this result is highly promising.
In actual use, most experiments will likely involve a much more sophisticated agent model; thus, the relative overhead of tracking will diminish significantly.
It is additionally worthwhile to note that caching and coarsening strategies discussed above have not yet been applied, which may reduce performance penalty of tracking considerably.

% https://github.com/mmore500/wse-sketches-mirror/actions/runs/8590107511/job/23537207835
% from https://github.com/mmore500/wse-sketches-mirror/commit/3a1bf8e9f2820a38cb7387a7624a86361485174b
% ASYNC_GA_GENOME_FLAVOR genome_purifyingplus
% ASYNC_GA_GLOBAL_SEED 0
% ASYNC_GA_NCYCLE_AT_LEAST 40
% ASYNC_GA_MSEC_AT_LEAST 0
% ASYNC_GA_TSC_AT_LEAST 0
% INFO: Using SIF: /home/runner/cerebras/bin/cbcore_sdk-202311111408-10-4a54bce5.sif
% INFO: User's specified CSL_IMPORT_PATH=
% NOTE: CSL_IMPORT_PATH accepts colon separated list of paths generated by 'realpath <path>'
% INFO:    Environment variable SINGULARITYENV_CSL_SUPPRESS_SIMFAB_TRACE is set, but APPTAINERENV_CSL_SUPPRESS_SIMFAB_TRACE is preferred
% compile successful
% Updated 1 path from the index
% CS_PYTHON cs_python
% INFO: Using SIF: /home/runner/cerebras/bin/cbcore_sdk-202311111408-10-4a54bce5.sif
% INFO:    Environment variable SINGULARITYENV_CSL_SUPPRESS_SIMFAB_TRACE is set, but APPTAINERENV_CSL_SUPPRESS_SIMFAB_TRACE is preferred
% whoami ===============================================================
% [[0 3 6]
%  [1 4 7]
%  [2 5 8]]
% whereami x ===========================================================
% [[0 1 2]
%  [0 1 2]
%  [0 1 2]]
% whereami y ===========================================================
% [[0 0 0]
%  [1 1 1]
%  [2 2 2]]
% cycle counter =======================================================
% [[40 40 40]
%  [40 40 40]
%  [40 40 40]]
% recv counter N ========================================================
% [[ 1  1  1]
%  [ 9 13 11]
%  [15 12 12]]
% recv counter S ========================================================
% [[ 7  9  8]
%  [10 11  9]
%  [ 1  1  1]]
% recv counter E ========================================================
% [[12 11  1]
%  [12 13  1]
%  [ 9 13  1]]
% recv counter W ========================================================
% [[ 1 11  9]
%  [ 1  7  9]
%  [ 1 10 11]]
% recv counter sum =====================================================
% [21, 32, 19, 32, 44, 30, 26, 36, 25]
% np.mean(recvSum)=29.444444444444443 np.std(recvSum)=7.304657739508267 sps.sem(recvSum)=2.5825865109265465
% send counter N ========================================================
% [[ 0  0  0]
%  [24 32 34]
%  [40 46 34]]
% send counter S ========================================================
% [[38 50 46]
%  [58 50 48]
%  [ 0  0  0]]
% send counter E ========================================================
% [[44 32  0]
%  [24 32  0]
%  [40 46  0]]
% send counter W ========================================================
% [[ 0 50 46]
%  [ 0 50 48]
%  [ 0 36 48]]
% send counter sum =====================================================
% [82, 132, 92, 106, 164, 130, 80, 128, 82]
% np.mean(sendSum)=110.66666666666667 np.std(sendSum)=27.744869395579748 sps.sem(sendSum)=9.809292646374773
% tscControl values ====================================================
% [30064968187, 30064968187, 30064968187, 30064968187, 30064968187, 30064968187, 30064968187, 30064968187, 30064968187]
% tscStart values ======================================================
% [2220, 2222, 2731, 2731, 1716, 2738, 3241, 3243, 3237]
% tscEnd values ========================================================
% [1414233, 1414662, 1406657, 1388294, 1438771, 1433887, 1412082, 1403426, 1390454]
% tsc diffs ============================================================
% --------------------------------------------------------------- ticks
% [1412013, 1412440, 1403926, 1385563, 1437055, 1431149, 1408841, 1400183, 1387217]
% np.mean(tsc_ticks)=1408709.6666666667 np.std(tsc_ticks)=16415.157825754963 sps.sem(tsc_ticks)=5803.63470641938
% -------------------------------------------------------------- seconds
% [0.0016611917647058824, 0.0016616941176470588, 0.0016516776470588235, 0.0016300741176470588, 0.0016906529411764705, 0.0016837047058823528, 0.00165746, 0.0016472741176470588, 0.00163202]
% np.mean(tsc_sec)=0.0016573054901960784 np.std(tsc_sec)=1.9311950383241098e-05 sps.sem(tsc_sec)=6.827805536963963e-06
% ---------------------------------------------------- seconds per cycle
% [4.152979411764706e-05, 4.154235294117647e-05, 4.129194117647059e-05, 4.075185294117647e-05, 4.226632352941176e-05, 4.209261764705882e-05, 4.1436499999999995e-05, 4.1181852941176466e-05, 4.0800500000000003e-05]
% np.mean(tsc_cysec)=4.143263725490196e-05 np.std(tsc_cysec)=4.827987595810268e-07 sps.sem(tsc_cysec)=1.7069513842409884e-07
% ---------------------------------------------------------- cycle hertz
% [24079.09842189838, 24071.81897992127, 24217.800653310787, 24538.761499837972, 23659.498070707108, 23757.135001317125, 24133.312417795907, 24282.540210815303, 24509.50356000539]
% np.mean(tsc_cyhz)=24138.829868401026 np.std(tsc_cyhz)=280.43062795032466 sps.sem(tsc_cyhz)=99.14719933803819
% --------------------------------------------------------- ns per cycle
% [41529.79411764706, 41542.35294117647, 41291.94117647059, 40751.852941176476, 42266.32352941176, 42092.61764705882, 41436.49999999999, 41181.85294117647, 40800.5]
% np.mean(tsc_cyns)=41432.63725490196 np.std(tsc_cyns)=482.7987595810264 sps.sem(tsc_cyns)=170.6951384240987
% fitness =============================================================
% [[0.00316905 0.00565182 0.0022315 ]
%  [0.00687918 0.00742484 0.00589414]
%  [0.00582986 0.0057458  0.00379858]]


% https://github.com/mmore500/wse-sketches-mirror/actions/runs/8590107511/job/23537207835
% from https://github.com/mmore500/wse-sketches-mirror/commit/3a1bf8e9f2820a38cb7387a7624a86361485174b
% CSLC cslc
% ASYNC_GA_GENOME_FLAVOR genome_purifyingstripped
% ASYNC_GA_GLOBAL_SEED 0
% ASYNC_GA_NCYCLE_AT_LEAST 40
% ASYNC_GA_MSEC_AT_LEAST 0
% ASYNC_GA_TSC_AT_LEAST 0
% INFO: Using SIF: /home/runner/cerebras/bin/cbcore_sdk-202311111408-10-4a54bce5.sif
% INFO: User's specified CSL_IMPORT_PATH=
% NOTE: CSL_IMPORT_PATH accepts colon separated list of paths generated by 'realpath <path>'
% INFO:    Environment variable SINGULARITYENV_CSL_SUPPRESS_SIMFAB_TRACE is set, but APPTAINERENV_CSL_SUPPRESS_SIMFAB_TRACE is preferred
% compile successful
% Updated 1 path from the index
% CS_PYTHON cs_python
% INFO: Using SIF: /home/runner/cerebras/bin/cbcore_sdk-202311111408-10-4a54bce5.sif
% INFO:    Environment variable SINGULARITYENV_CSL_SUPPRESS_SIMFAB_TRACE is set, but APPTAINERENV_CSL_SUPPRESS_SIMFAB_TRACE is preferred
% whoami ===============================================================
% [[0 3 6]
%  [1 4 7]
%  [2 5 8]]
% whereami x ===========================================================
% [[0 1 2]
%  [0 1 2]
%  [0 1 2]]
% whereami y ===========================================================
% [[0 0 0]
%  [1 1 1]
%  [2 2 2]]
% cycle counter =======================================================
% [[40 40 40]
%  [40 40 40]
%  [40 40 40]]
% recv counter N ========================================================
% [[ 1  1  1]
%  [13 11 14]
%  [11  7 11]]
% recv counter S ========================================================
% [[ 9 13  9]
%  [11 13 11]
%  [ 1  1  1]]
% recv counter E ========================================================
% [[11 15  1]
%  [ 7 11  1]
%  [ 7  9  1]]
% recv counter W ========================================================
% [[ 1  7  9]
%  [ 1  9 13]
%  [ 1 11 13]]
% recv counter sum =====================================================
% [22, 36, 20, 32, 44, 39, 20, 28, 26]
% np.mean(recvSum)=29.666666666666668 np.std(recvSum)=8.16496580927726 sps.sem(recvSum)=2.886751345948129
% send counter N ========================================================
% [[ 0  0  0]
%  [38 52 38]
%  [42 52 44]]
% send counter S ========================================================
% [[54 44 56]
%  [44 30 44]
%  [ 0  0  0]]
% send counter E ========================================================
% [[28 38  0]
%  [38 52  0]
%  [42 52  0]]
% send counter W ========================================================
% [[ 0 44 56]
%  [ 0 30 44]
%  [ 0 30 38]]
% send counter sum =====================================================
% [82, 126, 112, 120, 164, 126, 84, 134, 82]
% np.mean(sendSum)=114.44444444444444 np.std(sendSum)=26.192073063391234 sps.sem(sendSum)=9.260296238228726
% tscControl values ====================================================
% [30064968187, 30064968187, 30064968187, 30064968187, 30064968187, 30064968187, 30064968187, 30064968187, 30064968187]
% tscStart values ======================================================
% [1131, 1130, 1644, 1641, 628, 1650, 2151, 2155, 2149]
% tscEnd values ========================================================
% [709983, 736796, 714836, 730020, 721384, 731436, 713213, 730922, 713242]
% tsc diffs ============================================================
% --------------------------------------------------------------- ticks
% [708852, 735666, 713192, 728379, 720756, 729786, 711062, 728767, 711093]
% np.mean(tsc_ticks)=720839.2222222222 np.std(tsc_ticks)=9500.522988853212 sps.sem(tsc_ticks)=3358.9421151183965
% -------------------------------------------------------------- seconds
% [0.0008339435294117647, 0.0008654894117647059, 0.0008390494117647059, 0.0008569164705882353, 0.0008479482352941177, 0.0008585717647058823, 0.0008365435294117647, 0.0008573729411764705, 0.00083658]
% np.mean(tsc_sec)=0.0008480461437908496 np.std(tsc_sec)=1.1177085869239065e-05 sps.sem(tsc_sec)=3.9516966060216395e-06
% ---------------------------------------------------- seconds per cycle
% [2.0848588235294117e-05, 2.1637235294117648e-05, 2.097623529411765e-05, 2.1422911764705883e-05, 2.119870588235294e-05, 2.1464294117647056e-05, 2.0913588235294118e-05, 2.1434323529411762e-05, 2.0914499999999998e-05]
% np.mean(tsc_cysec)=2.1201153594771243e-05 np.std(tsc_cysec)=2.7942714673097676e-07 sps.sem(tsc_cysec)=9.879241515054106e-08
% ---------------------------------------------------------- cycle hertz
% [47964.878423140515, 46216.62547949749, 47672.99689284232, 46678.995413102246, 47172.6908967806, 46589.00006303218, 47815.80227884488, 46654.14323096409, 47813.71775562409]
% np.mean(tsc_cyhz)=47175.427825980936 np.std(tsc_cyhz)=620.9035009060691 sps.sem(tsc_cyhz)=219.52253797657457
% --------------------------------------------------------- ns per cycle
% [20848.58823529412, 21637.235294117647, 20976.23529411765, 21422.91176470588, 21198.70588235294, 21464.294117647056, 20913.58823529412, 21434.323529411762, 20914.499999999996]
% np.mean(tsc_cyns)=21201.15359477124 np.std(tsc_cyns)=279.42714673097595 sps.sem(tsc_cyns)=98.79241515054076
% fitness =============================================================
% [[0. 0. 0.]
%  [0. 0. 0.]
%  [0. 0. 0.]]

\subsection{Clade Reconstruction Trial}

% We performed extensive tests to be confident in our implementation of phylogenetic tracking for the Cerebras Software Language on the WSE device.
% Extensive other work CITE has validated the underlying hereditary surface algorithm and the reconstruction algorithm.
% We also used extensive unit tests in CSL to ensure the algorithm was working as expected.

Here, we demonstrate phylogenetic reconstructions from emulated WSE hardware and inspect clade structure to qualitatively assess their credibility.
% report the results of an integration test to assess the general validity of .
For these experiments, we tagged genomes with a 16-bit randomly generated identifier at simulation startup, as shown in Supplementary Figure \ref{fig:genome-layout} \citep{moreno2024supplement}.
% These identifiers identified clades descending from each founding genome.
Using the hardware emulator, we instantiated populations over a $3\times3$ PE collective for durations of 25, 50, 100, and 250 generation-cycles under drift conditions.
At the end of simulation, phylogenetic reconstruction was conducted using one genome sampled per PE.

\input{fig/tagged.tex}

Figure \ref{fig:tagged} shows reconstructed phylogenies from each duration.
As expected, taxa belonging to the same founding clade (shown by color) are reconstructed as more closely related to each other than to other taxa.
Additionally, and also as expected, the number of distinct remaining founding clades diminishes monotonically with increasing simulation duration.
These consistencies corroborate the general integrity of implemented annotation and reconstruction processes.
Note, however, the incidence of moderate overestimations for relatedness between independently-tagged clades throughout.
As mentioned earlier, and discussed in greater depth elsewhere \citep{moreno2024guide}, this is an expected artifact of hereditary stratigraphy with single-bit differentia.
Applications requiring greater reconstruction precision can opt for larger differentia sizes and/or higher differentia counts.

% Figure \ref{fig:validation-example:phylogeny} shows the result of phylogenetic reconstruction on these sampled genomes.
% To simplify visualization of the phylogeny with existing phyloinformatic tools, all clades were stitched together into a single tree by attaching them to a common ancestor.
% Taxa are colored according to their clade genesis tag.
% Clade arrangement in the reconstructed tree agrees well with founding clade identities.
% All different-colored taxa are predicted to have had ancient common ancestry.

\subsection{On-hardware Trial}

\input{fig/on-device}

Finally, we set out to assess the performance of our pipeline at full wafer scale.
For these experiments, we the used the four word, tracking-enabled genome layout, with the full first 32 bits containing a floating point fitness value.
We defined two treatments: \textit{purifying-only}, where 33\% of agent replication events decreased fitness by a normally-distributed amount,  and \textit{adaption-enabled}, which added beneficial mutations that increased fitness by a normally-distributed amount, occuring with 0.3\% probability.
These beneficial mutations introduced the possiblity for selective sweeps.
As before, we used tournament size 5 for both treatments.
We performed four on-hardware replicates of each treatment instantiated on 10k ($100\times100$), 250k ($500\times500$) and 562.5k ($750\times750$) PE arrays.
We halted each PE after it elapsed 1 million generations.
Perfmance metrics for these runs are described in the preceding section.

Upon completion, we sampled one genome from each PE.
Then, we performed an agglomerative trie-based reconstruction from subsamples of 10k end-state genomes \citep{moreno2024analysis}.
Figure \ref{fig:on-device} compares phylogenies generated under the purifying-only and adaption-enabled treatments.
As expected \citep{moreno2023toward}, purifying-only treatment phylogenies consistently exhibited greater sum branch length and mean evolutionary distinctiveness, with the effect on branch length particularly strong.
These structural effects are apparent in example phylogeny trees from 562.5k PE trials (Figures \labelcref{fig:on-device-adaptive,fig:on-device-purifying}).
Successful differentiation between treatments is a highly promising outcome.
This result not only supports the correctness of our methods and implementation, but also confirms capability for reconstruction-based analyses to extract meaningful information describing dynamics of very large-scale evolution simulations.
% We look forward to future work expand the repetoire of  \citep{moreno2023toward}, which


==> binder-wafer-scale/tex/text/frontmatter.tex <==
\title{ Trackable Agent-based Evolution Models at Wafer Scale}

\author[1,2,3,*]{Matthew Andres Moreno\orcidlink{0000-0003-4726-4479}}
\author[4]{Connor Yang\orcidlink{0009-0004-1240-2362}}
\author[5,6]{Emily Dolson\orcidlink{0000-0001-8616-4898}}
\author[1,2]{Luis Zaman\orcidlink{0000-0001-6838-7385}}

\affil[.  ]{\vspace{-4.4ex}}
\affil[1]{Department of Ecology and Evolutionary Biology, University of Michigan, Ann Arbor, United States}
\affil[2]{Center for the Study of Complex Systems, University of Michigan, Ann Arbor, United States}
\affil[3]{Michigan Institute for Data Science, University of Michigan, Ann Arbor, United States}
\affil[4]{Undergraduate Research Opportunities Program, University of Michigan, Ann Arbor, United States}
\affil[5]{Department of Computer Science and Engineering, Michigan State University, East Lansing, United States}
\affil[6]{Program in Ecology, Evolution, and Behavior, Michigan State University, East Lansing, United States}
\affil[*]{corresponding author: \textit{morenoma@umich.edu}}

\maketitle


==> binder-wafer-scale/tex/text/references.tex <==
\putbib


==> binder-wse-sketches/tex-access-proposal/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> binder-wse-sketches/tex-access-proposal/fig/async-ga-schematic.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\includegraphics[width=\linewidth]{img/async-ga-schematic.pdf}
\centering
\caption{Schematic overview of asynchronous island model evolutionary algorithm.}
\label{fig:async-ga-schematic}
\end{wrapfigure}


==> binder-wse-sketches/tex-access-proposal/fig/hsurf-schematic.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\includegraphics[width=\linewidth]{img/hsurf-schematic.pdf}
\centering
\caption{Panel A shows update sequence on a four-site HStrat curation space-time memory under steady policy. Panel B contrasts steady policy with tilted policy, which prioritizes recent data.}
\label{fig:hsurf-schematic}
\end{wrapfigure}


==> binder-wse-sketches/tex-access-proposal/fig/runtime-posthoc-schematic.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\includegraphics[width=\linewidth]{img/runtime-posthoc-schematic.pdf}
\caption{Proposed agent-based evolutionary simulation and observation framework, using HStrat markers to estimate phylogenetic history, thereby, infer evolutionary dynamics.}
\label{fig:runtime-posthoc-schematic}
\end{wrapfigure}


==> binder-wse-sketches/tex-access-proposal/fig/validation-example.tex <==
\begin{figure}[htbp]
    \centering

    % Top panel for the image
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{binder/binder/teeplots/genome=hsurftiltedsticky_tagged+viz=draw-biopython-tree+ext=}
        \caption{%
          Reconstructed phylogeny, generated under the assumption of shared ancestry.
          Hexidecimal codes in taxon names are fixed random markers generated at simulation start-up, indicating independent lineage originations.
          Color coding indicates clades with independent lineage originations.
          As expected, low relatedness is predicted for taxa originating from independent lineages.
        } \label{fig:validation-example:phylogeny}
    \end{subfigure}

    % Space between image and table
    \vspace{10pt}

    % Bottom panel for the table
    \begin{subfigure}[b]{\textwidth}

\begin{minipage}[t]{\textwidth}
\centering
\footnotesize
\begin{tabular}{
c
>{\columncolor{LighterBlue}}c
>{\columncolor{LighterBlue}}c
>{\columncolor{LighterSalmon}}c
>{\columncolor{LighterSalmon}}c
q % Thick divider
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
q % Thick divider
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
}
& \multicolumn{4}{cq}{\cellcolor{white}Word 0} & \multicolumn{4}{cq}{\cellcolor{white}Word 1} & \multicolumn{4}{c}{\cellcolor{white}Word 2} \\
\cmidrule(l{1.5pt}r{1.5pt}){2-5}
\cmidrule(l{1.5pt}r{1.5pt}){6-9}
\cmidrule(l{1.5pt}r{1.5pt}){10-13}
Byte & {\cellcolor{white}0} & {\cellcolor{white}1} & {\cellcolor{white}2} & {\cellcolor{white}3} & {\cellcolor{white}4} & {\cellcolor{white}5} & {\cellcolor{white}6} & {\cellcolor{white}7} & {\cellcolor{white}8} & {\cellcolor{white}9} & {\cellcolor{white}10} & {\cellcolor{white}11} \\
\cmidrule(l{1.5pt}r{1.5pt}){2-2}
\cmidrule(l{1.5pt}r{1.5pt}){3-3}
\cmidrule(l{1.5pt}r{1.5pt}){4-4}
\cmidrule(l{1.5pt}r{1.5pt}){5-5}
\cmidrule(l{1.5pt}r{1.5pt}){6-6}
\cmidrule(l{1.5pt}r{1.5pt}){7-7}
\cmidrule(l{1.5pt}r{1.5pt}){8-8}
\cmidrule(l{1.5pt}r{1.5pt}){9-9}
\cmidrule(l{1.5pt}r{1.5pt}){10-10}
\cmidrule(l{1.5pt}r{1.5pt}){11-11}
\cmidrule(l{1.5pt}r{1.5pt}){12-12}
\cmidrule(l{1.5pt}r{1.5pt}){13-13}
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 0} & \texttt{F9} & \texttt{02} & \texttt{79} & \texttt{00} & \texttt{8D} & \texttt{22} & \texttt{4F} & \texttt{F3} & \texttt{D2} & \texttt{78} & \texttt{AD} & \texttt{C7} \\
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 1} & \texttt{F9} & \texttt{02} & \texttt{75} & \texttt{00} & \texttt{8D} & \texttt{A1} & \texttt{CB} & \texttt{F2} & \texttt{D1} & \texttt{5B} & \texttt{CC} & \texttt{D4} \\
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 2} & \texttt{61} & \texttt{B6} & \texttt{65} & \texttt{00} & \texttt{66} & \texttt{29} & \texttt{B4} & \texttt{F0} & \texttt{62} & \texttt{99} & \texttt{5A} & \texttt{61} \\
{\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} &
{\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} \\
\end{tabular}
\end{minipage}


        \caption{%
          Example genomes sampled after simulation completion.
          In validation testing, genomes were composed of three 32-bit words.
          The first two bytes (blue) are fixed random markers generated at simulation start-up, indicating independent lineage originations.
          The next two bytes (salmon) are a generation counter.
          Bits within the final eight bytes are lineage checkpoint values to facilitate phylogenetic reconstruction, arranged according to a tilted hereditary stratigraphic algorithm.
          Note that this genome does not include any content affecting agent traits or fitness --- neutral selection was used for this validation experiment.
        } \label{fig:validation-example:genomes}
    \end{subfigure}

    \caption{
      Synopsis of preliminary experiment used to validate Cerebras Software Language implementation of asynchronous agent-based evolution framework and hereditary stratigraphy algorithms.
      Experiments were performed on Cerebras SDK hardware simulator.
      Subfigure \ref{fig:validation-example:phylogeny} shows an example reconstructed phylogeny from genomes tagged with fixed random identifiers that identify independent lineage originations.
      Subfigure \ref{fig:validation-example:genomes} overviews layout of fixed-size genomes used for validation testing and shows example end-state genomes corresponding to phylogeny taxa.
    }
    \label{fig:validation-example}
\end{figure}


==> binder-wse-sketches/tex-access-proposal/lib/dependencies.tex <==
\usepackage{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{authblk}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{csquotes}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{import}
\usepackage{natbib}
% \usepackage[moderate]{savetrees}
\usepackage{enumitem}
\setlist{nosep,topsep=-\parskip,noitemsep}
\usepackage{siunitx}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{wrapfig}
\usepackage{xcolor}

% Define lighter colors
\definecolor{LighterBlue}{rgb}{0.84, 0.92, 0.95}
\definecolor{LighterSalmon}{rgb}{1.0, 0.81, 0.76}
\definecolor{LighterPastelGreenYellow}{rgb}{0.88, 0.96, 0.90}

% Define thick vertical lines for section dividers
\newcolumntype{q}{!{\color{white} \vrule width 2pt}}

\setlength\parindent{24pt}
\captionsetup{font=small}
\setlength{\bibsep}{0pt plus 0.3ex}

\usepackage{ragged2e}
\setlength{\RaggedRightParindent}{\parindent}

==> binder-wse-sketches/tex-access-proposal/lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> binder-wse-sketches/tex-access-proposal/lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
asdf
}


==> binder-wse-sketches/tex-access-proposal/lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> binder-wse-sketches/tex-access-proposal/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> binder-wse-sketches/tex-access-proposal/lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> binder-wse-sketches/tex-access-proposal/lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> binder-wse-sketches/tex-access-proposal/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> binder-wse-sketches/tex-access-proposal/text/body.tex <==
% \input{text/body/abstract.tex}

\input{text/body/introduction.tex}

\input{text/body/objectives.tex}

\input{text/body/methods.tex}

\input{text/body/preliminary-work.tex}

\input{text/body/conclusion.tex}

\input{text/body/key-considerations.tex}

==> binder-wse-sketches/tex-access-proposal/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

Proposed work lays the foundations to harness wafer-scale computing for agent-based modeling.
Orders-of-magnitude scale-up will bring entirely new classes of cross-scale dynamics within reach across many ABM application areas.
To advance on this front, we explore a fundamental re-frame of simulation that shifts from a paradigm of complete, perfect data observability to dynamic, approximate observability akin to estimation approaches traditionally used to study physical systems.

Within ABM, our proposed work focuses in particular on the topic of evolutionary computation.
We will harness cutting-edge \textit{hereditary stratigraphy} (HStrat) approaches to distributed phylogenetic tracking to investigate fundamental questions about the relationship between phylogenetic structure, population scale, and time scale.
These new HStrat methods, and extensive development targeting the Cerebras CSL using the SDK hardware simulator, position our project to hit the ground running.
Our project design emphasizes concrete steps to demonstrate and evaluate novel algorithms to establish strong technical foundations for follow-on work with distributed agent-based digital evolution.
We are committed to organizing project implementation to produce reusable CSL and Python software tools to catalyze research capabilities among the broader ABM community.

Potential extensions of this work include repurposing HStrat's rolling cross-temporal sampling algorithms to facilitate efficient downsampled observability in additional application domains.
Possibilities include sampling time series activity at simulation sites or extracting coarsened agent histories (e.g., position over time).
Within the domain of evolution modeling, we anticipate building from the work proposed here to conduct cross-scale evo-epidemiological research into how pathogen trait evolution confronts fitness trade-offs related to within-host infection dynamics and between-host transmissibility.


==> binder-wse-sketches/tex-access-proposal/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

Agent-Based Modeling (ABM) has gained increasing adoption as a method to answer basic science questions and inform policy decisions.
Despite a wide berth of application domains --- spanning sectors like transportation infrastructure, public health, telecommunications, materials science and more --- much ABM work is unified by a common theme of interest in cross-scale dynamics.
To provide such insight, ABM requires sufficient scale to capture systems' emergent behaviors.
Advances in high-performance computing (HPC) have already yielded paradigm-shifting improvements to the capabilities of ABM.
However, across domains key questions remain out of computational reach.

\input{fig/runtime-posthoc-schematic.tex}
Significant untapped potential for ABM scale-up has been identified in hardware-accelerator-enabled computation.
Rapid advances in the capability of accelerator devices, driven in particular by market demand for deep learning operations, are anticipated to play a key role in future advances in ABM capabilities \citep{perumalla2022computer}.
Within this category, the emerging class of fabric-based accelerators, most notably the recently-introduced 850,000 core Cerebras CS-2 Wafer Scale Engine (WSE) \citep{lauterbach2021path,lie2022cerebras}, is a particularly exciting --- and fairly uncharted, with applications to HPC workloads still in early days.
This paradigm interfaces multitudinous processor elements (PEs) in a physical lattice, with PEs executing independently using individual on-chip memory and local PEs interacting through a network-like interface.

\subsection{Objectives}

This proposal establishes foundations for next-generation accelerator-enabled ABM computation by decentralized, approximate data export from agent-based evolutionary simulation.
In particular, we will evaluate asynchronous approaches for ABM migration/interaction on the WSE architecture to power agent-based evolution simulations, incorporating cutting-edge methods for distributed approximate phylogenetic (i.e., ancestry tree) tracking.

Proposed work advances two technical objectives:
\begin{enumerate}
\item to evaluate and demonstrate new approaches for phylogenetic tracking in a massively-distributed, resource-constrained setting,
\item to test the scalability of desynchronized agent migration procedures on WSE hardware,
\end{enumerate}

These technical capabilities will unlock capability to investigate a broad array of science questions.
In this proposal, we focus on one science objective:
\begin{enumerate}
\item to evaluate how phylogenetic structure scales across orders-of-magnitude population sizes, and the extent to which commonly used phylogeny structure metrics are scale-invariant or scale-sensitive.
\end{enumerate}

% Proposed work falls within the domain of agent-based evolution modeling, and uses it to  phylogenetics-related inquiry by leveraging Cerebras WSE hardware.
Our dual technical objectives constitute significant advancement of methodological capabilities within agent-based digital evolution, and our project will directly address fundamental open questions within the domain of phylogenetic theory.
However, findings and methodologies will also generalize to other ABM domains beyond evolutionary simulation and to broader classes of highly distributed HPC architectures.

\subsection{Agent-based Evolution Simulation}

Evolutionary processes are not confined to matters of natural history.
Rather, evolutionary processes pervade our contemporary, everyday world.
Key societal challenges stem from evolving systems: antibiotic resistance, epidemiology, conservation biology, and oncology among others.  % citations?
Evolutionary biology provides the fundamental foothold to efforts to address these problems \citep{aktipis2013evolutionary}.

Mathematical and computational modeling complements natural history field work and benchtop evolution experiments as a crucial third leg to stand evolutionary inquiry.
Simulation-based approaches provide key capabilities complementary to work with natural systems: complete observability, arbitrary manipulability, and rapid generational turnover.
Within this context, agent-based simulation plays an important connective role between natural systems and abstracted, aggregate-based mathematical and numerical models.
Agent-based approaches instantiate \textit{bona fide} evolutionary processes that track populations of virtual genomes subject to mutation, heredity, and selection \citep{pennock2007models}.
This characteristic incorporates some of the critical complications and subtleties characteristic of natural systems --- e.g., arbitrary agent behavior, sophisticated agent-agent interactions, and complex genotype-phenotype maps, albeit at significantly reduced scope and sophistication.

Indeed, agent-based evolution approaches have provided means for fruitful investigation of wide-ranging hypotheses, including evolution of evolvability \citep{wilke2001evolution}, host-parasite co-evolution \citep{zaman2014coevolution}, evolution of complex traits \citep{lenski2003evolutionary}.

Ambitious work advancing the field increasingly targets large cross-scale questions, including major transitions in evolution (e.g., multicellularity and symbiosis) \citep{goldsby2020major,vostinar2021symbiosis} and open-ended evolution (e.g., long-term trajectories of complex ecosystems with strong biotic selection) \citep{stanley2019open,taylor2016open}.
Progress on these fronts demands computational substrate for orders-of-magnitude larger simulation scale than tractable today \citep{moreno2022exploring,channon2019maximum}.

%as well as scenarios where replicating entities like cultural artifacts or computer viruses.
% At the frontiers of evolutionary computation, there is in particular growing interest in the question of ``open-ended evolution'' \citep{}.
% This refers to the problem of the inability to recreate the ongoing generation of novelty, complexity, and adaptation within the natural world.

\subsection{HPC and Agent-based Evolution}
% opportunity


% Evolutionary questions often explicitly span scopes, with key areas of inquiry including ecologies of interacting populations and assembly of individuals into multicellular organisms and eusocial colonies \citep{morenoDISHTINYTODO, citephageTODO}.
Researchers using agent-based evolution recognize HPC as critical to the future of the field \citep{ackley2016indefinite}.
Indeed, the field has played host to notable boundary-pushing approaches to computing at the frontiers of computing hardware and modalities such as best-effort computing, reservoir computing, global-scale time-available computing, and modular tile-based computing in addition to more traditional cluster and GPU-oriented approaches \citep{moreno2021conduit,ackley2020best,ackley2023robust,heinemann2008artificial,miikkulainen2024evolving}.

The diversity of HPC strategies for evolutionary simulation stems in large part from unique properties largely distinct from other HPC application domains.
Given its inherent underlying stochastic nature and the stabilizing influence of adaptive selection, evolutionary simulation can often tolerate significant arbitrary asynchronicity or even entirely lost simulation components (e.g., dropped messages, crashed nodes, etc.).
Likewise, digital evolution is typically amenable to locality restrictions of computation due to the inherent spatial structure of natural systems we are seeking to model.
% In particular, massively-distributed, spatial computing being directly highlighted to be of particular interest \citep{ackleyTODO}.
Because agent behavior evolves over time, the influence of population-level drift and adaptive change can inject extreme heterogeneity into the computational workload profile of evolutionary simulation over time and simulation space.
Finally, emerging research questions have introduced challenging communication-intensive requirements to support rich interactions between evolving agents.
The largely decoupled nature of classic approaches within evolutionary computation like island models or controller/worker schemes  \citep{bennett1999building,cantu2001master} no longer suffice to realize the dynamic, communication-intensive interaction characteristic of major transitions in individuality (e.g., multicellularity) and ecological communities \citep{moreno2022engineering}.

These distinctive workload properties position agent-based evolution as a potentially valuable testbed for HPC innovation and leadership.
% There is reason to expect a highly synergistic, reciprocal relationship between digital evolution and the broader HPC enterprise.
Work proposed here steps in this direction, seeking to blaze new territory that opens new possibilities to benefit broader constituencies of ABM/HPC practitioners.

However, despite the strong motivation for large-scale simulation, the algorithmic pliability of evolutionary simulation, and the increasing availability of highly capable parallel, distributed, and accelerator-driven hardware platforms, significant methodological limitations currently hold back scale-up of digital evolution.
Work proposed here takes significant steps to position the agent-based evolution simulations to benefit significantly from this emerging class of hardware accelerators.

\subsection{Phylogenetic Tracking Methods}

To serve as a useful experimental platform, digital evolution simulations must be observable.
In addition to end-state information (i.e., evolved traits), scientific questions demand information sufficient to characterize the underlying mode and tempo of evolution.
Additionally, it is often useful to be able to trace the history of notable evolutionary events (e.g., extinctions, evolutionary innovations)
Observability counts, too, in application-oriented aspects of evolutionary computation, where such data serves as a critical diagnostic to tune configuration for good performance \citep{hernandez2022can}.

In evolutionary biology, phylogenetic history is a valuable tool for triangulating the context of notable evolutionary events, as well as characterizing the underlying mode and tempo of evolution.
The same holds true in evolutionary simulation.
% https://github.com/mmore500/phylotrack-algorithm-analysis/blob/fe16d2b2d7df99faade09c01b72f681160749f51/tex/text/body/introduction.tex
In addition to addressing questions of natural history, access to the phylogenetic record of biological life has proven informative to conservation biology, epidemiology, medicine, and biochemistry among other domains \citep{faithConservationEvaluationPhylogenetic1992, STAMATAKIS2005phylogenetics, frenchHostPhylogenyShapes2023,kim2006discovery}.
Nonetheless, existing analyses of phylogenetic structure within digital systems have already proven valuable, enabling diagnosis of underlying evolutionary dynamics \citep{moreno2023toward,hernandez2022can,shahbandegan2022untangling, lewinsohnStatedependentEvolutionaryModels2023a} and even serving as mechanism to guide evolution in application-oriented domains \citep{lalejini2024phylogeny,lalejini2024runtime,murphy2008simple,burke2003increased}.
Further, comparison of observed phylogenies against simulation phylogenies can be used to evaluate hypotheses for underlying dynamics within real-life evolutionary/epidemiological systems \citep{giardina2017inference,voznica2022deep}.

Unfortunately, existing approaches to recording phylogenetic history from digital evolution simulations do not scale robustly.
Simulation phylogenies have typically been collected using a centralized record-keeping approach where every reproduction event is stitched together in a tree data structure to produce a complete record.
Record-keeping often involves pruning the records of extinct lineages to prevent memory bloat \citep{dolson2023phylotrack}.
Although the direct-tracking approach is well suited to serial simulation substantial limitations and runtime overhead make scaling this up to highly parallel/distributed systems --- particularly those with low memory capacity like the Cerebras WSE --- essentially untenable \citep{moreno2024analysis}.

To overcome this limitation to phylogenetic analysis within many-processor HPC contexts, we have proposed a new class of reconstruction-based approaches to phylogenetic tracking in silico \citep{moreno2022hereditary}.
These approaches require no centralized data collection during simulation runtime; instead, they use post hoc comparisons between end-state agent genomes to deduce approximate phylogenetic history --- akin to how DNA-based analyses tell how lineages of contemporary organisms relate in natural history.
Figure \ref{fig:runtime-posthoc-schematic} depicts our reconstruction-based strategy.

To achieve efficient, tractable phylogenetic reconstructions in practice, some careful consideration is required.
DNA-based is notoriously data-hungry, typically requiring on the order of thousands of genome sites, and can be significantly biased by physical/functional traits of the underlying genetic information.
These concerns motivated our recent development of HStrat, a genetic architecture explicitly designed for fast, accurate reconstruction requiring only small amounts of data.
HStrat data is designed to be attached to the underlying genomes within particular digital evolution systems as a neutral annotation.
Benchmarking experiments to evaluate HStrat performance have achieved high-quality reconstruction of phylogenetic histories for tens of thousands of fully distributed agents using just 96 bits of tracking information per agent genome.
Details on this methodology and our proposed approach to translate it to the WSE context are provided in Section \ref{sec:methods}.

% \subsection{Outline}

% The remainder of this proposal is structured as follows
% \begin{itemize}
% \item Section \ref{sec:objectives} describes proposed work,
% \item Section \ref{sec:methods} overviews proposed methods,
% \item Section \ref{sec:preliminary-work} reviews established work on this project,
% \item Section \ref{sec:conclusion} provides concluding remarks, and
% \item Section \ref{sec:key-considerations} recaps key technical considerations highlighted in the program solicitation.
% \end{itemize}


==> binder-wse-sketches/tex-access-proposal/text/body/key-considerations.tex <==
\section{Key Considerations} \label{sec:key-considerations}

\begin{enumerate} \itshape \bfseries
\item %
% Using the SDK requires programming in CSL, a C-like language designed specifically for the problem of massively parallel programming on the CS-2.
What is your experience with HPC programming paradigms and languages, such as MPI, OpenMP, CUDA, OpenCL, etc.?
\end{enumerate}
\noindent
Dr. Moreno has extensive experience working with HPC technologies, most notably developing asynchronous, best-effort computing approaches using MPI and C++.
He has also received training in GPU programming (e.g., OpenCL, CUDA).
Dr. Dolson and Dr. Zaman are both experienced systems-level programmers.

\begin{enumerate}[resume] \itshape \bfseries
\item What are the underlying computational algorithms you're interested in exploring?
What existing software packages or libraries use these algorithms?
\end{enumerate}
\noindent
The core algorithm is an island-style GA, which is well-supported by digital evolution frameworks targeting serial processing on traditional HPC hardware \citep{bohm2017mabe}.
Those that support parallelism generally apply a centralized coordinator-worker strategy \citep{fortin2012deap}, which is best suited to small population sizes with expensive fitness evaluations.

\begin{enumerate}[resume] \itshape \bfseries
\item How is this problem bottlenecked on current hardware?
% Is the problem more bottlenecked by memory bandwidth, or communication costs associated with scaling up across distributed compute nodes?
\end{enumerate}
\noindent
Memory bandwidth and synchronization costs to exchange population members.
Compute bound memory latency.

\begin{enumerate}[resume] \itshape \bfseries
\item What range of problem sizes are you interested in addressing?
% For example, how much memory does your problem use?
How does memory usage or program run-time scale with problem size?
\end{enumerate}
\noindent
We are interested in developing population-scale, cross-scale simulations with hundreds of millions of agents.
The memory usage of the program and run-time scale linearly with problem size, either defined as evolutionary duration or population size.
Precise memory usage depends largely on the agent genomes used.
For smaller agent genomes, sized on the order of four words, thousands of agents could be supported per PE --- yielding a net whole-wafer population size on the order of a billion agents.

\begin{enumerate}[resume] \itshape \bfseries
\item What portion of your algorithm do you plan to port to the CS-2?
% Why are you interested in exploring this part of your algorithm?
\end{enumerate}
\noindent
We plan to port the core evolutionary generational loop to the CS-2 as an island model-style genetic algorithm.
The stages are 1) migration, 2) selection, 3) replication with mutation.
We are interested in porting it because it is the most computationally intensive to scale and because it is embarrassingly parallel.
Postprocessing to analyze evolved traits, and reconstruct evolutionary history will take place off-device.

\begin{enumerate}[resume] \itshape \bfseries
\item %
% The CS-2 offers native half and single precision data types.
What precision does your algorithm or use case need?
\end{enumerate}
\noindent
Due to the agent-based modeling, this is a primarily discrete domain.
However, floating point types may be used to represent traits.
Because they are only used for comparisons between agents, single or half precision suffice.

\begin{enumerate}[resume] \itshape \bfseries
\item %
% The CS-2 is a network-attached accelerator. 
% At a high level, the CSL programming model is similar to that of CUDA, in which data is moved between host CPU nodes and the device (CS-2) on which computational kernels are launched.
How often will data need to be moved between the wafer and the worker nodes?
\end{enumerate}
\noindent
For preliminary versions of the project, we are planning to only collect data at the end of execution through the Cerebras memcpy infrastructure.
As the model is self-contained, no data except for the PE code will need to be moved onto the device.
In the future, we are interested in exploring samples throughout the evolutionary process to serve as a kind of ``fossil record.''

\begin{enumerate}[resume] \itshape \bfseries
\item Describe your general plan to map your problem onto 850,000 cores. 
% In answering this question, it might be helpful to recall some details of the CS-2 architecture.
% The 850,000 cores are laid out in a mesh, with each core connected on fabric to its four nearest neighbors on the East, South, North, and West.
% Memory is distributed among the cores, with each core having 48 KB of local memory.
% 64-bit local memory reads and writes take roughly a cycle, as does sending and receiving 32-bit messages between the four neighboring cores.
\end{enumerate}
\noindent
We plan to exploit an island model genetic algorithm where each PE is an island and genomes migrate between adjacent islands.
As natural systems are typically asynchronous, synchronization is not a concern.
We plan to use CSL asynchronous send/receive operations to implement migration.

Genomes will be represented as contiguous buffers of u32 and each PE's population as a contiguous buffer of genome data using a simple synchronous generational model (i.e., a swap buffer.)
Population-level operations (e.g., selection, reproduction, mutation) will take advantage of the CSL's data structure descriptors.
The local memory is sufficient for a population size on the order of hundreds or low thousands.
This could give a global population size on the order of hundreds of millions.


==> binder-wse-sketches/tex-access-proposal/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

In this section, we describe the primary two algorithmic components for our on-device simulation:
\begin{enumerate}
\item the asynchronous compute-communicate cycle used to instantiate an island model evolutionary process across the WSE engine, and
\item the lightweight hereditary stratigraphy element used to annotate virtual genomes and facilitate robust \textit{post hoc} phylogenetic reconstruction.
\end{enumerate}

\subsection{Asynchronous Island-model Evolutionary Computation}

\input{fig/async-ga-schematic.tex}
We apply an island-model genetic algorithm to instantiate an evolutionary process spanning PEs.
Island-model approaches are common in applications of parallel and distributed computing to evolutionary computation \citep{bennett1999building}.
Under this model, each processor element (PE) hosts an independent population.
Migration between PEs stitches island populations together into a common gene pool.

Core kernel activity proceeds via an update cycle performed on each PE, which comprises several steps.
Figure \ref{fig:async-ga-schematic} provides a schematic overview.

The first step of this update loop is to handle migration, depicted as blue-red arrows in Figure \ref{fig:async-ga-schematic}.
We adopt a fully asynchronous approach to migration between neighboring PEs.
Evolutionary processes tend to occur asynchronously with arbitrary factors influencing things, so this is a reasonable relaxation to make.

Each PE maintains independent immigration buffers and emigration buffers dedicated to each cardinal neighbor, depicted in blue and red, respectively, in Figure \ref{fig:async-ga-schematic}.
On simulation startup, an asynchronous DSD receive operation is opened to accept genomes from neighboring PEs into the appropriate immigration buffer.
At startup, additionally, the emigration buffer is populated with one or more genomes copied from the population.
Then, an asynchronous send request is opened to dispatch wavelets containing genome data from the emigration buffer to the neighbor.
Both operations register an on-completion callback to set a ``send complete'' or ``receive complete'' flag variable associated with their corresponding buffer.

In each update cycle, the main update loop tests all ``send complete'' and ``receive complete'' flags.
For each immigration flag that is set, corresponding received genomes are written into the main population buffer, replacing randomly chosen population members.
Then, the flag is reset a new receive request is initiated.
Likewise, for each emigration flag set, corresponding send buffers are re-populated with randomly sampled genomes from the main population buffer.
Corresponding flags are then reset and new send requests are initiated.
The bottom right corner of Figure \ref{fig:async-ga-schematic} summarizes this process.

The remainder of the main update loop handles evolutionary operations within the scope of the executing PE.
Each genome within the population is evaluated to produce a floating point fitness value.
Modular implementation ensures evaluation criteria can be chosen appropriately for underlying experimental objectives.
For the purposes of this project, we will use a trivial fitness function that explicitly models additive accumulation of beneficial/deleterious mutations as a floating point value within each genome.

After evaluation, tournament selection is applied.
Each slot in the next generation is populated with a genome exhibiting maximal fitness among $n$ randomly sampled individuals, ties broken randomly.

Finally, a mutational operator is applied across all genomes in the next population.
As with evaluation criteria, a modular implementation allows mutation operations to be defined based on experimental objectives.
Here, we use a simple Gaussian mutation on each genome's stored fitness value.
At this point, hereditary stratigraphy annotations --- discussed next --- are updated to reflect an elapsed generation.

The process then repeats, with a self-activating wavelet dispatched to execute the next cycle of the main update loop.

Kernel source code implementing described procedures can be viewed at \url{https://hopth.ru/cl}.
Our implementation is defined modularly with respect to genome size, layout, mutational operator, and fitness evaluation criteria, allowing for direct re-use of produced software for follow-on evolution experiments on WSE hardware.

% A key question will be the extent to which intentionally desynchronizing affects performance, stability, and computation quality.

\subsection{Distributed Phylogenetic Tracking}

Our approach to the analysis of evolutionary history for wafer-scale simulation draws inspiration from the inference-based paradigm used to characterize history in natural systems.
This approach is fully distributed, with ancestry information contained within genomes themselves rather than in any external tracking mechanism.
Just as mutational drift encodes ancestry information in DNA genomes, the inference-based paradigm requires only local updates to individual genomes at runtime as generations elapse.

Recent work introducing \textit{hereditary stratigraphy} (HStrat) methodology has explored how best to organize genetic material to maximize reconstruction quality and minimize memory footprint \citep{moreno2022hstrat, moreno2022hereditary}.
Proposed work bundles HStrat material with underlying agent genomes as an instrumentative ornament, entirely neutral with respect to agent traits or fitness.

The hereditary stratigraphy algorithm associates each generation along individual lineages with an identifying ``fingerprint'' value.
Each time a generation elapses, all offspring generate a new identifier value.
Within each offspring, generated identifiers append to an inherited running chronological record of fingerprint values.
To prevent $\mathcal{O}(n)$ space complexity as generations elapse, not all fingerprints can be kept.
Instead, excess fingerprints are pruned away according to a deterministic program that ensures retention of fingerprint values from checkpoint generations spaced across evolutionary history.

% \input{fig/hsurf-schematic.tex}

Limitations of the Cerebras WSE environment required significant elaboration of hereditary stratigraphy algorithms to minimize memory use, avoid complex data structures with dynamically allocated memory, and minimize iterative computation.
We use a constant-time indexing scheme that maps each lineage's fingerprint stream onto a fixed-width memory buffer such that eviction of existing fingerprint values by new placements maintains a temporally-representative sampling over elapsed time.
We call this approach ``surface''-based to distinguish it from earlier hereditary stratigraphy methods.
Time stamps can be positionally inferred and thus do not need to be stored --- a several-fold savings that enables fingerprint values to be shrunk down and packed together.
Single-bit checkpoints have been shown to produce good quality phylogenies using only 96 bits per genome \citep{moreno2023toward}.
The semantic structure of HStrat annotations streamlines \textit{post hoc} phylogenetic reconstruction, which essentially boils down to a simple trie-building procedure
\citep{moreno2024analysis}.


==> binder-wse-sketches/tex-access-proposal/text/body/objectives.tex <==
\section{Proposed Work} \label{sec:objectives}

Our project will unfold in three phases:
\begin{enumerate}
\item \textbf{Algorithm Validation}: compare replicate evolutionary runs across selection pressure levels, and evaluate capability of instrumentation and reconstruction pipeline to detect expected effects on phylogenetic structure in wafer-scale agent populations;
\item \textbf{Scalability Analysis}: assess stability, efficiency, and migration throughput of asynchronous agent exchange between PEs in collections ranging from hundreds of PEs, to thousands, to full wafer scale; and
\item \textbf{Phylogenetic Structure Across Population Scales}: exploit wafer scale computation to answer fundamental questions of how common phylogeny structure metrics vary with scale in time and space.
\end{enumerate}

Proposed work will provide a technical demonstration and evaluation of novel approaches that harness CS-2 capabilities for ABM, opening up an entirely new class of HPC applications for wafer-scale technology.
We will exploit this prototype software to answer foundational questions about how phylogenetic structure differs across orders-of-magnitude changes in population size.

\subsection{Algorithm Validation}

Initial work will augment existing software tests and hardware-simulation integration tests to prove the capability of newly developed genome annotations and phylogeny reconstruction processes to recover accurate, actionable depictions of evolutionary history.
We will generate experimental replicates across several levels of selection pressure by varying the tournament size in our island model genetic algorithm.
This property has well-defined expectations for effects on sum branch length in phylogenetic structure, allowing us to evaluate the capability of the developed genome instrumentation and tree reconstruction pipeline to recover expected effects from wafer-scale agent populations.

\subsection{Scalability Analysis}

To assess the scalability of asynchronous agent exchange between PEs within the Cerebras architecture, we will perform replicate benchmark experiments at collective sizes of 850k, 85k, 8.5k and 850 PEs.
At each scale, we will assess the following metrics:
\begin{itemize}
\item uniformity of cycle count across processor elements,
\item mean per-PE generational turnover rate, and
\item net migration per-PE per unit time.
\end{itemize}

\subsection{Phylogenetic Structure Across Population Scales}

We will apply the unique capabilities of WSE-enabled simulation to test the scaling properties of common phylogenetic structure metrics, including the Colless-like index, mean evolutionary distinctiveness, mean pairwise distance, and sum branch length \citep{tucker2017guide}.
% Several of these metrics are generally assumed to be perfectly or nearly scale invariant \citep{TODOaskemily}.
For metrics that explicitly scale with tree size (e.g., sum branch length) we will apply conventional normalization approaches.
Due to spatial structure introduced under the lattice island model, we expect to observe scale-dependence outcomes across metrics despite normalization.
However, the effect sign and size is difficult to predict \textit{a priori}, and will be the focus of our investigation.
Findings will strengthen foundational understanding of how evolutionary dynamics produce phylogenetic structure, especially due to the influence of two-dimensional spatial structure within many natural systems.
Strengthened theory will benefit applications in many sectors including ecology, natural history, and application-oriented evolutionary computation.

% We will collect under selection pressure and with small colletions of PEs and large collections of PEs
% Test for differences in phylogenetic structure metrics.
% (how to control for reconstruction quality?)
% Relatedly: are phylometrics time invariant to duration of simulation?
% Another objective: does streaming samples off the chip asynchronously bias phylometrics (as opposed to collecting everything all at the end.


==> binder-wse-sketches/tex-access-proposal/text/body/preliminary-work.tex <==
\section{Preliminary Work} \label{sec:preliminary-work}

In preparation for proposed work, we joined the Cerebras SDK program \citep{selig2022cerebras} and assembled Cerebras Software Language (CSL) software implementations that will be necessary to conduct experiments with WSE hardware.
For the time being, we have used Cerebras' hardware emulator to test our software implementations.
This section reports a small-scale experiment performed to validate the core software functionality.
In addition to this integration test, software quality has also been verified through an associated unit test suite.

\subsection{Validation Experiment}

% fab w,h = 10,5
% Kernel x,y w,h = 4,1 3,3
% memcpy x,y w,h = 1,1 8,3
% whoami ===============================================================
% [[0 3 6]
%  [1 4 7]
%  [2 5 8]]
% whereami x ===========================================================
% [[0 1 2]
%  [0 1 2]
%  [0 1 2]]
% whereami y ===========================================================
% [[0 0 0]
%  [1 1 1]
%  [2 2 2]]
% cycle counter =======================================================
% [[120 120 120]
%  [120 120 120]
%  [120 120 120]]
% recv counter N ========================================================
% [[ 1  1  1]
%  [33 31 29]
%  [29 28 29]]
% recv counter S ========================================================
% [[31 33 31]
%  [33 31 29]
%  [ 1  1  1]]
% recv counter E ========================================================
% [[31 29  1]
%  [28 29  1]
%  [30 33  1]]
% recv counter W ========================================================
% [[ 1 28 29]
%  [ 1 31 32]
%  [ 1 33 30]]
% send counter N ========================================================
% [[  0   0   0]
%  [124 130 124]
%  [132 122 114]]
% send counter S ========================================================
% [[130 126 112]
%  [118 112 118]
%  [  0   0   0]]
% send counter E ========================================================
% [[112 116   0]
%  [124 130   0]
%  [132 122   0]]
% send counter W ========================================================
% [[  0 126 112]
%  [  0 112 118]
%  [  0 120 128]]

In addition to unit and integration tests, we performed a simple experiment to validate generated phylogenetic reconstructions.
In this experiment, we evolved a population of simple genomes with HStrat annotations under drift conditions on the island model GA kernel, exported end-state genomes for postprocessing, and used the HStrat annotations to reconstruct their phylogenetic history.

Simulation ran for 120 PE generation cycles with a tournament size of 5 and a population size of 32 per PE.
For simplicity, drift conditions were imposed --- all genomes were evaluated to a fitness value of 0.0.
Due to slow execution of the hardware simulator, we performed this experiment using a small 3x3 grid of processor elements.

Genomes were fixed-length 3-word arrays represented using data type \texttt{u32}.
Figure \ref{fig:validation-example:genomes} details the content and layout of genomes, and provides example genome values yielded from simulation.
Notably, the first sixteen bits were used to tag clade geneses.
At the outset of simulation, founding population members were each assigned a randomized tag value.
This value was inherited without mutation throughout simulation.
Thus, it can be used to identify end-state genomes that evolved from the same original ancestor.

The send buffers were sized to hold one genome and the receive buffers to hold 4 genomes.
Within the simulation window, between 28 and 33 receive cycles were completed for each PE and between 112 and 132 send cycles were completed for each PE.

\input{fig/validation-example.tex}

At the end of simulation, one genome was sampled per PE.
Figure \ref{fig:validation-example:phylogeny} shows the result of phylogenetic reconstruction on these sampled genomes.
To simplify visualization of the phylogeny with existing phyloinformatic tools, all clades were stitched together into a single tree by attaching them to a common ancestor.
Taxa are colored according to their clade genesis tag.
Taxon arrangement in the reconstructed tree agrees well with founding clade identities.
All different-colored taxa are predicted to have had ancient common ancestry.
Note that relatedness between \texttt{0x5fb} and \texttt{0xde40} is slightly overestimated, due to a configured lack of precise resolution necessary to ensure compact genetic annotations.
Applications requiring high reconstruction precision can opt to use larger HStrat annotations.

\subsection{Software and Data Availability}

Reported work used CSL code hosted on GitHub at \url{https://github.com/mmore500/wse-sketches/tree/v0.1.0} \citep{moreno2024wse} with the Cerebras SDK v1.0.0 compiler and hardware emulator \citep{selig2022cerebras}.
Reference Python implementations for HStrat surface algorithms are v0.3.0 at \citep{moreno2024hsurf}.
Reconstruction used the Python \texttt{hstrat} package, v1.11.1 \citep{moreno2022hstrat}.
Data from this experiment is available via the Open Science Framework at \url{https://osf.io/bfm2z/} \citep{moreno2024toward} and associated notebook code can be found at \url{https://hopth.ru/cm}.


==> binder-wse-sketches/tex-access-proposal/text/frontmatter.tex <==
\title{\vspace{-1cm}Characterization of Phylogenetic Structure Across Population Scales using Wafer-scale Agent-based Evolution Simulation}

\author[1,2,3]{\vspace{-0.5cm}\normalsize Matthew Andres Moreno\thanks{\normalsize Corresponding Author: morenoma@umich.edu}}
\author[4,5]{\normalsize Emily Dolson}
\author[1,2]{\normalsize Luis Zaman\vspace{-0.5cm}}

\affil[1]{\footnotesize Ecology and Evolutionary Biology, University of Michigan, Ann Arbor, USA}
\affil[2]{\footnotesize Center for the Study of Complex Systems, University of Michigan, Ann Arbor, USA}
\affil[3]{\footnotesize Michigan Institute for Data Science, University of Michigan, Ann Arbor, USA}
\affil[4]{\footnotesize Computer Science and Engineering, Michigan State University, East Lansing, USA}
\affil[5]{\footnotesize Ecology, Evolution, and Behavior, Michigan State University, East Lansing, USA}

\date{} % Suppress the date

\maketitle
\vspace{-1.5cm}

==> binder-wse-sketches/tex-access-proposal/text/references.tex <==
{ \footnotesize
\putbib
}

==> binder-wse-sketches/tex/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> binder-wse-sketches/tex/lib/dependencies.tex <==
\usepackage{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{import}
\usepackage{natbib}
\usepackage{siunitx}
\usepackage{subcaption}
\usepackage{textcomp}
\usepackage{xcolor}


==> binder-wse-sketches/tex/lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> binder-wse-sketches/tex/lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
asdf
}


==> binder-wse-sketches/tex/lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> binder-wse-sketches/tex/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> binder-wse-sketches/tex/lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> binder-wse-sketches/tex/lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> binder-wse-sketches/tex/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> binder-wse-sketches/tex/text/body.tex <==
\input{text/body/abstract.tex}

\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> binder-wse-sketches/tex/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}


==> binder-wse-sketches/tex/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

example \citep{gagliardi2019international}


==> binder-wse-sketches/tex/text/body/methods.tex <==
\section{Methods} \label{sec:methods}


==> binder-wse-sketches/tex/text/body/results-and-discussion.tex <==
\section{Results and Discussion} \label{sec:results}


==> binder-wse-sketches/tex/text/frontmatter.tex <==
\title{ TODO }

\author{
Matthew Andres Moreno\\
Computer Science and Engineering \\
Michigan State University\\
East Lansing, United States \\
\url{https://orcid.org/0000-0003-4726-4479} \\
\and
Charles Ofria
Computer Science and Engineering \\
Michigan State University\\
East Lansing, United States \\
\url{https://orcid.org/0000-0003-2924-1732}
}

\maketitle


==> binder-wse-sketches/tex/text/references.tex <==
\section*{References}

\putbib


==> binder/tex-access-proposal/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> binder/tex-access-proposal/fig/async-ga-schematic.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\includegraphics[width=\linewidth]{img/async-ga-schematic.pdf}
\centering
\caption{Schematic overview of asynchronous island model evolutionary algorithm.}
\label{fig:async-ga-schematic}
\end{wrapfigure}


==> binder/tex-access-proposal/fig/hsurf-schematic.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\includegraphics[width=\linewidth]{img/hsurf-schematic.pdf}
\centering
\caption{Panel A shows update sequence on a four-site HStrat curation space-time memory under steady policy. Panel B contrasts steady policy with tilted policy, which prioritizes recent data.}
\label{fig:hsurf-schematic}
\end{wrapfigure}


==> binder/tex-access-proposal/fig/runtime-posthoc-schematic.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\includegraphics[width=\linewidth]{img/runtime-posthoc-schematic.pdf}
\caption{Proposed agent-based evolutionary simulation and observation framework, using HStrat markers to estimate phylogenetic history, thereby, infer evolutionary dynamics.}
\label{fig:runtime-posthoc-schematic}
\end{wrapfigure}


==> binder/tex-access-proposal/fig/validation-example.tex <==
\begin{figure}[htbp]
    \centering

    % Top panel for the image
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{binder/binder/teeplots/genome=hsurftiltedsticky_tagged+viz=draw-biopython-tree+ext=}
        \caption{%
          Reconstructed phylogeny, generated under the assumption of shared ancestry.
          Hexidecimal codes in taxon names are fixed random markers generated at simulation start-up, indicating independent lineage originations.
          Color coding indicates clades with independent lineage originations.
          As expected, low relatedness is predicted for taxa originating from independent lineages.
        } \label{fig:validation-example:phylogeny}
    \end{subfigure}

    % Space between image and table
    \vspace{10pt}

    % Bottom panel for the table
    \begin{subfigure}[b]{\textwidth}

\begin{minipage}[t]{\textwidth}
\centering
\footnotesize
\begin{tabular}{
c
>{\columncolor{LighterBlue}}c
>{\columncolor{LighterBlue}}c
>{\columncolor{LighterSalmon}}c
>{\columncolor{LighterSalmon}}c
q % Thick divider
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
q % Thick divider
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
}
& \multicolumn{4}{cq}{\cellcolor{white}Word 0} & \multicolumn{4}{cq}{\cellcolor{white}Word 1} & \multicolumn{4}{c}{\cellcolor{white}Word 2} \\
\cmidrule(l{1.5pt}r{1.5pt}){2-5}
\cmidrule(l{1.5pt}r{1.5pt}){6-9}
\cmidrule(l{1.5pt}r{1.5pt}){10-13}
Byte & {\cellcolor{white}0} & {\cellcolor{white}1} & {\cellcolor{white}2} & {\cellcolor{white}3} & {\cellcolor{white}4} & {\cellcolor{white}5} & {\cellcolor{white}6} & {\cellcolor{white}7} & {\cellcolor{white}8} & {\cellcolor{white}9} & {\cellcolor{white}10} & {\cellcolor{white}11} \\
\cmidrule(l{1.5pt}r{1.5pt}){2-2}
\cmidrule(l{1.5pt}r{1.5pt}){3-3}
\cmidrule(l{1.5pt}r{1.5pt}){4-4}
\cmidrule(l{1.5pt}r{1.5pt}){5-5}
\cmidrule(l{1.5pt}r{1.5pt}){6-6}
\cmidrule(l{1.5pt}r{1.5pt}){7-7}
\cmidrule(l{1.5pt}r{1.5pt}){8-8}
\cmidrule(l{1.5pt}r{1.5pt}){9-9}
\cmidrule(l{1.5pt}r{1.5pt}){10-10}
\cmidrule(l{1.5pt}r{1.5pt}){11-11}
\cmidrule(l{1.5pt}r{1.5pt}){12-12}
\cmidrule(l{1.5pt}r{1.5pt}){13-13}
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 0} & \texttt{F9} & \texttt{02} & \texttt{79} & \texttt{00} & \texttt{8D} & \texttt{22} & \texttt{4F} & \texttt{F3} & \texttt{D2} & \texttt{78} & \texttt{AD} & \texttt{C7} \\
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 1} & \texttt{F9} & \texttt{02} & \texttt{75} & \texttt{00} & \texttt{8D} & \texttt{A1} & \texttt{CB} & \texttt{F2} & \texttt{D1} & \texttt{5B} & \texttt{CC} & \texttt{D4} \\
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 2} & \texttt{61} & \texttt{B6} & \texttt{65} & \texttt{00} & \texttt{66} & \texttt{29} & \texttt{B4} & \texttt{F0} & \texttt{62} & \texttt{99} & \texttt{5A} & \texttt{61} \\
{\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} &
{\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} \\
\end{tabular}
\end{minipage}


        \caption{%
          Example genomes sampled after simulation completion.
          In validation testing, genomes were composed of three 32-bit words.
          The first two bytes (blue) are fixed random markers generated at simulation start-up, indicating independent lineage originations.
          The next two bytes (salmon) are a generation counter.
          Bits within the final eight bytes are lineage checkpoint values to facilitate phylogenetic reconstruction, arranged according to a tilted hereditary stratigraphic algorithm.
          Note that this genome does not include any content affecting agent traits or fitness --- neutral selection was used for this validation experiment.
        } \label{fig:validation-example:genomes}
    \end{subfigure}

    \caption{
      Synopsis of preliminary experiment used to validate Cerebras Software Language implementation of asynchronous agent-based evolution framework and hereditary stratigraphy algorithms.
      Experiments were performed on Cerebras SDK hardware simulator.
      Subfigure \ref{fig:validation-example:phylogeny} shows an example reconstructed phylogeny from genomes tagged with fixed random identifiers that identify independent lineage originations.
      Subfigure \ref{fig:validation-example:genomes} overviews layout of fixed-size genomes used for validation testing and shows example end-state genomes corresponding to phylogeny taxa.
    }
    \label{fig:validation-example}
\end{figure}


==> binder/tex-access-proposal/lib/dependencies.tex <==
\usepackage{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{authblk}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{colortbl}
\usepackage{csvsimple}
\usepackage{csquotes}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{import}
\usepackage{natbib}
% \usepackage[moderate]{savetrees}
\usepackage{enumitem}
\setlist{nosep,topsep=-\parskip,noitemsep}
\usepackage{siunitx}
\usepackage{subcaption}
\usepackage{tabularx}
\usepackage{textcomp}
\usepackage{wrapfig}
\usepackage{xcolor}

% Define lighter colors
\definecolor{LighterBlue}{rgb}{0.84, 0.92, 0.95}
\definecolor{LighterSalmon}{rgb}{1.0, 0.81, 0.76}
\definecolor{LighterPastelGreenYellow}{rgb}{0.88, 0.96, 0.90}

% Define thick vertical lines for section dividers
\newcolumntype{q}{!{\color{white} \vrule width 2pt}}

\setlength\parindent{24pt}
\captionsetup{font=small}
\setlength{\bibsep}{0pt plus 0.3ex}

\usepackage{ragged2e}
\setlength{\RaggedRightParindent}{\parindent}

==> binder/tex-access-proposal/lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> binder/tex-access-proposal/lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
asdf
}


==> binder/tex-access-proposal/lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> binder/tex-access-proposal/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> binder/tex-access-proposal/lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> binder/tex-access-proposal/lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> binder/tex-access-proposal/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> binder/tex-access-proposal/text/body.tex <==
% \input{text/body/abstract.tex}

\input{text/body/introduction.tex}

\input{text/body/objectives.tex}

\input{text/body/methods.tex}

\input{text/body/preliminary-work.tex}

\input{text/body/conclusion.tex}

\input{text/body/key-considerations.tex}

==> binder/tex-access-proposal/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

Proposed work lays the foundations to harness wafer-scale computing for agent-based modeling.
Orders-of-magnitude scale-up will bring entirely new classes of cross-scale dynamics within reach across many ABM application areas.
To advance on this front, we explore a fundamental re-frame of simulation that shifts from a paradigm of complete, perfect data observability to dynamic, approximate observability akin to estimation approaches traditionally used to study physical systems.

Within ABM, our proposed work focuses in particular on the topic of evolutionary computation.
We will harness cutting-edge \textit{hereditary stratigraphy} (HStrat) approaches to distributed phylogenetic tracking to investigate fundamental questions about the relationship between phylogenetic structure, population scale, and time scale.
These new HStrat methods, and extensive development targeting the Cerebras CSL using the SDK hardware simulator, position our project to hit the ground running.
Our project design emphasizes concrete steps to demonstrate and evaluate novel algorithms to establish strong technical foundations for follow-on work with distributed agent-based digital evolution.
We are committed to organizing project implementation to produce reusable CSL and Python software tools to catalyze research capabilities among the broader ABM community.

Potential extensions of this work include repurposing HStrat's rolling cross-temporal sampling algorithms to facilitate efficient downsampled observability in additional application domains.
Possibilities include sampling time series activity at simulation sites or extracting coarsened agent histories (e.g., position over time).
Within the domain of evolution modeling, we anticipate building from the work proposed here to conduct cross-scale evo-epidemiological research into how pathogen trait evolution confronts fitness trade-offs related to within-host infection dynamics and between-host transmissibility.


==> binder/tex-access-proposal/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

Agent-Based Modeling (ABM) has gained increasing adoption as a method to answer basic science questions and inform policy decisions.
Despite a wide berth of application domains --- spanning sectors like transportation infrastructure, public health, telecommunications, materials science and more --- much ABM work is unified by a common theme of interest in cross-scale dynamics.
To provide such insight, ABM requires sufficient scale to capture systems' emergent behaviors.
Advances in high-performance computing (HPC) have already yielded paradigm-shifting improvements to the capabilities of ABM.
However, across domains key questions remain out of computational reach.

\input{fig/runtime-posthoc-schematic.tex}
Significant untapped potential for ABM scale-up has been identified in hardware-accelerator-enabled computation.
Rapid advances in the capability of accelerator devices, driven in particular by market demand for deep learning operations, are anticipated to play a key role in future advances in ABM capabilities \citep{perumalla2022computer}.
Within this category, the emerging class of fabric-based accelerators, most notably the recently-introduced 850,000 core Cerebras CS-2 Wafer Scale Engine (WSE) \citep{lauterbach2021path,lie2022cerebras}, is a particularly exciting --- and fairly uncharted, with applications to HPC workloads still in early days.
This paradigm interfaces multitudinous processor elements (PEs) in a physical lattice, with PEs executing independently using individual on-chip memory and local PEs interacting through a network-like interface.

\subsection{Objectives}

This proposal establishes foundations for next-generation accelerator-enabled ABM computation by decentralized, approximate data export from agent-based evolutionary simulation.
In particular, we will evaluate asynchronous approaches for ABM migration/interaction on the WSE architecture to power agent-based evolution simulations, incorporating cutting-edge methods for distributed approximate phylogenetic (i.e., ancestry tree) tracking.

Proposed work advances two technical objectives:
\begin{enumerate}
\item to evaluate and demonstrate new approaches for phylogenetic tracking in a massively-distributed, resource-constrained setting,
\item to test the scalability of desynchronized agent migration procedures on WSE hardware,
\end{enumerate}

These technical capabilities will unlock capability to investigate a broad array of science questions.
In this proposal, we focus on one science objective:
\begin{enumerate}
\item to evaluate how phylogenetic structure scales across orders-of-magnitude population sizes, and the extent to which commonly used phylogeny structure metrics are scale-invariant or scale-sensitive.
\end{enumerate}

% Proposed work falls within the domain of agent-based evolution modeling, and uses it to  phylogenetics-related inquiry by leveraging Cerebras WSE hardware.
Our dual technical objectives constitute significant advancement of methodological capabilities within agent-based digital evolution, and our project will directly address fundamental open questions within the domain of phylogenetic theory.
However, findings and methodologies will also generalize to other ABM domains beyond evolutionary simulation and to broader classes of highly distributed HPC architectures.

\subsection{Agent-based Evolution Simulation}

Evolutionary processes are not confined to matters of natural history.
Rather, evolutionary processes pervade our contemporary, everyday world.
Key societal challenges stem from evolving systems: antibiotic resistance, epidemiology, conservation biology, and oncology among others.  % citations?
Evolutionary biology provides the fundamental foothold to efforts to address these problems \citep{aktipis2013evolutionary}.

Mathematical and computational modeling complements natural history field work and benchtop evolution experiments as a crucial third leg to stand evolutionary inquiry.
Simulation-based approaches provide key capabilities complementary to work with natural systems: complete observability, arbitrary manipulability, and rapid generational turnover.
Within this context, agent-based simulation plays an important connective role between natural systems and abstracted, aggregate-based mathematical and numerical models.
Agent-based approaches instantiate \textit{bona fide} evolutionary processes that track populations of virtual genomes subject to mutation, heredity, and selection \citep{pennock2007models}.
This characteristic incorporates some of the critical complications and subtleties characteristic of natural systems --- e.g., arbitrary agent behavior, sophisticated agent-agent interactions, and complex genotype-phenotype maps, albeit at significantly reduced scope and sophistication.

Indeed, agent-based evolution approaches have provided means for fruitful investigation of wide-ranging hypotheses, including evolution of evolvability \citep{wilke2001evolution}, host-parasite co-evolution \citep{zaman2014coevolution}, evolution of complex traits \citep{lenski2003evolutionary}.

Ambitious work advancing the field increasingly targets large cross-scale questions, including major transitions in evolution (e.g., multicellularity and symbiosis) \citep{goldsby2020major,vostinar2021symbiosis} and open-ended evolution (e.g., long-term trajectories of complex ecosystems with strong biotic selection) \citep{stanley2019open,taylor2016open}.
Progress on these fronts demands computational substrate for orders-of-magnitude larger simulation scale than tractable today \citep{moreno2022exploring,channon2019maximum}.

%as well as scenarios where replicating entities like cultural artifacts or computer viruses.
% At the frontiers of evolutionary computation, there is in particular growing interest in the question of ``open-ended evolution'' \citep{}.
% This refers to the problem of the inability to recreate the ongoing generation of novelty, complexity, and adaptation within the natural world.

\subsection{HPC and Agent-based Evolution}
% opportunity


% Evolutionary questions often explicitly span scopes, with key areas of inquiry including ecologies of interacting populations and assembly of individuals into multicellular organisms and eusocial colonies \citep{morenoDISHTINYTODO, citephageTODO}.
Researchers using agent-based evolution recognize HPC as critical to the future of the field \citep{ackley2016indefinite}.
Indeed, the field has played host to notable boundary-pushing approaches to computing at the frontiers of computing hardware and modalities such as best-effort computing, reservoir computing, global-scale time-available computing, and modular tile-based computing in addition to more traditional cluster and GPU-oriented approaches \citep{moreno2021conduit,ackley2020best,ackley2023robust,heinemann2008artificial,miikkulainen2024evolving}.

The diversity of HPC strategies for evolutionary simulation stems in large part from unique properties largely distinct from other HPC application domains.
Given its inherent underlying stochastic nature and the stabilizing influence of adaptive selection, evolutionary simulation can often tolerate significant arbitrary asynchronicity or even entirely lost simulation components (e.g., dropped messages, crashed nodes, etc.).
Likewise, digital evolution is typically amenable to locality restrictions of computation due to the inherent spatial structure of natural systems we are seeking to model.
% In particular, massively-distributed, spatial computing being directly highlighted to be of particular interest \citep{ackleyTODO}.
Because agent behavior evolves over time, the influence of population-level drift and adaptive change can inject extreme heterogeneity into the computational workload profile of evolutionary simulation over time and simulation space.
Finally, emerging research questions have introduced challenging communication-intensive requirements to support rich interactions between evolving agents.
The largely decoupled nature of classic approaches within evolutionary computation like island models or controller/worker schemes  \citep{bennett1999building,cantu2001master} no longer suffice to realize the dynamic, communication-intensive interaction characteristic of major transitions in individuality (e.g., multicellularity) and ecological communities \citep{moreno2022engineering}.

These distinctive workload properties position agent-based evolution as a potentially valuable testbed for HPC innovation and leadership.
% There is reason to expect a highly synergistic, reciprocal relationship between digital evolution and the broader HPC enterprise.
Work proposed here steps in this direction, seeking to blaze new territory that opens new possibilities to benefit broader constituencies of ABM/HPC practitioners.

However, despite the strong motivation for large-scale simulation, the algorithmic pliability of evolutionary simulation, and the increasing availability of highly capable parallel, distributed, and accelerator-driven hardware platforms, significant methodological limitations currently hold back scale-up of digital evolution.
Work proposed here takes significant steps to position the agent-based evolution simulations to benefit significantly from this emerging class of hardware accelerators.

\subsection{Phylogenetic Tracking Methods}

To serve as a useful experimental platform, digital evolution simulations must be observable.
In addition to end-state information (i.e., evolved traits), scientific questions demand information sufficient to characterize the underlying mode and tempo of evolution.
Additionally, it is often useful to be able to trace the history of notable evolutionary events (e.g., extinctions, evolutionary innovations)
Observability counts, too, in application-oriented aspects of evolutionary computation, where such data serves as a critical diagnostic to tune configuration for good performance \citep{hernandez2022can}.

In evolutionary biology, phylogenetic history is a valuable tool for triangulating the context of notable evolutionary events, as well as characterizing the underlying mode and tempo of evolution.
The same holds true in evolutionary simulation.
% https://github.com/mmore500/phylotrack-algorithm-analysis/blob/fe16d2b2d7df99faade09c01b72f681160749f51/tex/text/body/introduction.tex
In addition to addressing questions of natural history, access to the phylogenetic record of biological life has proven informative to conservation biology, epidemiology, medicine, and biochemistry among other domains \citep{faithConservationEvaluationPhylogenetic1992, STAMATAKIS2005phylogenetics, frenchHostPhylogenyShapes2023,kim2006discovery}.
Nonetheless, existing analyses of phylogenetic structure within digital systems have already proven valuable, enabling diagnosis of underlying evolutionary dynamics \citep{moreno2023toward,hernandez2022can,shahbandegan2022untangling, lewinsohnStatedependentEvolutionaryModels2023a} and even serving as mechanism to guide evolution in application-oriented domains \citep{lalejini2024phylogeny,lalejini2024runtime,murphy2008simple,burke2003increased}.
Further, comparison of observed phylogenies against simulation phylogenies can be used to evaluate hypotheses for underlying dynamics within real-life evolutionary/epidemiological systems \citep{giardina2017inference,voznica2022deep}.

Unfortunately, existing approaches to recording phylogenetic history from digital evolution simulations do not scale robustly.
Simulation phylogenies have typically been collected using a centralized record-keeping approach where every reproduction event is stitched together in a tree data structure to produce a complete record.
Record-keeping often involves pruning the records of extinct lineages to prevent memory bloat \citep{dolson2023phylotrack}.
Although the direct-tracking approach is well suited to serial simulation substantial limitations and runtime overhead make scaling this up to highly parallel/distributed systems --- particularly those with low memory capacity like the Cerebras WSE --- essentially untenable \citep{moreno2024analysis}.

To overcome this limitation to phylogenetic analysis within many-processor HPC contexts, we have proposed a new class of reconstruction-based approaches to phylogenetic tracking in silico \citep{moreno2022hereditary}.
These approaches require no centralized data collection during simulation runtime; instead, they use post hoc comparisons between end-state agent genomes to deduce approximate phylogenetic history --- akin to how DNA-based analyses tell how lineages of contemporary organisms relate in natural history.
Figure \ref{fig:runtime-posthoc-schematic} depicts our reconstruction-based strategy.

To achieve efficient, tractable phylogenetic reconstructions in practice, some careful consideration is required.
DNA-based is notoriously data-hungry, typically requiring on the order of thousands of genome sites, and can be significantly biased by physical/functional traits of the underlying genetic information.
These concerns motivated our recent development of HStrat, a genetic architecture explicitly designed for fast, accurate reconstruction requiring only small amounts of data.
HStrat data is designed to be attached to the underlying genomes within particular digital evolution systems as a neutral annotation.
Benchmarking experiments to evaluate HStrat performance have achieved high-quality reconstruction of phylogenetic histories for tens of thousands of fully distributed agents using just 96 bits of tracking information per agent genome.
Details on this methodology and our proposed approach to translate it to the WSE context are provided in Section \ref{sec:methods}.

% \subsection{Outline}

% The remainder of this proposal is structured as follows
% \begin{itemize}
% \item Section \ref{sec:objectives} describes proposed work,
% \item Section \ref{sec:methods} overviews proposed methods,
% \item Section \ref{sec:preliminary-work} reviews established work on this project,
% \item Section \ref{sec:conclusion} provides concluding remarks, and
% \item Section \ref{sec:key-considerations} recaps key technical considerations highlighted in the program solicitation.
% \end{itemize}


==> binder/tex-access-proposal/text/body/key-considerations.tex <==
\section{Key Considerations} \label{sec:key-considerations}

\begin{enumerate} \itshape \bfseries
\item %
% Using the SDK requires programming in CSL, a C-like language designed specifically for the problem of massively parallel programming on the CS-2.
What is your experience with HPC programming paradigms and languages, such as MPI, OpenMP, CUDA, OpenCL, etc.?
\end{enumerate}
\noindent
Dr. Moreno has extensive experience working with HPC technologies, most notably developing asynchronous, best-effort computing approaches using MPI and C++.
He has also received training in GPU programming (e.g., OpenCL, CUDA).
Dr. Dolson and Dr. Zaman are both experienced systems-level programmers.

\begin{enumerate}[resume] \itshape \bfseries
\item What are the underlying computational algorithms you're interested in exploring?
What existing software packages or libraries use these algorithms?
\end{enumerate}
\noindent
The core algorithm is an island-style GA, which is well-supported by digital evolution frameworks targeting serial processing on traditional HPC hardware \citep{bohm2017mabe}.
Those that support parallelism generally apply a centralized coordinator-worker strategy \citep{fortin2012deap}, which is best suited to small population sizes with expensive fitness evaluations.

\begin{enumerate}[resume] \itshape \bfseries
\item How is this problem bottlenecked on current hardware?
% Is the problem more bottlenecked by memory bandwidth, or communication costs associated with scaling up across distributed compute nodes?
\end{enumerate}
\noindent
Memory bandwidth and synchronization costs to exchange population members.
Compute bound memory latency.

\begin{enumerate}[resume] \itshape \bfseries
\item What range of problem sizes are you interested in addressing?
% For example, how much memory does your problem use?
How does memory usage or program run-time scale with problem size?
\end{enumerate}
\noindent
We are interested in developing population-scale, cross-scale simulations with hundreds of millions of agents.
The memory usage of the program and run-time scale linearly with problem size, either defined as evolutionary duration or population size.
Precise memory usage depends largely on the agent genomes used.
For smaller agent genomes, sized on the order of four words, thousands of agents could be supported per PE --- yielding a net whole-wafer population size on the order of a billion agents.

\begin{enumerate}[resume] \itshape \bfseries
\item What portion of your algorithm do you plan to port to the CS-2?
% Why are you interested in exploring this part of your algorithm?
\end{enumerate}
\noindent
We plan to port the core evolutionary generational loop to the CS-2 as an island model-style genetic algorithm.
The stages are 1) migration, 2) selection, 3) replication with mutation.
We are interested in porting it because it is the most computationally intensive to scale and because it is embarrassingly parallel.
Postprocessing to analyze evolved traits, and reconstruct evolutionary history will take place off-device.

\begin{enumerate}[resume] \itshape \bfseries
\item %
% The CS-2 offers native half and single precision data types.
What precision does your algorithm or use case need?
\end{enumerate}
\noindent
Due to the agent-based modeling, this is a primarily discrete domain.
However, floating point types may be used to represent traits.
Because they are only used for comparisons between agents, single or half precision suffice.

\begin{enumerate}[resume] \itshape \bfseries
\item %
% The CS-2 is a network-attached accelerator. 
% At a high level, the CSL programming model is similar to that of CUDA, in which data is moved between host CPU nodes and the device (CS-2) on which computational kernels are launched.
How often will data need to be moved between the wafer and the worker nodes?
\end{enumerate}
\noindent
For preliminary versions of the project, we are planning to only collect data at the end of execution through the Cerebras memcpy infrastructure.
As the model is self-contained, no data except for the PE code will need to be moved onto the device.
In the future, we are interested in exploring samples throughout the evolutionary process to serve as a kind of ``fossil record.''

\begin{enumerate}[resume] \itshape \bfseries
\item Describe your general plan to map your problem onto 850,000 cores. 
% In answering this question, it might be helpful to recall some details of the CS-2 architecture.
% The 850,000 cores are laid out in a mesh, with each core connected on fabric to its four nearest neighbors on the East, South, North, and West.
% Memory is distributed among the cores, with each core having 48 KB of local memory.
% 64-bit local memory reads and writes take roughly a cycle, as does sending and receiving 32-bit messages between the four neighboring cores.
\end{enumerate}
\noindent
We plan to exploit an island model genetic algorithm where each PE is an island and genomes migrate between adjacent islands.
As natural systems are typically asynchronous, synchronization is not a concern.
We plan to use CSL asynchronous send/receive operations to implement migration.

Genomes will be represented as contiguous buffers of u32 and each PE's population as a contiguous buffer of genome data using a simple synchronous generational model (i.e., a swap buffer.)
Population-level operations (e.g., selection, reproduction, mutation) will take advantage of the CSL's data structure descriptors.
The local memory is sufficient for a population size on the order of hundreds or low thousands.
This could give a global population size on the order of hundreds of millions.


==> binder/tex-access-proposal/text/body/methods.tex <==
\section{Methods} \label{sec:methods}

In this section, we describe the primary two algorithmic components for our on-device simulation:
\begin{enumerate}
\item the asynchronous compute-communicate cycle used to instantiate an island model evolutionary process across the WSE engine, and
\item the lightweight hereditary stratigraphy element used to annotate virtual genomes and facilitate robust \textit{post hoc} phylogenetic reconstruction.
\end{enumerate}

\subsection{Asynchronous Island-model Evolutionary Computation}

\input{fig/async-ga-schematic.tex}
We apply an island-model genetic algorithm to instantiate an evolutionary process spanning PEs.
Island-model approaches are common in applications of parallel and distributed computing to evolutionary computation \citep{bennett1999building}.
Under this model, each processor element (PE) hosts an independent population.
Migration between PEs stitches island populations together into a common gene pool.

Core kernel activity proceeds via an update cycle performed on each PE, which comprises several steps.
Figure \ref{fig:async-ga-schematic} provides a schematic overview.

The first step of this update loop is to handle migration, depicted as blue-red arrows in Figure \ref{fig:async-ga-schematic}.
We adopt a fully asynchronous approach to migration between neighboring PEs.
Evolutionary processes tend to occur asynchronously with arbitrary factors influencing things, so this is a reasonable relaxation to make.

Each PE maintains independent immigration buffers and emigration buffers dedicated to each cardinal neighbor, depicted in blue and red, respectively, in Figure \ref{fig:async-ga-schematic}.
On simulation startup, an asynchronous DSD receive operation is opened to accept genomes from neighboring PEs into the appropriate immigration buffer.
At startup, additionally, the emigration buffer is populated with one or more genomes copied from the population.
Then, an asynchronous send request is opened to dispatch wavelets containing genome data from the emigration buffer to the neighbor.
Both operations register an on-completion callback to set a ``send complete'' or ``receive complete'' flag variable associated with their corresponding buffer.

In each update cycle, the main update loop tests all ``send complete'' and ``receive complete'' flags.
For each immigration flag that is set, corresponding received genomes are written into the main population buffer, replacing randomly chosen population members.
Then, the flag is reset a new receive request is initiated.
Likewise, for each emigration flag set, corresponding send buffers are re-populated with randomly sampled genomes from the main population buffer.
Corresponding flags are then reset and new send requests are initiated.
The bottom right corner of Figure \ref{fig:async-ga-schematic} summarizes this process.

The remainder of the main update loop handles evolutionary operations within the scope of the executing PE.
Each genome within the population is evaluated to produce a floating point fitness value.
Modular implementation ensures evaluation criteria can be chosen appropriately for underlying experimental objectives.
For the purposes of this project, we will use a trivial fitness function that explicitly models additive accumulation of beneficial/deleterious mutations as a floating point value within each genome.

After evaluation, tournament selection is applied.
Each slot in the next generation is populated with a genome exhibiting maximal fitness among $n$ randomly sampled individuals, ties broken randomly.

Finally, a mutational operator is applied across all genomes in the next population.
As with evaluation criteria, a modular implementation allows mutation operations to be defined based on experimental objectives.
Here, we use a simple Gaussian mutation on each genome's stored fitness value.
At this point, hereditary stratigraphy annotations --- discussed next --- are updated to reflect an elapsed generation.

The process then repeats, with a self-activating wavelet dispatched to execute the next cycle of the main update loop.

Kernel source code implementing described procedures can be viewed at \url{https://hopth.ru/cl}.
Our implementation is defined modularly with respect to genome size, layout, mutational operator, and fitness evaluation criteria, allowing for direct re-use of produced software for follow-on evolution experiments on WSE hardware.

% A key question will be the extent to which intentionally desynchronizing affects performance, stability, and computation quality.

\subsection{Distributed Phylogenetic Tracking}

Our approach to the analysis of evolutionary history for wafer-scale simulation draws inspiration from the inference-based paradigm used to characterize history in natural systems.
This approach is fully distributed, with ancestry information contained within genomes themselves rather than in any external tracking mechanism.
Just as mutational drift encodes ancestry information in DNA genomes, the inference-based paradigm requires only local updates to individual genomes at runtime as generations elapse.

Recent work introducing \textit{hereditary stratigraphy} (HStrat) methodology has explored how best to organize genetic material to maximize reconstruction quality and minimize memory footprint \citep{moreno2022hstrat, moreno2022hereditary}.
Proposed work bundles HStrat material with underlying agent genomes as an instrumentative ornament, entirely neutral with respect to agent traits or fitness.

The hereditary stratigraphy algorithm associates each generation along individual lineages with an identifying ``fingerprint'' value.
Each time a generation elapses, all offspring generate a new identifier value.
Within each offspring, generated identifiers append to an inherited running chronological record of fingerprint values.
To prevent $\mathcal{O}(n)$ space complexity as generations elapse, not all fingerprints can be kept.
Instead, excess fingerprints are pruned away according to a deterministic program that ensures retention of fingerprint values from checkpoint generations spaced across evolutionary history.

% \input{fig/hsurf-schematic.tex}

Limitations of the Cerebras WSE environment required significant elaboration of hereditary stratigraphy algorithms to minimize memory use, avoid complex data structures with dynamically allocated memory, and minimize iterative computation.
We use a constant-time indexing scheme that maps each lineage's fingerprint stream onto a fixed-width memory buffer such that eviction of existing fingerprint values by new placements maintains a temporally-representative sampling over elapsed time.
We call this approach ``surface''-based to distinguish it from earlier hereditary stratigraphy methods.
Time stamps can be positionally inferred and thus do not need to be stored --- a several-fold savings that enables fingerprint values to be shrunk down and packed together.
Single-bit checkpoints have been shown to produce good quality phylogenies using only 96 bits per genome \citep{moreno2023toward}.
The semantic structure of HStrat annotations streamlines \textit{post hoc} phylogenetic reconstruction, which essentially boils down to a simple trie-building procedure
\citep{moreno2024analysis}.


==> binder/tex-access-proposal/text/body/objectives.tex <==
\section{Proposed Work} \label{sec:objectives}

Our project will unfold in three phases:
\begin{enumerate}
\item \textbf{Algorithm Validation}: compare replicate evolutionary runs across selection pressure levels, and evaluate capability of instrumentation and reconstruction pipeline to detect expected effects on phylogenetic structure in wafer-scale agent populations;
\item \textbf{Scalability Analysis}: assess stability, efficiency, and migration throughput of asynchronous agent exchange between PEs in collections ranging from hundreds of PEs, to thousands, to full wafer scale; and
\item \textbf{Phylogenetic Structure Across Population Scales}: exploit wafer scale computation to answer fundamental questions of how common phylogeny structure metrics vary with scale in time and space.
\end{enumerate}

Proposed work will provide a technical demonstration and evaluation of novel approaches that harness CS-2 capabilities for ABM, opening up an entirely new class of HPC applications for wafer-scale technology.
We will exploit this prototype software to answer foundational questions about how phylogenetic structure differs across orders-of-magnitude changes in population size.

\subsection{Algorithm Validation}

Initial work will augment existing software tests and hardware-simulation integration tests to prove the capability of newly developed genome annotations and phylogeny reconstruction processes to recover accurate, actionable depictions of evolutionary history.
We will generate experimental replicates across several levels of selection pressure by varying the tournament size in our island model genetic algorithm.
This property has well-defined expectations for effects on sum branch length in phylogenetic structure, allowing us to evaluate the capability of the developed genome instrumentation and tree reconstruction pipeline to recover expected effects from wafer-scale agent populations.

\subsection{Scalability Analysis}

To assess the scalability of asynchronous agent exchange between PEs within the Cerebras architecture, we will perform replicate benchmark experiments at collective sizes of 850k, 85k, 8.5k and 850 PEs.
At each scale, we will assess the following metrics:
\begin{itemize}
\item uniformity of cycle count across processor elements,
\item mean per-PE generational turnover rate, and
\item net migration per-PE per unit time.
\end{itemize}

\subsection{Phylogenetic Structure Across Population Scales}

We will apply the unique capabilities of WSE-enabled simulation to test the scaling properties of common phylogenetic structure metrics, including the Colless-like index, mean evolutionary distinctiveness, mean pairwise distance, and sum branch length \citep{tucker2017guide}.
% Several of these metrics are generally assumed to be perfectly or nearly scale invariant \citep{TODOaskemily}.
For metrics that explicitly scale with tree size (e.g., sum branch length) we will apply conventional normalization approaches.
Due to spatial structure introduced under the lattice island model, we expect to observe scale-dependence outcomes across metrics despite normalization.
However, the effect sign and size is difficult to predict \textit{a priori}, and will be the focus of our investigation.
Findings will strengthen foundational understanding of how evolutionary dynamics produce phylogenetic structure, especially due to the influence of two-dimensional spatial structure within many natural systems.
Strengthened theory will benefit applications in many sectors including ecology, natural history, and application-oriented evolutionary computation.

% We will collect under selection pressure and with small colletions of PEs and large collections of PEs
% Test for differences in phylogenetic structure metrics.
% (how to control for reconstruction quality?)
% Relatedly: are phylometrics time invariant to duration of simulation?
% Another objective: does streaming samples off the chip asynchronously bias phylometrics (as opposed to collecting everything all at the end.


==> binder/tex-access-proposal/text/body/preliminary-work.tex <==
\section{Preliminary Work} \label{sec:preliminary-work}

In preparation for proposed work, we joined the Cerebras SDK program \citep{selig2022cerebras} and assembled Cerebras Software Language (CSL) software implementations that will be necessary to conduct experiments with WSE hardware.
For the time being, we have used Cerebras' hardware emulator to test our software implementations.
This section reports a small-scale experiment performed to validate the core software functionality.
In addition to this integration test, software quality has also been verified through an associated unit test suite.

\subsection{Validation Experiment}

% fab w,h = 10,5
% Kernel x,y w,h = 4,1 3,3
% memcpy x,y w,h = 1,1 8,3
% whoami ===============================================================
% [[0 3 6]
%  [1 4 7]
%  [2 5 8]]
% whereami x ===========================================================
% [[0 1 2]
%  [0 1 2]
%  [0 1 2]]
% whereami y ===========================================================
% [[0 0 0]
%  [1 1 1]
%  [2 2 2]]
% cycle counter =======================================================
% [[120 120 120]
%  [120 120 120]
%  [120 120 120]]
% recv counter N ========================================================
% [[ 1  1  1]
%  [33 31 29]
%  [29 28 29]]
% recv counter S ========================================================
% [[31 33 31]
%  [33 31 29]
%  [ 1  1  1]]
% recv counter E ========================================================
% [[31 29  1]
%  [28 29  1]
%  [30 33  1]]
% recv counter W ========================================================
% [[ 1 28 29]
%  [ 1 31 32]
%  [ 1 33 30]]
% send counter N ========================================================
% [[  0   0   0]
%  [124 130 124]
%  [132 122 114]]
% send counter S ========================================================
% [[130 126 112]
%  [118 112 118]
%  [  0   0   0]]
% send counter E ========================================================
% [[112 116   0]
%  [124 130   0]
%  [132 122   0]]
% send counter W ========================================================
% [[  0 126 112]
%  [  0 112 118]
%  [  0 120 128]]

In addition to unit and integration tests, we performed a simple experiment to validate generated phylogenetic reconstructions.
In this experiment, we evolved a population of simple genomes with HStrat annotations under drift conditions on the island model GA kernel, exported end-state genomes for postprocessing, and used the HStrat annotations to reconstruct their phylogenetic history.

Simulation ran for 120 PE generation cycles with a tournament size of 5 and a population size of 32 per PE.
For simplicity, drift conditions were imposed --- all genomes were evaluated to a fitness value of 0.0.
Due to slow execution of the hardware simulator, we performed this experiment using a small 3x3 grid of processor elements.

Genomes were fixed-length 3-word arrays represented using data type \texttt{u32}.
Figure \ref{fig:validation-example:genomes} details the content and layout of genomes, and provides example genome values yielded from simulation.
Notably, the first sixteen bits were used to tag clade geneses.
At the outset of simulation, founding population members were each assigned a randomized tag value.
This value was inherited without mutation throughout simulation.
Thus, it can be used to identify end-state genomes that evolved from the same original ancestor.

The send buffers were sized to hold one genome and the receive buffers to hold 4 genomes.
Within the simulation window, between 28 and 33 receive cycles were completed for each PE and between 112 and 132 send cycles were completed for each PE.

\input{fig/validation-example.tex}

At the end of simulation, one genome was sampled per PE.
Figure \ref{fig:validation-example:phylogeny} shows the result of phylogenetic reconstruction on these sampled genomes.
To simplify visualization of the phylogeny with existing phyloinformatic tools, all clades were stitched together into a single tree by attaching them to a common ancestor.
Taxa are colored according to their clade genesis tag.
Taxon arrangement in the reconstructed tree agrees well with founding clade identities.
All different-colored taxa are predicted to have had ancient common ancestry.
Note that relatedness between \texttt{0x5fb} and \texttt{0xde40} is slightly overestimated, due to a configured lack of precise resolution necessary to ensure compact genetic annotations.
Applications requiring high reconstruction precision can opt to use larger HStrat annotations.

\subsection{Software and Data Availability}

Reported work used CSL code hosted on GitHub at \url{https://github.com/mmore500/wse-sketches/tree/v0.1.0} \citep{moreno2024wse} with the Cerebras SDK v1.0.0 compiler and hardware emulator \citep{selig2022cerebras}.
Reference Python implementations for HStrat surface algorithms are v0.3.0 at \citep{moreno2024hsurf}.
Reconstruction used the Python \texttt{hstrat} package, v1.11.1 \citep{moreno2022hstrat}.
Data from this experiment is available via the Open Science Framework at \url{https://osf.io/bfm2z/} \citep{moreno2024toward} and associated notebook code can be found at \url{https://hopth.ru/cm}.


==> binder/tex-access-proposal/text/frontmatter.tex <==
\title{\vspace{-1cm}Characterization of Phylogenetic Structure Across Population Scales using Wafer-scale Agent-based Evolution Simulation}

\author[1,2,3]{\vspace{-0.5cm}\normalsize Matthew Andres Moreno\thanks{\normalsize Corresponding Author: morenoma@umich.edu}}
\author[4,5]{\normalsize Emily Dolson}
\author[1,2]{\normalsize Luis Zaman\vspace{-0.5cm}}

\affil[1]{\footnotesize Ecology and Evolutionary Biology, University of Michigan, Ann Arbor, USA}
\affil[2]{\footnotesize Center for the Study of Complex Systems, University of Michigan, Ann Arbor, USA}
\affil[3]{\footnotesize Michigan Institute for Data Science, University of Michigan, Ann Arbor, USA}
\affil[4]{\footnotesize Computer Science and Engineering, Michigan State University, East Lansing, USA}
\affil[5]{\footnotesize Ecology, Evolution, and Behavior, Michigan State University, East Lansing, USA}

\date{} % Suppress the date

\maketitle
\vspace{-1.5cm}

==> binder/tex-access-proposal/text/references.tex <==
{ \footnotesize
\putbib
}

==> binder/tex/draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> binder/tex/lib/dependencies.tex <==
\usepackage{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{cite}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{import}
\usepackage{natbib}
\usepackage{siunitx}
\usepackage{subcaption}
\usepackage{textcomp}
\usepackage{xcolor}


==> binder/tex/lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> binder/tex/lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
asdf
}


==> binder/tex/lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> binder/tex/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
   \csname pragma@\@pragmafile\endcsname
   \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> binder/tex/lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> binder/tex/lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> binder/tex/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> binder/tex/text/body.tex <==
\input{text/body/abstract.tex}

\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> binder/tex/text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}


==> binder/tex/text/body/introduction.tex <==
\section{Introduction} \label{sec:introduction}

example \citep{gagliardi2019international}


==> binder/tex/text/body/methods.tex <==
\section{Methods} \label{sec:methods}


==> binder/tex/text/body/results-and-discussion.tex <==
\section{Results and Discussion} \label{sec:results}


==> binder/tex/text/frontmatter.tex <==
\title{ TODO }

\author{
Matthew Andres Moreno\\
Computer Science and Engineering \\
Michigan State University\\
East Lansing, United States \\
\url{https://orcid.org/0000-0003-4726-4479} \\
\and
Charles Ofria
Computer Science and Engineering \\
Michigan State University\\
East Lansing, United States \\
\url{https://orcid.org/0000-0003-2924-1732}
}

\maketitle


==> binder/tex/text/references.tex <==
\section*{References}

\putbib


==> bindertex-evolutionary-inference/draft.tex <==
\def\mydraft{
  \usepackage{draftwatermark}
  \usepackage{lineno}
  \linenumbers
  \renewcommand{\linenumberfont}{\normalfont\small\color{red}}
  % \linespread{1.5}
}
\input{main.tex}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylogenies-log-avida.tex <==
\begin{figure*}
\begin{subfigure}[b]{1\columnwidth}
\includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/avida-genome/model=avida+taxon=genome+treatment=plain+seed=1+phylogeny-snapshot-100000.pdf}
    % \end{noindent}
    \caption{%
      genome-level tracking}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/avida-organism/model=avida+taxon=organism+treatment=plain_individual+seed=1+phylogeny-snapshot-100000.pdf}
    % \end{noindent}
    \caption{%
      organism-level tracking}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \caption{%
    \textbf{Sample reference phylogenies from Avida under ``plain'' regime.}
    Time axis is log-scale.
  }
  \label{fig:perfect-tree-phylogenies-log-avida}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylogenies-log.tex <==
\begin{figure*}
  \begin{minipage}{1\columnwidth}
    \centering
    Generations Ago (approx.)
  \end{minipage}
  \hfill
  \begin{minipage}{1\columnwidth}
    \centering
    Generations Ago (approx.)
  \end{minipage}
  \begin{minipage}{1\columnwidth}
    \hspace{0.02\linewidth}
    \rotatebox{30}{\makebox[0.1\linewidth][c]{200,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{50,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{10,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{2,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{30}}
    \rotatebox{90}{\makebox[0.05\linewidth][c]{0}}
  \end{minipage}
  \hfill
  \begin{minipage}{1\columnwidth}
    \hspace{0.02\linewidth}
    \rotatebox{30}{\makebox[0.1\linewidth][c]{200,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{50,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{10,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{2,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{30}}
    \rotatebox{90}{\makebox[0.05\linewidth][c]{0}}
  \end{minipage}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=2/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=4+treatment=2+_generation=262144+_index=2+scale=log+ext=.pdf}
    % \end{noindent}
    \caption{%
      strong selection}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=14/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=1+treatment=14+_generation=262144+_index=14+scale=log+ext=.pdf}
    % \end{noindent}
    \caption{%
      weak selection}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    \centering
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=8/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=2+treatment=8+_generation=262144+_index=8+scale=log+ext=.pdf}
    % \end{noindent}
    \caption{%
      plain}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=6/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=6+_generation=262144+_index=6+scale=log+ext=.pdf}
    % \end{noindent}
    \caption{%
      spatial structure}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=26/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-06+population_size=32768+r.../eplicate=0+tournament_size=2+treatment=26+_generation=262144+_index=26+scale=log+ext=.pdf}
    % \end{noindent}
    \caption{%
      weak 4 niche ecology}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    % \begin{noindent}
      \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=24/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-06+population_size=3276.../8+replicate=0+tournament_size=2+treatment=24+_generation=262144+_index=24+scale=log+ext=.pdf}    % \end{noindent}
    \caption{%
      weak 4 niche ecology with spatial structure }
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=10/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=2+treatment=10+_generation=262144+_index=10+scale=log+ext=.pdf}
    % \end{noindent}
    \caption{%
      4 niche ecology}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=22/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=22+_generation=262144+_index=22+scale=log+ext=.pdf}
    % \end{noindent}
    \caption{%
      4 niche ecology with spatial structure}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=20/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=8+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=2+treatment=20+_generation=262144+_index=20+scale=log+ext=.pdf}
    % \end{noindent}
    \caption{%
      8 niche ecology}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{1\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=18/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=8+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=18+_generation=262144+_index=18+scale=log+ext=.pdf}
    % \end{noindent}
    \caption{%
      8 niche ecology with spatial structure}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \caption{%
    Sample reference phylogenies across surveyed evolutionary metrics.
    Each phylogeny has 32,768 leaves.
    Note log-scale $x$ axis.
  }
  \label{fig:perfect-tree-phylogenies-log}
\end{figure*}

% \begin{subfigure}[b]{1\columnwidth}
% % \begin{noindent}
% \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=0/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=4+treatment=0+_generation=262144+_index=0+scale=log+ext=.pdf}
% % \end{noindent}
% \caption{%
% spatial structure strong election}
% % \label{fig:perfect-tree-phylogenies-log:TODO}
% \end{subfigure}

% \begin{subfigure}[b]{1\columnwidth}
% % \begin{noindent}
% \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=16/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=1+treatment=16+_generation=262144+_index=16+scale=log+ext=.pdf}
% % \end{noindent}
% \caption{%
% weak selection 4 niche ecology}
% % \label{fig:perfect-tree-phylogenies-log:TODO}
% \end{subfigure}

% \begin{subfigure}[b]{1\columnwidth}
% % \begin{noindent}
% \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=12/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=1+treatment=12+_generation=262144+_index=12+scale=log+ext=.pdf}
% % \end{noindent}
% \caption{%
% spatial structure weak selection}
% % \label{fig:perfect-tree-phylogenies-log:TODO}
% \end{subfigure}

% \begin{subfigure}[b]{1\columnwidth}
% % \begin{noindent}
% \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=4/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=4+treatment=4+_generation=262144+_index=4+scale=log+ext=.pdf}
% % \end{noindent}
% \caption{%
% 4 niche ecology strong selection}
% % \label{fig:perfect-tree-phylogenies-log:TODO}
% \end{subfigure}
% \hfill


==> bindertex-evolutionary-inference/fig/perfect-tree-phylogenies-nonlog.tex <==
\begin{figure*}
  \begin{minipage}{0.5\columnwidth}
    \centering
    Generations Ago (approx.)
  \end{minipage}
  \hfill
  \begin{minipage}{0.5\columnwidth}
    \centering
    Generations Ago (approx.)
  \end{minipage}
  \begin{minipage}{0.5\columnwidth}
    \hspace{0.02\linewidth}
    \rotatebox{30}{\makebox[0.1\linewidth][c]{200,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{150,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{100,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{50,000}}
    \hfill
    \rotatebox{90}{\makebox[0.05\linewidth][c]{0}}
  \end{minipage}
  \hfill
  \begin{minipage}{0.5\columnwidth}
    \hspace{0.02\linewidth}
    \rotatebox{30}{\makebox[0.1\linewidth][c]{200,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{150,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{100,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{50,000}}
    \hfill
    \rotatebox{90}{\makebox[0.05\linewidth][c]{0}}
  \end{minipage}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=2/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=4+treatment=2+_generation=262144+_index=2+scale=nonlog+ext=.pdf}
    % \end{noindent}
    \caption{%
      strong selection}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=14/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=1+treatment=14+_generation=262144+_index=14+scale=nonlog+ext=.pdf}
    % \end{noindent}
    \caption{%
      weak selection}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    \centering
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=8/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=2+treatment=8+_generation=262144+_index=8+scale=nonlog+ext=.pdf}
    % \end{noindent}
    \caption{%
      plain}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=6/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=6+_generation=262144+_index=6+scale=nonlog+ext=.pdf}
    % \end{noindent}
    \caption{%
      spatial structure}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=26/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-06+population_size=32768+r.../eplicate=0+tournament_size=2+treatment=26+_generation=262144+_index=26+scale=nonlog+ext=.pdf}
    % \end{noindent}
    \caption{%
      weak 4 niche ecology}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    % \begin{noindent}
      \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=24/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-06+population_size=3276.../8+replicate=0+tournament_size=2+treatment=24+_generation=262144+_index=24+scale=nonlog+ext=.pdf}    % \end{noindent}
    \caption{%
      weak 4 niche ecology with spatial structure }
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=10/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=2+treatment=10+_generation=262144+_index=10+scale=nonlog+ext=.pdf}
    % \end{noindent}
    \caption{%
      4 niche ecology}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=22/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=22+_generation=262144+_index=22+scale=nonlog+ext=.pdf}
    % \end{noindent}
    \caption{%
      4 niche ecology with spatial structure}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=20/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=8+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=2+treatment=20+_generation=262144+_index=20+scale=nonlog+ext=.pdf}
    % \end{noindent}
    \caption{%
      8 niche ecology}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.5\columnwidth}
    % \begin{noindent}
    \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=18/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=8+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=18+_generation=262144+_index=18+scale=nonlog+ext=.pdf}
    % \end{noindent}
    \caption{%
      8 niche ecology with spatial structure}
    % \label{fig:perfect-tree-phylogenies-log:TODO}
  \end{subfigure}
  \hfill
  \caption{%
    \textbf{Sample reference phylogenies from the simple model across evolutionary regimes.}
    Each phylogeny has 32,768 leaves.
    Note linear-scale $x$ axis.
  }
  \label{fig:perfect-tree-phylogenies-nonlog}
\end{figure*}

% \begin{subfigure}[b]{0.5\columnwidth}
% % \begin{noindent}
% \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=0/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=4+treatment=0+_generation=262144+_index=0+scale=nonlog+ext=.pdf}
% % \end{noindent}
% \caption{%
% spatial structure strong election}
% % \label{fig:perfect-tree-phylogenies-log:TODO}
% \end{subfigure}

% \begin{subfigure}[b]{0.5\columnwidth}
% % \begin{noindent}
% \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=16/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=1+treatment=16+_generation=262144+_index=16+scale=nonlog+ext=.pdf}
% % \end{noindent}
% \caption{%
% weak selection 4 niche ecology}
% % \label{fig:perfect-tree-phylogenies-log:TODO}
% \end{subfigure}

% \begin{subfigure}[b]{0.5\columnwidth}
% % \begin{noindent}
% \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=12/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=1+treatment=12+_generation=262144+_index=12+scale=nonlog+ext=.pdf}
% % \end{noindent}
% \caption{%
% spatial structure weak selection}
% % \label{fig:perfect-tree-phylogenies-log:TODO}
% \end{subfigure}

% \begin{subfigure}[b]{0.5\columnwidth}
% % \begin{noindent}
% \includegraphics[height=0.12\textheight,width=\textwidth]{img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=4/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=32768+r.../eplicate=0+tournament_size=4+treatment=4+_generation=262144+_index=4+scale=nonlog+ext=.pdf}
% % \end{noindent}
% \caption{%
% 4 niche ecology strong selection}
% % \label{fig:perfect-tree-phylogenies-log:TODO}
% \end{subfigure}
% \hfill


==> bindertex-evolutionary-inference/fig/perfect-tree-phylogeny-gen3sis.tex <==
\begin{figure*}
\centering
\begin{subfigure}[b]{1\columnwidth}
\includegraphics[height=0.12\textheight,width=\textwidth]{img/gen3sis-species/model=gen3sis+taxon=species+treatment=plain+seed=1+phylogeny-snapshot-100000.pdf}
    % \end{noindent}
  \end{subfigure}
  \caption{%
    \textbf{Sample reference phylogeny from Gen3sis under ``plain'' regime.}
    Time axis is linear-scale.
  }
  \label{fig:perfect-tree-phylogeny-gen3sis}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-avida.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/col=phylometric+epoch=0+mut_distn=default+viz=boxplot+x=value+y=regime+ext=.pdf}
    \caption{No spatial structure.}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/col=phylometric+epoch=0+mut_distn=default+spatial=true+viz=boxplot+x=value+y=regime+ext=.pdf}
    \caption{With spatial structure.}
  \end{subfigure}
  \caption{%
    Distribution of tree phylometrics measured with perfect phylogenetic tracking across surveyed evolutionary regimes in Avida.
    Sample size of $n=30$ per distribution.
  }
  \label{fig:perfect-tree-phylometrics-avida}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-boxplot-gen3sis.tex <==
\begin{figure*}
  \centering
    \includegraphics[width=\textwidth]{binder/binder/gen3sis/teeplots/col=phylometric+epoch=0+mut_distn=default+viz=boxplot+x=value+y=regime+ext=.pdf}
  \caption{%
    Distribution of tree phylometrics measured with perfect phylogenetic tracking across surveyed evolutionary regimes under Gen3sis model.
    Sample size of $n=30$ per distribution.
  }
  \label{fig:perfect-tree-phylometrics-boxplot-gen3sis}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-gen3sis.tex <==
\begin{figure*}
  \begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/gen3sis/teeplots/epoch=0+mut_distn=default+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{non-spatial baseline}
    \label{fig:perfect-tree-phylometrics-heatmap-gen3sis}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/gen3sis/teeplots/epoch=0+mut_distn=default+spatial=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{spatial baseline}
    \label{fig:perfect-tree-phylometrics-spatial-heatmap-gen3sis}
  \end{subfigure}
  \caption{%
    Evolutionary regimes' effect sizes relative to ``plain'' baseline under the Gen3sis model with perfect phylogenetic tracking, normalized via Cliff's delta.
    Sample sizes $n=30$.
    Annotated +'s indicate small, medium, and large effect sizes using the Cliff's delta statistic and *'s indicate statistical significance at $\alpha = 0.05$ via Mann-Whitney U test.
  }
  \label{fig:perfect-tree-phylometrics-gen3sis}
\end{figure*}

==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-heatmap-avida-gen3sis.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/avida/teeplots/epoch=0+mut_distn=default+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{Avida.}
  \end{subfigure}
  \vspace{1cm} 
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/avida/teeplots/epoch=0+mut_distn=default+spatial=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{Avida, with spatial structure.}
  \end{subfigure}
  \vspace{1cm} 
  \begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/gen3sis/teeplots/epoch=0+mut_distn=default+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{gen3sis.}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/gen3sis/teeplots/epoch=0+mut_distn=default+spatial=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{gen3sis, with spatial barriers}
    \label{fig:perfect-tree-phylometrics-heatmap-avida-gen3sis}
  \end{subfigure}
  \caption{Heatmap of normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenetic records.}
  \label{fig:perfect-tree-phylometrics-heatmap-avida-gen3sis}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-heatmap-avida-genome.tex <==
\begin{figure*}
  \centering
\includegraphics[width=\textwidth]{binder/binder/avida/teeplots/epoch=0+mut_distn=default+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
\caption{%
  \textbf{Phylometrics for genotype-level phylogenies in Avida.}
  Tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenies in which the taxonomic unit is genotype rather than individual.
  Note that nonparametric effect size normalization caps out to 1.0/-1.0 past the point of complete disbributional nonoverlap.
  For heatmap charts, +'s indicate small, medium, and large effect sizes using the Cliff's delta statistic and *'s indicate statistical significance at $\alpha = 0.05$ via Mann-Whitney U test.
}  
  \label{fig:perfect-tree-phylometrics-heatmap-avida-genome}
\end{figure*}

==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-heatmap-avida.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \end{noindent}
  \caption{%
    Heatmap of normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenetic records.
    See Supplementary Figure \ref{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis} for results under sensitivity analysis conditions.
  }
  \label{fig:perfect-tree-phylometrics-heatmap}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-heatmap-gen3sis.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=0.5\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \includegraphics[width=0.5\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+spatial=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \end{noindent}
  \caption{%
  \textbf{Phylometrics in Gen3sis.}
   Evolutionary regimes' effect sizes relative to ``plain'' baseline under the Gen3sis model with perfect phylogenetic tracking, normalized via Cliff's delta.
    Sample sizes $n=30$.
  }
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-heatmap-parametric.tex <==
\begin{figure*}
  \centering
\includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+normed=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
\caption{%
  \textbf{Normalized phylometric responses.}
  Heatmap of normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity phylogenies from the simple model.
  Note that normalization shows magnitude of phylometric effect beyond the point of distributional nonoverlap, unlike nonparametric normalization which tops out with complete distributional nonoverlap.
}  
  \label{fig:perfect-tree-phylometrics-heatmap-parametric}
\end{figure*}

==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-heatmap-sensitivity-analysis.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    \centering
    % \begin{noindent}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=0+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{%
      gaussian mutation distribution at epoch 0 (generation 32,768)}
    \label{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis:epoch0}
    % \end{noindent}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    \centering
    % \begin{noindent}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=2+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{%
      gaussian mutation distribution at epoch 2 (generation 98,304)}
    \label{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis:epoch2}
    % \end{noindent}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    % \begin{noindent}
    \centering
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.exponential+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{%
      exponential mutation distribution at epoch 7 (generation 262,144)}
    \label{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis:exponential}
    % \end{noindent}
  \end{subfigure}
  \caption{%
    Sensitivity analysis results for normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenetic records.
    Normalized tree phylometrics are depicted as a heatmap for each sensitivity analysis condition.
  }
  \label{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-heatmap.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \end{noindent}
  \caption{%
    Heatmap of normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenetic records.
    See Supplementary Figure \ref{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis} for results under sensitivity analysis conditions.
  }
  \label{fig:perfect-tree-phylometrics-heatmap}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-parametric-heatmap.tex <==
\begin{figure*}
  \centering
\includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+normed=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
\caption{%
  Heatmap of normalized tree phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity simulation phylogenetic records.
  See Supplementary Figure \ref{fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis} for results under sensitivity analysis conditions.
}  
  \label{fig:perfect-tree-phylometrics-parametric-heatmap}
\end{figure*}

==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-sensitivity-analysis.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    % \begin{noindent}
    \centering
    \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=0+mut_distn=np.random.standard_normal+viz=boxplot+x=value+y=regime+ext=.pdf}
    % \end{noindent}
    \caption{%
      gaussian mutation distribution at epoch 0 (generation 32,768)}
    \label{fig:perfect-tree-phylometrics-sensitivity-analysis:epoch0}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    % \begin{noindent}
    \centering
    \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=2+mut_distn=np.random.standard_normal+viz=boxplot+x=value+y=regime+ext=.pdf}
    % \end{noindent}
    \caption{%
      gaussian mutation distribution at epoch 2 (generation 98,304)}
    \label{fig:perfect-tree-phylometrics-sensitivity-analysis:epoch2}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    % \begin{noindent}
    \centering
    \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=0+mut_distn=np.random.exponential+viz=boxplot+x=value+y=regime+ext=.pdf}
    % \end{noindent}
    \caption{%
      exponential mutation distribution at epoch 7 (generation 262,144)}
    \label{fig:perfect-tree-phylometrics-sensitivity-analysis:exponential}
  \end{subfigure}
  % \begin{noindent}
  \caption{
    Distribution of tree phylometrics across surveyed evolutionary regimes for sensitivity analysis conditions.
    Phylometrics were calculated on perfect-fidelity simulation phylogenetic records.
    Sample sizes of $n=50$ replicates define each depicted distribution.
  }
  \label{fig:perfect-tree-phylometrics-sensitivity-analysis}
  % \end{noindent}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-with-spatial-nuisance-sensitivity-analysis.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    \centering
    % \begin{noindent}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=0+mut_distn=np.random.standard_normal+nuisance=spatial-structure+viz=boxplot+x=value+y=regime+ext=.pdf}
    % \end{noindent}
    \caption{%
      gaussian mutation distribution at epoch 0 (generation 32,768)}
    \label{fig:perfect-tree-phylometrics-with-spatial-nuisance-sensitivity-analysis:epoch0}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    \centering
    % \begin{noindent}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=2+mut_distn=np.random.standard_normal+nuisance=spatial-structure+viz=boxplot+x=value+y=regime+ext=.pdf}
    % \end{noindent}
    \caption{%
      gaussian mutation distribution at epoch 2 (generation 98,304)}
    \label{fig:perfect-tree-phylometrics-with-spatial-nuisance-sensitivity-analysis:epoch2}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    \centering
    % \begin{noindent}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=0+mut_distn=np.random.exponential+nuisance=spatial-structure+viz=boxplot+x=value+y=regime+ext=.pdf}
    % \end{noindent}
    \caption{%
      exponential mutation distribution at epoch 7 (generation 262,144)}
    \label{fig:perfect-tree-phylometrics-with-spatial-nuisance-sensitivity-analysis:exponential}
  \end{subfigure}
  % \begin{noindent}
  \caption{%
    Distribution of phylometrics across surveyed evolutionary regimes with spatial structure (i.e., island count 1,024) for sensitivity analysis conditions.
    Phylometrics were calculated on perfect-fidelity simulation phylogenetic records.
    Sample sizes of $n=50$ replicates define each depicted distribution.
  }
  \label{fig:perfect-tree-phylometrics-with-spatial-nuisance-sensitivity-analysis}
  % \end{noindent}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics-with-spatial-nuisance.tex <==
\begin{figure*}
  \centering
\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=7+mut_distn=np.random.standard_normal+nuisance=spatial-structure+viz=boxplot+x=value+y=regime+ext=.pdf}
  \caption{ Distribution of phylometrics under the simple model.
    Sample sizes $n=50$.}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+spatial=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  \caption{Sizes of the effect of evolutionary regimes on each phylometric relative to ``plain'' baseline in the simple model.
    Sample sizes $n=50$.}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/col=phylometric+epoch=0+mut_distn=default+spatial=true+viz=boxplot+x=value+y=regime+ext=.pdf}
  \caption{ Distribution of phylometrics in Avida.
  Sample sizes $n=30$.}
\end{subfigure}%

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/epoch=0+mut_distn=default+spatial=true+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
\caption{%
Sizes of the effect of evolutionary regimes on each phylometric relative to ``plain'' baseline in Avida.
    Sample sizes $n=30$.
}
\end{subfigure}
\vspace{1cm}


  \caption{%
    \textbf{Phylometric responses under spatial structure.}
    Distribution of phylometrics across the three surveyed ecological regimes and the control non-ecological regime---all with spatial population structure (i.e., island count 1,024 for simple model, toroidal population grid for Avida).
    Phylometrics were calculated on perfect-fidelity phylogenies.
    Note that nonparametric effect size normalization caps out to 1.0/-1.0 past the point of complete disbributional nonoverlap.
    For heatmap charts, +'s indicate small, medium, and large effect sizes using the Cliff's delta statistic and *'s indicate statistical significance at $\alpha = 0.05$ via Mann-Whitney U test.
    Results from simple model are for standard experimental conditions: gaussian mutation distribution at epoch 7 (generation 262,144).
    See Figure \ref{fig:perfect-tree-phylometrics-with-spatial-nuisance-sensitivity-analysis} for results under sensitivity analysis conditions.
  }
  \label{fig:perfect-tree-phylometrics-with-spatial-nuisance}
\end{figure*}


==> bindertex-evolutionary-inference/fig/perfect-tree-phylometrics.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=7+mut_distn=np.random.standard_normal+viz=boxplot+x=value+y=regime+ext=.pdf}
  \caption{%
    Distribution of phylometrics under the simple model.
    Sample sizes $n=50$.
  }
  \label{fig:perfect-tree-phylometrics-simple-boxplot}
  \end{subfigure}

  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{
 Sizes of the effect of evolutionary regimes on each phylometric relative to ``plain'' baseline in the simple model.
    Sample sizes $n=50$.
    }
\label{fig:perfect-tree-phylometrics-simple-heatmap}
  \end{subfigure}%

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/col=phylometric+epoch=0+mut_distn=default+viz=boxplot+x=value+y=regime+ext=.pdf}
  \caption{
  Distribution of phylometrics in Avida.
  Sample sizes $n=30$.
  }
  \label{fig:perfect-tree-phylometrics-avida-boxplot}
\end{subfigure}%

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/epoch=0+mut_distn=default+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
\caption{%
   Sizes of the effect of evolutionary regimes on each phylometric relative to ``plain'' baseline in Avida. Sample sizes $n=30$.
}
\label{fig:perfect-tree-phylometrics-avida-heatmap}
\end{subfigure}

  \caption{%
  \textbf{Phylometric responses for simple model and Avida.}
  Phylometrics across surveyed evolutionary regimes, calculated on perfect-fidelity individual-level phylogenies from the simple model and Avida.
  Note that nonparametric effect size normalization caps out to 1.0/-1.0 past the point of complete disbributional nonoverlap.
  For heatmap charts, +'s indicate small, medium, and large effect sizes using the Cliff's delta statistic and *'s indicate statistical significance at $\alpha = 0.05$ via Mann-Whitney U test.
  Results from simple model are for standard experimental conditions: gaussian mutation distribution at epoch 7 (generation 262,144).
  See Figure \ref{fig:perfect-tree-phylometrics-sensitivity-analysis} for results under sensitivity analysis conditions.
  }
  \label{fig:perfect-tree-phylometrics}
\end{figure*}

==> bindertex-evolutionary-inference/fig/plain-perfect-and-reconstruction-phylogenies.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=\textwidth, height=0.13\textheight]{img/reference}
    \caption{%
      reference tree}
    \label{fig:plain-perfect-and-reconstruction-phylogenies:reference}
  \end{subfigure}
  \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=\textwidth, height=0.13\textheight]{img/plain_resolution_100}
    \caption{%
      1\% resolution}
    \label{fig:plain-perfect-and-reconstruction-phylogenies:resolution_100}
  \end{subfigure}
  \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=\textwidth, height=0.13\textheight]{img/plain_resolution_30}
    \caption{%
      3\% resolution}
    \label{fig:plain-perfect-and-reconstruction-phylogenies:resolution_30}
  \end{subfigure}
  \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=\textwidth, height=0.13\textheight]{img/plain_resolution_10}
    \caption{%
      10\% resolution}
    \label{fig:plain-perfect-and-reconstruction-phylogenies:resolution_10}
  \end{subfigure}
  % \begin{noindent}
  \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=\textwidth, height=0.13\textheight]{img/plain_resolution_3} \caption{%
      33\% resolution}
    \label{fig:plain-perfect-and-reconstruction-phylogenies:resolution_3}
  \end{subfigure}
  % \end{noindent}
  \caption{%
  \textbf{Comparison of phylogeny reconstructions across different hereditary stratigraphy resolutions in the plain evolutionary regime.}
    To maintain visual legibility, these trees contain the same sub-sample of 100 leaf nodes out of the 32,768 in the full trees.
    Sub-figures are arranged from top to bottom in coarsening order of reconstruction resolution.
    Taxon and branch color coding is consistent across subpanels.
    Visit \url{mmore500.com/hstrat-evolutionary-inference/} for mouseover-based highlighting of corresponding clades between reconstructions and reference.
  }
  \label{fig:plain-perfect-and-reconstruction-phylogenies}
\end{figure}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-avida.tex <==
\begin{sidewaysfigure*}
  \centering
  % \begin{noindent}
  \includegraphics[height=\textwidth,angle=-90]{binder/binder/avida-individual/teeplots/col=phylometric+epoch=0+mut_distn=default+row=regime+viz=boxplot+x=value+y=quality+ext=.pdf}
  % \end{noindent}
  \caption{%
    Distributions of phylometrics across surveyed reconstruction fidelities and evolutionary regimes under Avida model.
    Sample sizes $n=30$.
  }
  \label{fig:reconstructed-tree-phylometrics-avida}
\end{sidewaysfigure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-epoch0.tex <==
\begin{sidewaysfigure*}
  \centering
  % \begin{noindent}
  \includegraphics[height=\textwidth,angle=-90]{binder/binder/teeplots/col=phylometric+epoch=0+mut_distn=np.random.standard_normal+row=regime+viz=boxplot+x=value+y=quality+ext=.pdf}
  % \end{noindent}
  \caption{%
    Sensitivity analysis result for distributions of phylometrics across surveyed reconstruction fidelities and evolutionary regimes.
    Sensitivity analysis condition is gaussian mutation distribution at epoch 0 (generation 32,768).
    Sample sizes of $n=50$ replicates define each depicted distribution.
  }
  \label{fig:reconstructed-tree-phylometrics-epoch0}
\end{sidewaysfigure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-epoch2.tex <==
\begin{sidewaysfigure*}
  \centering
  % \begin{noindent}
  \includegraphics[height=\textwidth,angle=-90]{binder/binder/teeplots/col=phylometric+epoch=2+mut_distn=np.random.standard_normal+row=regime+viz=boxplot+x=value+y=quality+ext=.pdf}
  % \end{noindent}
  \caption{%
    Sensitivity analysis result for distributions of phylometrics across surveyed reconstruction fidelities and evolutionary regimes.
    Sensitivity analysis condition is gaussian mutation distribution at epoch 2 (generation 98,304).
    Sample sizes of $n=50$ replicates define each depicted distribution.
  }
  \label{fig:reconstructed-tree-phylometrics-epoch2}
\end{sidewaysfigure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-error-avida.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/epoch=0+hue=quality-threshold+mut_distn=default+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \end{noindent}
  \caption{%
    Reconstruction resolutions required to achieve statistical indistinguishability between reconstructions corresponding reference trees for each phylometric across surveyed evolutionary conditions.
    Significance level $p<0.05$ under the Wilcoxon signed-rank test between samples of 30 replicates each is used as the threshold for statistical distinguishability.
    Phylometrics with looser reconstruction resolution thresholds (i.e., higher resolution percentages) are less sensitive to reconstruction error.
    White heat map tiles indicate that no surveyed reconstruction resolution threshold was sufficient to achieve indistinguishability from the reference tree with respect a particular phylometric.
  }
  \label{fig:reconstructed-tree-phylometrics-error-avida}
\end{figure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-error-sensitivity-analysis.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    % \begin{noindent}
    \centering
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=0+hue=quality-threshold+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{%
      gaussian mutation distribution at epoch 0 (generation 32,768)}
    \label{fig:reconstructed-tree-phylometrics-error-sensitivity-analysis:epoch0}
    % \end{noindent}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    % \begin{noindent}
    \centering
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=2+hue=quality-threshold+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{%
      gaussian mutation distribution at epoch 2 (generation 98,304)}
    \label{fig:reconstructed-tree-phylometrics-error-sensitivity-analysis:epoch2}
    % \end{noindent}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    % \begin{noindent}
    \centering
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+hue=quality-threshold+mut_distn=np.random.exponential+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{%
      exponential mutation distribution}
    \label{fig:reconstructed-tree-phylometrics-error-sensitivity-analysis:exponential}
    % \end{noindent}
  \end{subfigure}
  \caption{%
    Sensitivity analysis results for reconstruction resolutions required to achieve statistical indistinguishability between reconstructions corresponding reference trees for each phylometric across surveyed evolutionary conditions.
    Significance level $p<0.05$ under the Wilcoxon signed-rank test between samples of 50 replicates each is used as the threshold for statistical distinguishability.
    Phylometrics with looser reconstruction resolution thresholds (i.e., higher resolution percentages) are less sensitive to reconstruction error.
    White heat map tiles indicate that no surveyed reconstruction resolution threshold was sufficient to achieve indistinguishability from the reference tree with respect a particular phylometric.
  }
  \label{fig:reconstructed-tree-phylometrics-error-sensitivity-analysis}
\end{figure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-error-spatial-nuisance-sensitivity-analysis.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    \centering
    % \begin{noindent}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=0+hue=quality-threshold+mut_distn=np.random.standard_normal+nuisance=spatial-structure+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{%
      gaussian mutation distribution at epoch 0 (generation 32,768)}
    \label{fig:reconstructed-tree-phylometrics-error-spatial-nuisance-sensitivity-analysis:epoch0}
    % \end{noindent}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    \centering
    % \begin{noindent}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=2+hue=quality-threshold+mut_distn=np.random.standard_normal+nuisance=spatial-structure+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{%
      gaussian mutation distribution at epoch 2 (generation 98,304)}
    \label{fig:reconstructed-tree-phylometrics-error-spatial-nuisance-sensitivity-analysis:epoch2}
    % \end{noindent}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}
    \centering
    % \begin{noindent}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+hue=quality-threshold+mut_distn=np.random.exponential+nuisance=spatial-structure+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{%
    exponential mutation distribution at epoch 7 (generation 262,144)}
    \label{fig:reconstructed-tree-phylometrics-error-spatial-nuisance-sensitivity-analysis:exponential}
    % \end{noindent}
  \end{subfigure}
  \caption{%
    Sensitivity analysis results for reconstruction resolutions required to achieve statistical indistinguishability between reconstructions corresponding reference trees for each phylometric across surveyed evolutionary conditions with spatial structure (i.e., island count 1,024).
    Significance level $p<0.05$ under the Wilcoxon signed-rank test between samples of 50 replicates each is used as the threshold for statistical distinguishability.
    Phylometrics with looser reconstruction resolution thresholds (i.e., higher resolution percentages) are less sensitive to reconstruction error.
    White heat map tiles indicate that no surveyed reconstruction resolution threshold was sufficient to achieve indistinguishability from the reference tree with respect a particular phylometric.
  }
  \label{fig:reconstructed-tree-phylometrics-error-spatial-nuisance-sensitivity-analysis}
\end{figure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-error-spatial-nuisance.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+hue=quality-threshold+mut_distn=np.random.standard_normal+nuisance=spatial-structure+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \end{noindent}
  \caption{%
    Reconstruction resolutions required to achieve statistical indistinguishability between reconstructions corresponding reference trees for each phylometric across surveyed evolutionary conditions with spatial structure (i.e., island count 1,024).
    Significance level $p<0.05$ under the Wilcoxon signed-rank test between samples of 50 replicates each is used as the threshold for statistical distinguishability.
    Phylometrics with looser reconstruction resolution thresholds (i.e., higher resolution percentages) are less sensitive to reconstruction error.
    White heat map tiles indicate that no surveyed reconstruction resolution threshold was sufficient to achieve indistinguishability from the reference tree with respect a particular phylometric.
    See Supplementary Figure \ref{fig:reconstructed-tree-phylometrics-error-spatial-nuisance-sensitivity-analysis} for sensitivity analysis results.
  }
  \label{fig:reconstructed-tree-phylometrics-error-spatial-nuisance}
\end{figure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-error.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+hue=quality-threshold+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  % \end{noindent}
  \caption{%
    \textbf{Reconstruction resolutions required to achieve statistical indistinguishability between reconstructions and ground-truth reference trees.}
    Significance level $p<0.05$ under the Wilcoxon signed-rank test between samples of 50 replicates each is used as the threshold for statistical distinguishability.
    Phylometrics with looser reconstruction resolution thresholds (i.e., higher resolution percentages) are less sensitive to reconstruction error.
    White heat map tiles indicate that no surveyed reconstruction resolution threshold was sufficient to achieve indistinguishability from the reference tree with respect a particular phylometric.
    See Supplementary Figure \ref{fig:reconstructed-tree-phylometrics-error-sensitivity-analysis} for sensitivity analysis results.
  }
  \label{fig:reconstructed-tree-phylometrics-error}
\end{figure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-exponential.tex <==
\begin{sidewaysfigure*}
  \centering
  % \begin{noindent}
  \includegraphics[height=\textwidth,angle=-90]{binder/binder/teeplots/col=phylometric+epoch=7+mut_distn=np.random.standard_normal+row=regime+viz=boxplot+x=value+y=quality+ext=.pdf}
  % \end{noindent}
  \caption{%
    Sensitivity analysis result for distributions of phylometrics across surveyed reconstruction fidelities and surveyed evolutionary regimes.
    Sensitivity analysis condition is exponential mutation distribution at epoch 7 (generation 262,144).
    Sample sizes of $n=50$ replicates define each depicted distribution.
  }
  \label{fig:reconstructed-tree-phylometrics-exponential}
\end{sidewaysfigure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-progressive-heatmap-avida.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/epoch=0+mut_distn=default+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{Reference phylogeny.}
  \end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/epoch=0+mut_distn=default+resolution=100.0+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  \caption{1\% resolution reconstruction.}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/epoch=0+mut_distn=default+resolution=33.0+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  \caption{3\% resolution reconstruction.}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/epoch=0+mut_distn=default+resolution=10.0+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  \caption{10\% resolution reconstruction.}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/avida-individual/teeplots/epoch=0+mut_distn=default+resolution=3.0+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  \caption{30\% resolution reconstruction.}
\end{subfigure}

  \caption{
Tree phylometrics across surveyed evolutionary regimes, calculated on reconstructed and perfect-fidelity simulation phylogenetic records from Avida model.
Note that nonparametric effect size normalization caps out to 1.0/-1.0 past the point of complete disbributional nonoverlap.
For heatmap charts, +'s indicate small, medium, and large effect sizes using the Cliff's delta statistic and *'s indicate statistical significance at $\alpha = 0.05$ via Mann-Whitney U test.
  }
  \label{fig:reconstructed-tree-phylometrics-progressive-heatmap-avida}
\end{figure*}

==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-progressive-heatmap.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[b]{\textwidth}
    \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
    \caption{Reference phylogeny.}
  \end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+resolution=100.0+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  \caption{1\% resolution reconstruction.}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+resolution=30.0+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  \caption{3\% resolution reconstruction.}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+resolution=10.0+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  \caption{10\% resolution reconstruction.}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/epoch=7+mut_distn=np.random.standard_normal+resolution=3.0+viz=heatmap+x=regime+y=phylometric+ext=.pdf}
  \caption{30\% resolution reconstruction.}
\end{subfigure}

  \caption{
Tree phylometrics across surveyed evolutionary regimes, calculated on reconstructed and perfect-fidelity simulation phylogenetic records from simple model.
Note that nonparametric effect size normalization caps out to 1.0/-1.0 past the point of complete disbributional nonoverlap.
For heatmap charts, +'s indicate small, medium, and large effect sizes using the Cliff's delta statistic and *'s indicate statistical significance at $\alpha = 0.05$ via Mann-Whitney U test.
Results from simple model are for standard experimental conditions: gaussian mutation distribution at epoch 7 (generation 262,144).
  }
  \label{fig:reconstructed-tree-phylometrics-progressive-heatmap}
\end{figure*}

==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-with-spatial-nuisance-epoch0.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=7+mut_distn=np.random.standard_normal+nuisance=spatial-structure+row=regime+viz=boxplot+x=value+y=quality+ext=.pdf}
  % \end{noindent}
  \caption{%
    Sensitivity analysis result for distributions of phylometrics across surveyed reconstruction fidelities for evolutionary regimes with underlying spatial structure (i.e., 1,024 niches).
    Sensitivity analysis condition is gaussian mutation distribution at epoch 0 (generation 32,768).
    Sample sizes of $n=50$ replicates define each depicted distribution.
  }
  \label{fig:reconstructed-tree-phylometrics-with-spatial-nuisance-epoch0}
\end{figure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-with-spatial-nuisance-epoch2.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=2+mut_distn=np.random.standard_normal+nuisance=spatial-structure+row=regime+viz=boxplot+x=value+y=quality+ext=.pdf}
  % \end{noindent}
  \caption{%
    Sensitivity analysis result for distributions of phylometrics across surveyed reconstruction fidelities for evolutionary regimes with underlying spatial structure (i.e., 1,024 niches).
    Sensitivity analysis condition is gaussian mutation distribution at epoch 2 (generation 98,304).
    Sample sizes of $n=50$ replicates define each depicted distribution.
  }
  \label{fig:reconstructed-tree-phylometrics-with-spatial-nuisance-epoch2}
\end{figure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-with-spatial-nuisance-exponential.tex <==
\begin{figure*}
  % \begin{noindent}
  \centering
  \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=7+mut_distn=np.random.exponential+nuisance=spatial-structure+row=regime+viz=boxplot+x=value+y=quality+ext=.pdf}
  % \end{noindent}
  \caption{%
    Sensitivity analysis result for distributions of phylometrics across surveyed reconstruction fidelities for evolutionary regimes with underlying spatial structure (i.e., 1,024 niches).
    Sensitivity analysis condition is exponential mutation distribution at epoch 7 (generation 262,144).
    Sample sizes of $n=50$ replicates define each depicted distribution.
  }
  \label{fig:reconstructed-tree-phylometrics-with-spatial-nuisance-exponential}
\end{figure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics-with-spatial-nuisance.tex <==
\begin{figure*}
  \centering
  % \begin{noindent}
  \includegraphics[width=\textwidth]{binder/binder/teeplots/col=phylometric+epoch=7+mut_distn=np.random.standard_normal+nuisance=spatial-structure+row=regime+viz=boxplot+x=value+y=quality+ext=.pdf}
  % \end{noindent}
  \caption{%
    Distributions of phylometrics across surveyed reconstruction fidelities for evolutionary regimes with underlying spatial structure (i.e., 1,024 niches).
    Results are for standard experimental conditions: gaussian mutation distribution at epoch 7 (generation 262,144).
    See Figures \labelcref{fig:reconstructed-tree-phylometrics-with-spatial-nuisance-epoch0,fig:reconstructed-tree-phylometrics-with-spatial-nuisance-epoch2,fig:reconstructed-tree-phylometrics-with-spatial-nuisance-exponential} for results under sensitivity analysis conditions.
    Sample sizes of $n=50$ replicates define each depicted distribution.
  }
  \label{fig:reconstructed-tree-phylometrics-with-spatial-nuisance}
\end{figure*}


==> bindertex-evolutionary-inference/fig/reconstructed-tree-phylometrics.tex <==
\begin{sidewaysfigure*}
  \centering
  % \begin{noindent}
  \includegraphics[height=\textwidth,angle=-90]{binder/binder/avida-individual/teeplots/col=phylometric+epoch=0+mut_distn=default+row=regime+viz=boxplot+x=value+y=quality+ext=.pdf}
  % \end{noindent}
  \caption{%
    Distributions of phylometrics across surveyed reconstruction fidelities and evolutionary regimes.
    Results are for standard experimental conditions: gaussian mutation distribution at epoch 7 (generation 262,144).
    See Figures \labelcref{fig:reconstructed-tree-phylometrics-epoch0,fig:reconstructed-tree-phylometrics-epoch2,fig:reconstructed-tree-phylometrics-exponential} for results under sensitivity analysis conditions.
    Sample sizes $n=50$.
  }
  \label{fig:reconstructed-tree-phylometrics}
\end{sidewaysfigure*}


==> bindertex-evolutionary-inference/lib/dependencies.tex <==
\usepackage{adjustbox}
\usepackage{algorithmic}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{array}
\usepackage{authblk}
\usepackage{bibunits}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{csvsimple}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref,cleveref}
\usepackage{import}
\usepackage{natbib}[sort]
\usepackage{rotating}
\usepackage[moderate]{savetrees}
\usepackage{siunitx}
\usepackage{subcaption}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{lib/alifeconf}
\usepackage{orcidlink}
\usepackage{pdflscape,longtable}
\usepackage{listings}
\usepackage{placeins}
\usepackage{pythonhighlight}


==> bindertex-evolutionary-inference/lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
  % adapted from https://tex.stackexchange.com/a/33577
  \ifdefined\DISSERTATION
  \else
    #1
  \fi
}


==> bindertex-evolutionary-inference/lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
  % adapted from https://tex.stackexchange.com/a/33577
  \ifdefined\DISSERTATION%
    #1%
  \else%
  \fi
  asdf
}


==> bindertex-evolutionary-inference/lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
\def\importpath{\import@path}
\makeatother


==> bindertex-evolutionary-inference/lib/pragmaonce.tex <==
% pragma once, adapted from https://tex.stackexchange.com/a/195173
\makeatletter
\let\pragma@iinput=\@iinput
\def\@iinput#1{\xdef\@pragmafile{#1}\pragma@iinput{#1} }
\def\@pragmafile{default}
\def\pragmaonce{%
  \csname pragma@\@pragmafile\endcsname
  \global\expandafter\let \csname pragma@\@pragmafile\endcsname = \endinput
}
\makeatother


==> bindertex-evolutionary-inference/lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> bindertex-evolutionary-inference/lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> bindertex-evolutionary-inference/tab/phylostatistics-comparison-between-regimes-allpairs-spatial-nuisance-wilcox.tex <==
\providecommand{\thecaption}{
  All-pairs two-tailed Wilcoxon signed-rank comparisons of phylometrics between surveyed evolutionary regimes with spatial structure (i.
  e., island count 1,024).
  Phylometrics were calculated on perfect-fidelity reference trees.
  All-pairs comparisons within each sensitivity analysis condition are provided.
  Sample size $n=50$ for each population.
  Reported $p$ values are not corrected for multiple comparisons.
  Instead, a Bonferoni-corrected significance threshold of $5.26 \times 10^{-4}$ was used.
}

\begin{landscape}
  \csvstyle{myTableStyle}{
    longtable=c c c c c c c c,
    before reading=\footnotesize,
    table head=\toprule evolutionary regime 1 & evolutionary regime 2 & $n$ & Phylometric & Statistic & $p$ & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }\endfoot\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }
    \label{tab:phylostatistics-comparison-between-regimes-allpairs-spatial-nuisance-wilcox}\endlastfoot,
    head to column names,
    respect all,
  }

  \csvreader[myTableStyle]{binder/binder/outdata/a=phylostatistics-comparison-between-regimes-allpairs-spatial-nuisance-wilcox+ext=.csv}{}{\csvlinetotablerow}
\end{landscape}


==> bindertex-evolutionary-inference/tab/phylostatistics-comparison-between-regimes-allpairs-wilcox.tex <==
\providecommand{\thecaption}{
  All-pairs two-tailed Wilcoxon signed-rank comparisons of phylometrics between surveyed evolutionary regimes.
  Phylometrics were calculated on perfect-fidelity reference trees.
  All-pairs comparisons within each sensitivity analysis condition are provided.
  Sample size $n=50$ for each population.
  Reported $p$ values are not corrected for multiple comparisons.
  Instead, a Bonferoni-corrected significance threshold of $1.49 \times 10^{-4}$ was used.
}

\begin{landscape}
  \csvstyle{myTableStyle}{
    longtable=c c c c c c c c,
    before reading=\footnotesize,
    table head=\toprule evolutionary regime 1 & evolutionary regime 2 & $n$ & Phylometric & Statistic & $p$ & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }\endfoot\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }
    \label{tab:phylostatistics-comparison-between-regimes-allpairs-wilcox}\endlastfoot,
    head to column names,
    respect all,
  }

  \csvreader[myTableStyle]{binder/binder/outdata/a=phylostatistics-comparison-between-regimes-allpairs-wilcox+ext=.csv}{}{\csvlinetotablerow}
\end{landscape}


==> bindertex-evolutionary-inference/tab/phylostatistics-comparison-between-regimes-kwallis-avida.tex <==
\providecommand{\thecaption}{
  Kruskal-Wallis one-way analysis of variance tests for nonequivalence of distributions for each phylometric among surveyed evolutionary regimes.
  Phylometrics were calculated on perfect-fidelity reference trees.
  Kruskal-Wallis test results within each sensitivity analysis condition are provided.
  Sample size $n=30$ for each population, with $N=7$ populations (i.e., evolutionary regimes) compared within each sensitivity analysis condition.
}

\csvstyle{myTableStyle}{
  longtable=c c c c c c c c,
  before reading=\footnotesize,
  table head=\toprule $n$ & $N$ & Phylometric & Statistic & $p$ & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }\endfoot\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }\endlastfoot,
  after reading=
  \label{tab:phylostatistics-comparison-between-regimes-kwallis},
  head to column names,
  respect all,
}

\csvreader[myTableStyle]{binder/binder/avida-individual/outdata/a=phylostatistics-comparison-between-regimes-kwallis+ext=.csv}{}{\csvlinetotablerow}


==> bindertex-evolutionary-inference/tab/phylostatistics-comparison-between-regimes-kwallis.tex <==
\providecommand{\thecaption}{
  Kruskal-Wallis one-way analysis of variance tests for nonequivalence of distributions for each phylometric among surveyed evolutionary regimes for Avida experiments.
  Phylometrics were calculated on perfect-fidelity reference trees.
  Kruskal-Wallis test results within each sensitivity analysis condition are provided.
  Sample size $n=50$ for each population, with $N=7$ populations (i.e., evolutionary regimes) compared within each sensitivity analysis condition.
}

\csvstyle{myTableStyle}{
  longtable=c c c c c c c c,
  before reading=\footnotesize,
  table head=\toprule $n$ & $N$ & Phylometric & Statistic & $p$ & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }\endfoot\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }\endlastfoot,
  after reading=
  \label{tab:phylostatistics-comparison-between-regimes-kwallis-avida},
  head to column names,
  respect all,
}

\csvreader[myTableStyle]{binder/binder/outdata/a=phylostatistics-comparison-between-regimes-kwallis+ext=.csv}{}{\csvlinetotablerow}


==> bindertex-evolutionary-inference/tab/phylostatistics-comparison-between-regimes-spatial-nuisance-kwallis-avida.tex <==
\providecommand{\thecaption}{
  Kruskal-Wallis one-way analysis of variance tests for nonequivalence of distributions for each phylometric among surveyed evolutionary regimes with spatial structure (i.
  e., island count 1,024) for Avida experiments.
  Phylometrics were calculated on perfect-fidelity reference trees.
  Kruskal-Wallis test results within each sensitivity analysis condition are provided.
  Sample size $n=30$ for each population, with $N=4$ populations (i.e., evolutionary regimes) compared within each sensitivity analysis condition.
}

\csvstyle{myTableStyle}{
  longtable=c c c c c c c c,
  before reading=\footnotesize,
  table head=\toprule $n$ & $N$ & Phylometric & Statistic & $p$ & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }\endfoot\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }
  \label{tab:phylostatistics-comparison-between-regimes-spatial-nuisance-kwallis-avida}\endlastfoot,
  head to column names,
  respect all,
}

\csvreader[myTableStyle]{binder/binder/avida-individual/outdata/a=phylostatistics-comparison-between-regimes-spatial-nuisance-kwallis+ext=.csv}{}{\csvlinetotablerow}


==> bindertex-evolutionary-inference/tab/phylostatistics-comparison-between-regimes-spatial-nuisance-kwallis.tex <==
\providecommand{\thecaption}{
  Kruskal-Wallis one-way analysis of variance tests for nonequivalence of distributions for each phylometric among surveyed evolutionary regimes with spatial structure (i.
  e., island count 1,024).
  Phylometrics were calculated on perfect-fidelity reference trees.
  Kruskal-Wallis test results within each sensitivity analysis condition are provided.
  Sample size $n=50$ for each population, with $N=4$ populations (i.e., evolutionary regimes) compared within each sensitivity analysis condition.
}

\csvstyle{myTableStyle}{
  longtable=c c c c c c c c,
  before reading=\footnotesize,
  table head=\toprule $n$ & $N$ & Phylometric & Statistic & $p$ & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }\endfoot\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }
  \label{tab:phylostatistics-comparison-between-regimes-spatial-nuisance-kwallis}\endlastfoot,
  head to column names,
  respect all,
}

\csvreader[myTableStyle]{binder/binder/outdata/a=phylostatistics-comparison-between-regimes-spatial-nuisance-kwallis+ext=.csv}{}{\csvlinetotablerow}


==> bindertex-evolutionary-inference/tab/phylostatistics-comparison-between-resolutions-allpairs-wilcox-spatial-nuisance.tex <==
\providecommand{\thecaption}{
  Two-tailed Wilcoxon signed-rank comparisons between phylometric distributions for reconstructed trees and corresponding perfect-fidelity reference trees.
  Comparisons were performed separately for each surveyed reconstruction fidelity, evolutionary regime, and phylometric.
  Evolutionary regimes described here all included spatial structure (i.e., island count 1,024).
  Sample size $n=50$ for each population.
  Reported $p$ values are not corrected for multiple comparisons, in order to conservatively detect possible phylometric bias from reconstruction error.
}

\begin{landscape}
  \csvstyle{myTableStyle}{
    longtable=c c c c c c c c,
    before reading=\footnotesize,
    table head=\toprule Reconstruction Fidelity & $n$ & Phylometric & Statistic & $p$ & Evolutionary Regime & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }\endfoot\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }
    \label{tab:phylostatistics-comparison-between-resolutions-allpairs-wilcox-spatial-nuisance}\endlastfoot,
    head to column names,
    respect all,
  }

  \csvreader[myTableStyle]{binder/binder/outdata/a=phylostatistics-comparison-between-resolutions-allpairs-wilcox-spatial-nuisance+ext=.csv}{}{\csvlinetotablerow}
\end{landscape}


==> bindertex-evolutionary-inference/tab/phylostatistics-comparison-between-resolutions-allpairs-wilcox.tex <==
\providecommand{\thecaption}{
  Two-tailed Wilcoxon signed-rank comparisons between phylometric distributions for reconstructed trees and corresponding perfect-fidelity reference trees.
  Comparisons were performed separately for each surveyed reconstruction fidelity, evolutionary regime, and phylometric.
  Sample size $n=50$ for each population.
  Reported $p$ values are not corrected for multiple comparisons, in order to conservatively detect possible phylometric bias from reconstruction error.
}

\begin{landscape}
  \csvstyle{myTableStyle}{
    longtable=c c c c c c c c,
    before reading=\footnotesize,
    table head=\toprule Reconstruction Fidelity & $n$ & Phylometric & Statistic & $p$ & Evolutionary Regime & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
    \caption{
      \thecaption
    }\endfoot\bottomrule\\[-1em]\caption{%
      \thecaption
    }
    \label{tab:phylostatistics-comparison-between-resolutions-allpairs-wilcox}\endlastfoot,
    head to column names,
    respect all,
  }

  \csvreader[myTableStyle]{binder/binder/outdata/a=phylostatistics-comparison-between-resolutions-allpairs-wilcox+ext=.csv}{}{\csvlinetotablerow}
\end{landscape}


==> bindertex-evolutionary-inference/tab/reconstruction-error-comparisons-between-regimes.tex <==
\providecommand{\thecaption}{
  Kruskal-Wallis one-way analysis of variance tests for nonequivalence of reconstruction error distributions among surveyed evolutionary regimes.
  Comparisons were performed independently within each sensitivity analysis condition and reconstruction fidelities.
  Error reported as both quartet and triplet distance between reconstructed tree and corresponding reference tree.
  Sample size $n=50$ for each population, with $N=7$ populations (i.e., evolutionary regimes) compared within each sensitivity analysis condition.
}

\csvstyle{myTableStyle}{
  longtable=c c c c c c c c,
  before reading=\scriptsize,
  table head=\toprule $n$ & $N$ & Tree Distance Metric & Statistic & $p$ & Reconstruction Fidelity & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }\endfoot
  \label{tab:reconstruction-error-comparisons-between-regimes},
  head to column names,
  respect all,
}

\csvreader[myTableStyle]{binder/binder/outdata/a=reconstruction-error-comparisons-between-regimes+ext=.csv}{}{\csvlinetotablerow}


==> bindertex-evolutionary-inference/tab/reconstruction-error-comparisons-between-resolutions.tex <==
\providecommand{\thecaption}{
  Kruskal-Wallis one-way analysis of variance tests for nonequivalence of reconstruction error distributions among reconstruction fidelities.
  Comparisons were performed independently within each sensitivity analysis condition and evolutionary regime.
  Error reported as both quartet and triplet distance between reconstructed tree and corresponding reference tree.
  Sample size $n=50$ for each population, with $N=4$ populations (i.e., reconstruction fidelities) compared within each sensitivity analysis condition.
}

\csvstyle{myTableStyle}{
  longtable=c c c c c c c c,
  before reading=\scriptsize,
  table head=\toprule $n$ & $N$ & Tree Distance Metric & Statistic & $p$ & Evolutionary Regime & Epoch & Mutation Distribution\\ \midrule\endhead\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }\endfoot\bottomrule\\[-1em]
  \caption{%
    \thecaption
  }
  \label{tab:reconstruction-error-comparisons-between-resolutions}\endlastfoot,
  head to column names,
  respect all,
}

\csvreader[myTableStyle]{binder/binder/outdata/a=reconstruction-error-comparisons-between-resolutions+ext=.csv}{}{\csvlinetotablerow}


==> bindertex-evolutionary-inference/tab/tree-reconstruction-quality-quartet-summary-statistics.tex <==
\providecommand{\thecaption}{
  Summary statistics for reconstruction error across reconstruction fidelity levels and evolutionary conditions, measured as quartet distance between reconstructions and corresponding reference trees.
}

\begin{landscape}
  \csvstyle{myTableStyle}{
    longtable=c c c c c c c c,
    before reading=\scriptsize,
    table head=\toprule evolutionary regime & reconstruction quality & sensitivity analysis conditions & quartet dist mean & quartet dist median & quartet dist std & quartet dist max\\ \midrule\endhead\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }\endfoot\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }
    \label{tab:tree-reconstruction-quality-quartet-summary-statistics}\endlastfoot,
    head to column names,
    respect all,
  }

  \csvreader[myTableStyle]{binder/binder/outdata/a=tree-reconstruction-quality-quartet-summary-statistics.csv}{}{\csvlinetotablerow}
\end{landscape}


==> bindertex-evolutionary-inference/tab/tree-reconstruction-quality-triplet-summary-statistics.tex <==
\providecommand{\thecaption}{
  Summary statistics for reconstruction error across reconstruction fidelity levels and evolutionary conditions, measured as triplet distance between reconstructions and corresponding reference trees.
}

\begin{landscape}
  \csvstyle{myTableStyle}{
    longtable=c c c c c c c c,
    before reading=\scriptsize,
    table head=\toprule evolutionary regime & reconstruction quality & sensitivity analysis conditions & triplet dist mean & triplet dist median & triplet dist std & triplet dist max\\ \midrule\endhead\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }\endfoot\bottomrule\\[-1em]
    \caption{%
      \thecaption
    }
    \label{tab:tree-reconstruction-triplet-summary-statistics}\endlastfoot,
    head to column names,
    respect all,
  }

  \csvreader[myTableStyle]{binder/binder/outdata/a=tree-reconstruction-quality-triplet-summary-statistics.csv}{}{\csvlinetotablerow}

\end{landscape}


==> bindertex-evolutionary-inference/text/acknowledgement.tex <==
\section*{Acknowledgment}

This research was supported in part by NSF grants DEB-1655715 and DBI-0939454 as well as by Michigan State University through the computational resources provided by the Institute for Cyber-Enabled Research.
This material is based upon work supported by the National Science Foundation Graduate Research Fellowship under Grant No. DGE-1424871.
Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.
This material is based upon work supported by the Eric and Wendy Schmidt AI in Science Postdoctoral Fellowship, a Schmidt Futures program.

==> bindertex-evolutionary-inference/text/body.tex <==
\input{text/body/abstract.tex}

\input{text/body/introduction.tex}

\input{text/body/methods.tex}

\input{text/body/results-and-discussion.tex}

\input{text/body/conclusion.tex}


==> bindertex-evolutionary-inference/text/body/abstract.tex <==
% Here, we assess the potential of phylogenetic analyis as a means to study fundamental, universal evolutionary dynamics --- ecology, selection pressure, and spatial structure.
% Specifically, we consider the following questions,
% \begin{enumerate}
%   \item Do these dynamics leave a detectable signatures in phylogenetic structure?
%   \item If so, to what extent are these dynamics' signatures discernable from one another?
%   \item To what extent do the structure of these dynamics' signatures generalize across evolutionary systems?
% \end{enumerate}

% We use simulation experiments to investigate these questions.
% To quantify organism-level phylogenetic structure within asexual populations, we measure phylogenetic summary statistics from both a minimalistic, forward-time simulation and a rich artificial life system \citep{ofria2004avida}.
% We additionaly contrast organism-level simulation with species phylogenies generated from a population-level simulation \citep{hagen2021gen3sis}.



 % for observing
 % Ultimately, these contributions advance phylogenetic observation as a promising technique for key evolutionary drivers in large-scale populations within closer reach.

%As digital evolution systems grow in scale and complexity, observing and interpreting their evolutionary dynamics will become increasingly challenging.
%Distributed and parallel computing, in particular, introduce obstacles to maintaining the high level of observability that makes digital evolution a powerful experimental tool.
%Phylogenetic analyses represent a promising tool for drawing inferences from digital evolution experiments at scale.
%Recent work has introduced promising techniques for decentralized phylogenetic inference in parallel and distributed digital evolution systems.
%However, foundational phylogenetic theory necessary to apply these techniques to characterize evolutionary dynamics is lacking.
%Here, we lay the groundwork for practical applications of distributed phylogenetic tracking in three ways: 1) we present an improved technique for reconstructing phylogenies from tunably-precise genome annotations, 2) we begin the process of identifying how the signatures of various evolutionary dynamics manifest in phylogenetic metrics, and 3) we quantify the impact of reconstruction-induced imprecision on phylogenetic metrics.

\begin{abstract}
  Evolutionary dynamics are shaped by a variety of fundamental, generic drivers, including spatial structure, ecology, and selection pressure.
  These drivers impact the trajectory of evolution, and have been hypothesized to influence phylogenetic structure.
  For instance, they can help explain natural history, steer behavior of contemporary evolving populations, and influence efficacy of application-oriented evolutionary optimization.
  Likewise, in inquiry-oriented artificial life systems, these drivers constitute key building blocks for open-ended evolution.
  Here, we set out to assess (1) if spatial structure, ecology, and selection pressure leave detectable signatures in phylogenetic structure, (2) the extent, in particular, to which ecology can be detected and discerned in the presence of spatial structure, and (3) the extent to which these phylogenetic signatures generalize across evolutionary systems.
  To this end, we analyze phylogenies generated by manipulating spatial structure, ecology, and selection pressure within three computational models of varied scope and sophistication.
  We find that selection pressure, spatial structure, and ecology have characteristic effects on phylogenetic metrics, although these effects are complex and not always intuitive.
  Signatures have some consistency across systems when using equivalent taxonomic unit definitions (e.g., individual, genotype, species).
  Further, we find that sufficiently strong ecology can be detected in the presence of spatial structure.
  We also find that, while low-resolution phylogenetic reconstructions can bias some phylogenetic metrics, high-resolution reconstructions recapitulate them faithfully.
  Although our results suggest potential for evolutionary inference of spatial structure, ecology, and selection pressure through phylogenetic analysis, further methods development is needed to distinguish these drivers' phylometric signatures from each other and to appropriately normalize phylogenetic metrics.
   With such work, phylogenetic analysis could provide a versatile toolkit to study large-scale evolving populations.
\end{abstract}


==> bindertex-evolutionary-inference/text/body/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

Because phylogenies are an abstraction that generalizes across all evolutionary processes, phylogenetic analysis can be applied across a breadth of biological and artificial life systems.
Consequently, a broad set of cross-disciplinary use cases exist for inferring the processes that shaped a phylogeny by quantifying its topology.
Indeed, extraction of information about evolutionary dynamics from phylogenetic history has been a longstanding and productive theme in evolutionary biology \citep{pagel1997inferring}.
This work seeks to contribute in that vein, by establishing foundations necessary to assess three fundamental evolutionary drivers --- spatial structure, ecology, and selection pressure --- in complex, distributed evolving populations.

First, we investigated the strength and character of structural signatures in phylogenetic histories left by selection pressure, ecology, and spatial population structure.
These drivers induced readily detectable effects across our suite of four surveyed phylometrics.
These effects were generally consistent across surveyed individual-level phylogenies, but differed notably under genotype-level tracking and under species-level simulation.
Although the directions of phylometric effects were generally consistent across treatments expected to increase phylogenetic richness (i.e., weak selection, ecologies, and spatial structure), effect significance/size for particular phylometrics differed among some treatments.
Compared to results from the simple model, which was amenable to strong treatment manipulations, the more sophisticated Avida model system expressed fewer phylometric effects between treatments.

Compared to spatial structure and selection pressure, drivers designed to induce ecological coexistence exerted relatively muted, sparse effects on phylogenetic metrics.
However, follow-up experiments with both individual-level model systems revealed that phylometric signatures can remain detectable under background conditions of spatial population structure.
Interactions, though, are sometimes surprising.
A notable example is the reduced mean pairwise distance observed in Avida under conditions combining spatial structure and ecology, but not in the baseline ecology treatment.
These results highlight the complexity of how interacting evolutionary dynamics impact phylogenetic structure.
Even a single dynamic in isolation can influence phylometrics in opposite directions.
For instance, we found that changes to selection pressure in either direction significantly reduced trees' Colless-like index under the simple model.

Comparison of phylometrics from perfect-fidelity trees against corresponding reconstructions revealed that phylometric statistics differed in sensitivity to reconstruction error introduced by hereditary stratigraphy-based tracking.
% TODO summarize specific examples as (i.e., metric for this vs. that)
Colless-like index and mean pairwise distance were more sensitive, and in some conditions, reconstruction persisted at even 1\% reconstruction resolution.
On the other hand, mean evolutionary distinctiveness and sum pairwise distance were particularly robust to reconstruction error, with no bias detected even at 33\% resolution reconstruction.
Results suggest 3\% reconstruction resolution as a reasonable ballpark parameterization for applications of hereditary stratigraphy with downstream phylogenetic analysis.
Where it did occur, the sign effect of phylometric bias was consistent, which might simplify considerations to account for it in experiments.

Our findings identify key next steps necessary for development of rigorous phylogenetic assays to test for key evolutionary drivers.
Because treatments did not induce widespread opposite-sign effects, our results do not indicate a straightforward, qualitative approach to disambiguate drivers' signatures.
Future work should survey comprehensive panels of phylometrics, which might provide a stronger foothold to this end \citep{tuckerGuidePhylogeneticMetrics2017}.
Alternately, more sophisticated quantitative approaches leveraging differential effect size ratios may be fruitful.
Possibilities include application of machine learning techniques over broad phylometric panels \citep{voznica2022deep} or even inference directly over phylogenetic structure itself via graph neural networks and related methods \citep{lajaaiti2023comparison}.
The capability of artificial life approaches to generate high-quality data sets with high replication counts will be a significant asset to such work.
More information could be harnessed by incorporating trait data \citep{nozoe2017inferring} or by using time-sampled phylogenies \citep{volz2013viral}, which would include information about ``ghost'' lineages that have extincted at earlier time points.

Additionally, robust normalization methods will be crucial to enable meaningful comparisons between phylogenies differing in (1) population size, (2) population subsampling level, (3) depth of evolutionary history, and (4) demographic characteristics of organism life histories.
Despite some substantial work on this front \citep{shao1990tree,mir2018sound}, significant challenges remain.
It is worth noting that most analysis reported here normalizes to phylometric values sampled from ``plain'' evolutionary regimes, thereby implicitly depending on the availability of such data.
However, stripped-down baseline condition experiments may not always be possible, especially in biological model systems.
Extensive, likely sophisticated, considerations would be necessary to establish \textit{a priori} phylometric value predictions that could be compared against instead of testing against empirical values.
Finally, as evidenced in our experiments, reconstruction error can systematically bias phylometric values.
In scenarios where reconstruction error is unavoidable, additional normalizations may be necessary.
However, it is promising that some phylometrics appear thoroughly robust to reconstruction error and, in other cases, sufficient reconstruction accuracy might be achieved to obviate error bias.

The overriding objective of work presented here is to equip biologists and computational researchers with capability to investigate fundamental evolutionary drivers within large-scale evolving populations.
To this end, methodology must advance hand-in-hand with the software infrastructure required to put it into practice.
Artificial life experiments, specifically, tend to require particular instrumentation to collect phylogenetic histories, and we have been active in making general-use plug-and-play solutions available freely through the Python Packaging Index \citep{moreno2022hstrat,dolson2024phylotrackpy}.
As each field develops, artificial life will benefit greatly from domain-specific software and methods developed within traditional evolutionary bioinformatics and, we hope, vice versa.

% Together, our findings support development of more rigorous phylogenetic assays that might eventually be capable of identifying the evolutionary conditions that produced a phylogeny.
% look forward to continuing to push forward the

% Ultimately, the goal is to develop methodology that can be put into practice to increase the power of digital evolution and artificial life systems as experimental model systems.
% In addition to , this objective hinges on software availability.

% Production-ready software implementation available via the Python Packaging Index.
% C++ bindings for hereditary stratigraph genome annotation are under active development and will be released imminently.
% We are eager to collaborate to , and to contribute to developing large-scale (parallel and distributed) artificial life systems as an experimental tool



% Much future work

% \begin{itemize}
% \item better theory and methodology for null models; in this work we performed comparisons between replicates with different system parameterizations; in many contexts, this might not be practical or possible
% \item leverage these foundational observational findings to devise systematic testing protocols to identify evolutionary dynamics
% % \item incorporate information about ancestral state through ``fossils'' and see how well/accurately they can be tied into the tree of extant organisms (initial signs are good; unit tests with reconstructions from organisms sampled from different phylogenetic depths)
% % \item understanding complications of sexual recombinaton

% \end{itemize}

% Ultimately, the goal is to develop methodology that can be put into practice to increase the power of digital evolution and artificial life systems as experimental model systems.
% In addition to , this objective hinges on software availability.

% Production-ready software implementation available via the Python Packaging Index.
% C++ bindings for hereditary stratigraph genome annotation are under active development and will be released imminently.
% We are eager to collaborate to , and to contribute to developing large-scale (parallel and distributed) artificial life systems as an experimental tool

% recap work and findings
% In this paper, we focus on
% \begin{enumerate}
% \item need to be able to do fast, accurate tree reconstructions for very large distributed populations can efficiently create high-quality phylogenetic reconstructions for population sizes as large as 32,768
% \item need to understand the relationship between evolutionary dynamics and phylogenetic metrics
% \item
% \item nuisance factors of spatial structure and phylogenetic reconstruction error accompanying large-scale parallel and distributed digital evolution systems.

% \begin{enumerate}
% \item how much precision is required for accurate phylogenetic metrics?
% \item if bias is introduced, what type of bias (so could still detect "conservatively")
% \end{enumerate}
% \end{enumerate}


==> bindertex-evolutionary-inference/text/body/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Within evolutionary biology, the structure of ancestry relationships among organisms within an evolving system is described as their ``phylogeny.''
Phylogenies detail the sequence of historical lineage-branching events that gave rise to contemporary populations.
Most obviously, the phylogenetic record can reveal the ordering and timing of particular contingencies (e.g., trait originations, population separations) that gave rise to current populations \citep{pagel1999inferring,arbogast2002estimating}.
For instance, phylogenies reconstructed from fungal gene sequences suggest frequent switching of nutritional sources and that spore-dispersal mechanisms have multiple independent origins \citep{james2006reconstructing}.

However, phylogenetic analyses can also test more general hypotheses about underlying evolutionary dynamics.
Rather than seeking to detect specific events, researchers using phylogenies for this purpose instead measure structural patterns that may be indicative of different evolutionary regimes.
For instance, analysis of the counts of coexisting lineages over time has been used to detect density-dependent changes in speciation rate \citep{rabosky2008density}, which can be interpreted as an indication of transition away from niche expansion due to lessening availability of ecological opportunity.

Indeed, methods to infer underlying evolutionary dynamics from phylogenetic structure are increasingly harnessed for tangible, impactful applications.
In evolutionary oncology, for example, phylogenetic analysis has been used to quantify patterns of tumor evolution \citep{scottInferringTumorProliferative2020,lewinsohnStatedependentEvolutionaryModels2023}.
Likewise, pathogen phylogenies have been studied to identify dynamics of epidemiological spread of Ebola and HIV \citep{giardina2017inference,saulnier2017inferring,voznica2022deep}.
Phylogenetic information also has a long history of helping identify policy priorities for ecological conservation \citep{forestPreservingEvolutionaryPotential2007}.

In computational evolutionary systems, phylogenetic structure metrics are a powerful tool for summarizing evolutionary history \citep{dolson2020interpreting}.
These analyses can help digital systems further our knowledge of biology, but they are also directly valuable for learning about digital systems themselves.
Notably, within the realm of artificial life research, phylogeny-based metrics have been proposed to identify hallmarks of open-ended evolution \citep{dolson2019modes}.
They have also been used to understand evolutionary trajectories that lead to outcomes of interest \citep{lenskiEvolutionaryOriginComplex2003,lalejiniEvolutionaryOriginsPhenotypic2016,johnsonEndosymbiosisBustInfluence2022a}.
For evolution-inspired optimization algorithms, phylogeny-based metrics have been used to predict which runs of evolutionary computation will be successful \citep{hernandezWhatCanPhylogenetic2022a,shahbandeganUntanglingPhylogeneticDiversity2022a,ferguson2023potentiating} and even proactively guide artificial selection algorithms \citep{lalejini2024phylogeny,burke2003increased}.
% @ELD: Maybe cite Austin's ALife paper here too, once it's citable

Here, we assess the potential of phylogenetic analysis as a means to study fundamental, universal evolutionary dynamics --- ecology, selection pressure, and spatial structure.
Specifically, we consider the following questions,
\begin{enumerate}
  \item Do these dynamics leave detectable signatures in phylogenetic structure?
  \item If so, to what extent are these dynamics' signatures discernable from one another?
  \item To what extent do the structure of these dynamics' signatures generalize across evolutionary systems?
\end{enumerate}

We use \textit{in silico} experiments to investigate these questions, and test across two levels of taxonomic abstraction.
To quantify phylogenetic structure at organism-level abstraction --- meaning that phylogeny is represented at the granularity of individual parent-child relationships --- we use both a minimalistic, forward-time simulation and a rich artificial life system \citep{ofria2004avida}.
In contrast, at species-level abstraction (i.e. species trees), we used a population-level simulation designed to study origins of biodiversity \citep{hagen2021gen3sis}.

A major strength of simulation experiments for this purpose is that they provide exact ground-truth phylogenies due to their perfectly observable evolutionary history.
However, for \textit{in vivo} systems perfect phylogeny tracking is not typically possible. Although new techniques are making increasingly high-fidelity lineage tracking possible in some experiments \citep{nozoe2017inferring,woodworth2017building}, phylogenies are still usually estimated from naturally-occuring biosequence data.
Moreover, as digital evolution systems scale, issues of data loss and centralization overhead make perfect tracking at best inefficient and at worst untenable.
Thus, some systems will likely need to adopt a decentralized, reconstruction-based approach similar to biological data \citep{moreno2024analysis}, which can be achieved through the recently-developed ``hereditary stratigraphy'' methodology \citep{moreno2022hstrat}.

Effective use of phylogenetic metrics in scenarios where exact phylogenies are not available requires understanding of potential confounding effects from inaccuracies introduced by reconstruction.
However, it is in precisely such scenarios where the new capabilities to characterize evolutionary dynamics could have the largest impact; large-scale systems can produce an intractable quantity of data, making phylometrics valuable as summary statistics of the evolutionary process \citep{dolson2020interpreting}.
In particular, methods are needed to handle large-scale artificial life systems where complete, perfect visibility is not feasible and evolution operates according to implicit, contextually-dependent fitness dynamics \citep{moreno2022exploring,kojima2023implementation}.
Thus, an additional goal of this paper is to quantify the magnitude and character of bias that reconstruction error introduces.
In particular, we calculate phylometric metrics across range of reconstruction accuracy levels, and report the level of accuracy necessary to attain metric readings statistically indistinguishable from ground truth.

The utility of a model system for experimental evolution hinges on sufficient ability to observe and interpret underlying evolutionary dynamics.
Benchtop and field-based biological models continue to benefit from ongoing methodological advances that have profoundly increased visibility into genetic, phenotypic, and phylogenetic state \citep{woodworth2017building,blomberg2011measuring,schneider2019past}.
Simulation systems, in contrast, have traditionally enjoyed perfect, complete observability \citep{hindre2012new}.
However, ongoing advances in parallel and distributed computing hardware have begun to strain analytical omnipotence, as increasingly vast throughput introduces challenges centralizing, storing, and analyzing data \citep{klasky2021data}.
These trends, although unfolding opposite one another, exhibit intriguing convergence: computational and biological domains will provide data that is multimodal and high-resolution but also incomplete and imperfect.
Such convergence establishes great potential for productive interdisciplinary exchange.

% These come in two forms: 1) that can be used to draw abstract insights from lineages and phylogenies \citep{dolsonInterpretingTapeLife2020}, and 2) algorithmic techniques for efficiently collecting phylogenetic data at scale \citep{morenoHereditaryStratigraphyGenome2022}.

% Currently, most research on this topic is either very abstract (e.g., the presence of negative-frequency dependent selection increases phylogenetic diversity) or very specific (e.g., phylogenetic structure can be used to infer cell division rates in solid tumors \citep{lewinsohnStatedependentEvolutionaryModels2023}).
% Here, we lay the groundwork for identifying the fingerprints left on phylogenetic structure by a larger range of evolutionary dynamics in a scalable and robust manner.

%Some groundwork has been done in the fields of conservation biology and cancer biology, as well as in artificial life (cite ``tape of life''?) to understand how evolutionary dynamics affect phylogenetic structure (and the fingerprints of evolutionary dynamics on phylogenetic structure) but this is still a rapidly emerging field (be sure to hedge here).
%In particular, existing work has shown x, y and z.

% %One major difference between digital study systems and biological study systems is the availability of perfect data.
% %In biology, we rely on reconstructions to estimate phylogenetic history; the effect of estimation error on phylometrics is poorly understood.
% Historically, digital evolution systems have had the advantage of providing perfectly accurate phylogenetic data, in contrast to the reconstructed phylogenies relied upon in traditional biology.
% However, as digital evolution systems scale, issues of data loss and decentralization will make perfect tracking at best inefficient and at worst untenable.
% Thus, some systems will likely need to adopt a decentralized, reconstruction-based approach similar to biological data.
% %Decentralization will also likely introduce an aspect of spatial structure (i.e., populations will no longer be ``well-mixed'') which will further complicate phylogenetic analyses.
% Consequently, if our goal is to use phylogenetic metrics to increase the scalability of our data analysis, we must also understand how robust they are to inaccuracies introduced by reconstruction.
% % (maybe briefly cite/mention effect of spatial structure on phylogenies)

% In this paper, we build the following methodological and theoretical foundations that will be needed to use phylogenetic analyses to observe evolutionary dynamics in complex, decentralized systems with imperfect observability:
% \begin{enumerate}
%   \item understanding of the relationship between evolutionary dynamics and phylogenetic metrics,
%   \item quantification of the effects of reconstruction-induced estimation error on phylogenetic structure, both in terms of the amount of precision required for accuracy and the amount of bias introduced by inadequate precision, and
%   \item quantification of the phylogenetic effects of spatial structure, as distributed computation does not support well-mixed populations.
% \end{enumerate}

% \begin{enumerate}
% \item how much precision is required for accurate phylogenetic metrics?
% \item if bias is introduced, what type of bias (so could still detect "conservatively")
% \end{enumerate}

% In evolutionary biology, phylogenetic history is a valuable tool to triangulating the context of notable evolutionary events, as well as characterizing the underlying mode and tempo of evolution.
% The same holds true in evolutionary simulation.
% % https://github.com/mmore500/phylotrack-algorithm-analysis/blob/fe16d2b2d7df99faade09c01b72f681160749f51/tex/text/body/introduction.tex
% In addition to addressing questions of natural history, access to the phylogenetic record of biological life has proven informative to conservation biology, epidemiology, medicine, and biochemistry among other domains \citep{faithConservationEvaluationPhylogenetic1992, STAMATAKIS2005phylogenetics, frenchHostPhylogenyShapes2023,kim2006discovery}.
% Nonetheless, existing analyses of phylogenetic structure within digital systems have already proven valuable, enabling diagnosis of underlying evolutionary dynamics \citep{moreno2023toward,hernandez2022can,shahbandegan2022untangling, lewinsohnStatedependentEvolutionaryModels2023a} and even serving as mechanism to guide evolution in application-oriented domains \citep{lalejini2024phylogeny,lalejini2024runtime,murphy2008simple,burke2003increased}.
% Further, comparison of observed phylogenies against simulation phylogenies can be used to evaluate hypotheses for underlying dynamics within real-life evolutionary/epidemiological systems \citep{giardina2017inference,voznica2022deep}.


==> bindertex-evolutionary-inference/text/body/methods.tex <==
\section{Methods}
\label{sec:methods}

\subsection{Model Systems}

To assess the generality of evolutionary dynamics' effects on phylogenetic structure, we replicated experiments across models differing in subject and approach.
We used three systems,
\begin{enumerate}
\item a simple agent-based model with explicitly encoded fitness values;
\item Avida, a self-replicating agent-based evolutionary platform \citep{ofria2004avida}; and
\item Gen3sis, a population-level macro-ecological/evolutionary model \citep{hagen2021gen3sis}.
\end{enumerate}

The following introduces each model and details experiment-specific configurations.

\noindent
\textbf{Simple Explicit-Fitness Model}

\noindent
Experiments testing the relationships between evolutionary dynamics, reconstruction error, and phylogenetic structure required a model system amenable to direct, interpretable tuning of ecology, spatial structure, and selection pressure.
% @ELD: Maybe rename this section? I got through the first paragraph without realizing it was specifically about the simple modelAdditionally, in order to make findings relevant to large-scale phylogenetic analyses, computational efficiency was necessary to facilitate large population size and high generation counts.
Finally, a parsimonious and generic model system was desired so that findings would better generalize across digital evolution systems.
The core of this work relies on a simple agent-based model devised to fulfill these objectives.
% @ELD: Do we still want to say this is the core of the work now that we've got the other systems?
% @MAM: Depends how much of results the other parts end up taking up, I kind of imagine they might appear in a single section if they end up being similar to the simple model

Genomes in the simple explicit-fitness model comprised a single floating-point value, with higher magnitude corresponding to higher fitness.
Population size 32,768 ($2^{15}$) was used for all experiments.
Selection was performed using tournament selection with synchronous generations.
Treatments' selection pressure was controlled via tournament size.
Mutation was applied after selection, with a value drawn from a unit Gaussian distribution added to all genomes.
Evolutionary runs were ended after 262,144 ($2^{18}$) generations.
Each run required around 4 hours of compute time.

Treatments incorporating spatial structure used a simple island model.
In spatially structured treatments, individuals were evenly divided among 1,024 islands and only competed in selection tournaments against sympatric population members.
Islands were arranged in a one-dimensional closed ring and 1\% of population members migrated to a neighboring island each generation.

Treatments incorporating ecology used a simple niche model.
Population slots were split evenly between niches.
Organisms were arbitrarily assigned to a niche at simulation startup and were only allowed to occupy population slots assigned to that niche.
Therefore, individuals exclusively participated in selection tournaments with members of their own niche.
In treatments also incorporating spatial structure, an even allotment of population slots was provided for every niche on every island.
Every generation, individuals swapped niches with probability $3.0517578125 \times 10^{-8}$ (chosen so one niche swap would be expected every 1,000 generations).

For our main experiments, we defined the following ``regimes'' of evolutionary conditions:
\begin{itemize}
  \item \textit{plain}: tournament size 2 with no niching and no islands,
  \item \textit{weak selection}: tournament size 1 with no niching and no islands,
  \item \textit{strong selection}: tournament size 4 with no niching and no islands,
  \item \textit{spatial structure}: tournament size 2 with no niching and 1,024 islands,
  \item \textit{weak ecology}: tournament size 2 with 4 niches and niche swap probability increased 100$\times$,
  \item \textit{ecology}: tournament size 2 with 4 niches, and
  \item \textit{rich ecology}: tournament size 2 with 8 niches.
\end{itemize}

In follow-up experiments testing ecological dynamics with a spatial background, we defined the following additional evolutionary ``regimes:''
\begin{itemize}
  \item \textit{plain}: tournament size 2 with no niching over 1,024 islands,
  \item \textit{weak ecology}: tournament size 2 with 4 niches and niche swap probability increased 100$\times$ over 1,024 islands,
  \item \textit{ecology}: tournament size 2 with 4 niches over 1,024 islands, and
  \item \textit{rich ecology}: tournament size 2 with 8 niches over 1,024 islands.
\end{itemize}

Finally, to foster generalizability of findings, all experiments were performed with two alternate ``sensitivity'' variables: evolutionary length in generations and mutation operator.
We saved phylogenetic snapshots at 32,768 generation epochs.
This allowed us to test shorter runs of 32,768 and 98,304 generations (through epochs 0 and 2) in addition to the full-length runs (through epoch 7).
One additional mutation operator was tested to contrast the unit Gaussian distribution: the unit exponential distribution.
Under this distribution, deleterious mutations are not possible and large-effect mutations are more likely.

Across all experiments, each treatment comprised 50 replicates.

\noindent
\textbf{Avida Model}

\noindent
Avida is a virtual agent-based model system used for sophisticated \textit{in silico} evolution experiments \citep{ofria2004avida}.
Notably, unlike the simple model described above, fitness within Avida arises implicitly from agents' self-replication activity, in relation to other agents' self-replication and the availability of shared exogenous resources.
Within Avida, digital organisms' genomes comprise a sequence of virtual CPU instructions.
Avida conducts open-ended evaluation of each agent's genetic program, affording the opportunity of copying itself into output memory and thereby creating an offspring agent.
Replication imposes an intrinsic baseline level of copy errors (i.e., mutations), ensuring an ongoing supply of genetic variation.
Because self-replicators compete for a limited quantity of population slots, Darwinian evolution ensues.
This scheme induces a complex fitness landscape, which is thought to better reflect the character of biological evolution \citep{adami2006digital}.

Under baseline conditions, Avidians compete on the basis of self-replication efficiency.
However, Avida may be configured to award extra CPU cycles to agents that complete boolean logic tasks.
To create the potential for multiple niches, we associated each task with a depletable resource.
Avidians only recieve CPU cycles for completeing a task if the corresponding resource is available, and completing a task depletes the associated resource.
Importantly, tasks can each be associated with different resources, or they can all be associated with the same resource.
Association of each task to an independent resource creates potential for stable ecological coexistence between task-specialized clades.
We added the constraint that Avidians may harvest at most two tasks with the intention of preventing generalists from disrupting task specialization.

Our baseline ``\textit{plain}'' treatment rewarded four boolean logic tasks (echo, not, nand, and), all drawing from a single resource with inflow rate 400 units per update.
Population structure was well-mixed and, to somewhat weaken the fecundity of high-fitness Avidians, replication destroyed the parent organism with probability 0.2.

We surveyed six additional ``regimes'' of evolutionary conditions, defined accoring to pre-existing Avida configuration options.
Notably, compared to the simple model above, these manipulations are somewhat more indirect and, therefore, potentially weaker in nature.
We anticipate they might better reflect the character of variations in evolutionary drivers that might be encountered in practice.

Regimes were configured as follows,
\begin{itemize}
  \item \textit{weak selection}: the probability of parent death was increased to 0.5;
  \item \textit{strong selection}: parent death probability was set to 0.0 and offspring were protected from replacement by their own offspring;
  \item \textit{spatial structure}: population was arranged as a two-dimensional toroidal grid, with Avidians replicating exclusively between neighboring population sites;
  \item \textit{weak ecology}: tasks were assigned independent resource pools, but three resources were only supplied at an inflow rate of 33 units while the fourth was supplied at 300 units per update,
  \item \textit{ecology}: each task drew from an independent resource pool with inflow rate of 100 units, and
  \item \textit{rich ecology}: 28 tasks were rewarded, each drawing from an independent resource pool with an inflow rate of 100 units.
\end{itemize}

In follow-up experiments, we defined the following additional evolutionary ``regimes'' with two-dimensional toroidal spatial structure,
\begin{itemize}
  \item \textit{plain}: four boolean logic tasks drawing from a single resource with inflow rate 400 units per update,
  \item \textit{weak ecology}: tasks were assigned independent resource pools, but three resources were only supplied at an inflow rate of 33 units while the fourth was supplied at 300 units per update,
  \item \textit{ecology}: each task drew from an independent resource pool with inflow rate of 100 units, and
  \item \textit{rich ecology}: 28 tasks were rewarded, each drawing from an independent resource pool with an inflow rate of 100 units.
\end{itemize}

\input{fig/perfect-tree-phylogenies-log-avida}

Experimental treatments using Avida comprised 30 replicates, conducted with population size 3,600 for durations of 100,000 time steps (c. 20k generations; range 9k-40k).

In order to achieve the phylogenetic tracking necessary for our experiments, we used a fork of Avida originally developed for research on MODES \citep{dolson2019modes}, linked in supplemental materials described below.
This tracking system allowed two configurations: (1) tracking on the level of individual agents, where each Avidian constituted a taxonomic unit, or (2) tracking on the level of genotypes, where clonal sets of Avidians with identical genotypes constituted a taxonomic unit.
Figure \ref{fig:perfect-tree-phylogenies-log-avida} compares example phylogenies from Avida under the ``plain'' treatment, tracked at organism and genome level.
Surprisingly, we noticed several sign-change differences between individual-level and genotype-level tracking with respect to treatments' effects on phylometrics (Figures \ref{fig:perfect-tree-phylometrics-avida-heatmap} and \ref{fig:perfect-tree-phylometrics-heatmap-avida-genome}).
Much, but not all, of the difference related to effects of spatial structure.
These differences may be in part related to occurrences of polytomies within genotype-level tracked phylogenies, as arbitrarily resolving polytomies into sets of bifurcating nodes gave somewhat more similar results to individual-level tracking.
Here, we report results from individual-level tracking, which corresponds to how phylogenies were tracked in the simple model.


\noindent
\textbf{Gen3sis Model}


\noindent
In contrast to Avida and the simple model, which are agent-based, Gen3sis is a population-level model.
Gen3sis abstracts evolution to interactions between spatially-dispersed, speciating subpopulations.
Co-located subpopulations of different species compete for shares of site-specific carrying capacity.
Interaction between subpopulation traits and environmental factors (e.g., aridity, temperature) mediates abundance determinations.
Disjoined subpopulations of the same species accumulate genetic incompatibilities absent sufficient gene flow and, past a defined incompatibility threshold, speciate.
Within this model, the taxonomic unit of phylogeny is species.

Gen3sis also stands out in its intended level of direct biological realism.
The software can be configured to reflect the particular geological and climate histories of continental biomes.
For our experiments, we used curated raster files depicting conditions over 30 million years in South America bundled with the package that had been synthesized from a number of sources \citep{straume2020global,westerhold2020astronomically,fick2017worldclim,hagen2019mountain,annan2013new,cramwinckel2018synchronous,evans2018eocene,hollis2019deepmip,hutchinson2018climate,keating2011warm,sijp2014role,zhang2019evolution}.

Among other features, Gen3sis allows differentiation of aquatic (e.g., lakes, ocean) zones from terrestrial regions with respect to suppression of inter-population migration rates.
To enhance potential for manipulable spatial structure within the model, we converted 30 randomly-selected thin linear segments spanning the map to be aquatic rather than terrestrial (i.e., ``rivers'').
Spatial structure was then induced by adjusting the water traversal cost function.

\input{fig/perfect-tree-phylogeny-gen3sis}

We assessed the following evolutionary regimes,
\begin{itemize}
\item \textit{plain}: aquatic terrain imposed no additional migration penalties and population traits did not influence abundances;
\item \textit{spatial structure}: aquatic terrain imposed a migration barrier $50\times$ that of terrestrial terrain;
\item \textit{ecology}: species abundances were determined according to how close populations' trait value matches to site temperature; and
\item \textit{ecology + spatial structure}: the $50\times$ aquatic dispersal penalty was applied, and site temperature was used to determine species' abundances.
\end{itemize}
Figure \ref{fig:perfect-tree-phylogeny-gen3sis} shows an example Gen3sis phylogeny from the ``plain'' regime.

Gen3sis treatments comprised 30 replicates.
Note that, unlike other surveyed models, Gen3sis does not operate with constant ``population size.''
Rather, species count increased continuously over each of the 30 simulated 1 million year time steps as a consequence of ongoing speciation.
Maximum species count per spatial site was configured as 2,500 and within the entire simulation as 25,000, although neither limit was ever reached.

Full Gen3sis configuration files are linked in supplemental materials, described below.
For more on Gen3sis itself, see \citep{hagen2021gen3sis}.

\subsection{Hereditary Stratigraphic Annotations and Tree Reconstruction}

Experiments testing the impact of phylogenetic inference error on phylometrics employ the recently-developed ``hereditary stratigraphy'' technique to facilitate phylogenetic inference \citep{moreno2022hstrat}.
This technique works by attaching heritable annotations to individual digital genomes.
Every generation, a new random ``fingerprint'' is generated and appended to the individuals' inherited annotations.
To reconstruct phylogenetic history, fingerprints from extant organisms' annotations can be compared.
Where two organisms share identical fingerprints along the record, they likely shared common ancestry.
Mismatching fingerprints indicate a split in compared organisms' ancestry.
Although extensions of hereditary stratigraphy to sexual lineages are possible \citep{moreno2024methods}, all lineages used for experiments were asexual in nature.

Hereditary stratigraphy enables a tunable trade-off between annotation size and estimation accuracy.
Fingerprints may be discarded to decrease annotation size at the cost of reduced density of reference points to test for common (or divergent) ancestry along organisms' generational histories.

We test four levels of fingerprint retention.
Each level is described as a $p\%$ ``resolution'' meaning that the generational distance between reference points any number of generations $k$ back is less than $(p / 100) \times k$.
So, a high percentage $p$ indicates coarse resolution and a low percentage $p$ indicates fine resolution.
In detail, at the conclusion of 262,144 generation evolutionary runs,
\begin{itemize}
  \item at 33\% resolution 68 fingerprints are retained per genome,
  \item at 10\% resolution 170 fingerprints are retained per genome,
  \item at 3\% resolution 435 fingerprints are retained per genome, and
  \item at 1\% resolution 1,239 fingerprints are retained per genome.
\end{itemize}

This work uses 1 byte fingerprints, which collide with probability $1/256$.
Greater space efficiency could be achieved using 1 bit fingerprints.
However, this would require careful accounting for ubiquitous generation of identical fingerprints by chance and is left to future work.

Previous work with hereditary stratigraphy used UPGMA distance-based reconstruction techniques \citep{moreno2022hereditary}.
Large-scale reconstructions required for these experiments necessitated development of a more efficient technique that did not require all pairs (i.e., $O(n^2)$ distance comparison.
To accomplish this, we devised an agglomerative tree building algorithm that works by successively adding leaf organism annotations and percolating them down from the tree root along the tree path of internal nodes consistent with their fingerprint sequence, then affixing them where common ancestry ends.
This new tree-building approach reduced compute time from multiple hours to around 5 minutes in most cases.
Supplementary Listing \ref{lst:build_tree_trie} provides source code with full implementation details, see \citep{moreno2024analysis} for a more detailed discussion.

\input{fig/plain-perfect-and-reconstruction-phylogenies}

To assess the efficacy of the new agglomerative tree-building approach, we calculated all reconstructed trees' quartet distance to their respective reference.
Quartet distance ranges from 0 (between identical trees) to 0.75 (between random trees), providing in this case a measure of reconstruction error.
As expected, this measure of reconstruction error varied significantly with resolution for trees across all evolutionary regimes (Kruskal-Wallis tests; all $p < 10^{-20}$; Supplementary Table \ref{tab:reconstruction-error-comparisons-between-resolutions}).
Reconstruction error also varied significantly with evolutionary regime for each reconstruction resolution level (Kruskal-Wallis tests; all $p < 10^{-8}$; Supplementary Table \ref{tab:reconstruction-error-comparisons-between-regimes}).

For 3\% and 1\% resolutions, mean reconstruction error was less than 0.01 in all cases and at 10\% resolution mean reconstruction error was less than 0.05 in all cases.
At 33\% resolution, mean reconstruction error was less than 0.12 in all cases.
The largest reconstruction errors observed at 1\%, 3\%, 10\%, and 33\% resolutions were, respectively, 0.051 (weak selection regime), 0.093 (weak 4 niche ecology regime), 0.14 (plain evolutionary regime), and 0.45 (plain evolutionary regime).
Supplementary Table \ref{tab:tree-reconstruction-quality-quartet-summary-statistics} reports mean, median, standard deviation, and maxima for reconstruction error across surveyed evolutionary conditions.

To generate reconstructed trees in experiments, we simulated the inheritance of hereditary stratigraphic annotations along a reference phylogeny to yield the set of annotations that would be attached to extant population members at the end of a run, then used our agglomerative tree building technique to infer.
Thus, each reconstruction replicate has a directly-corresponding reference tree from a perfect-tree treatment replicate.
Figure \ref{fig:plain-perfect-and-reconstruction-phylogenies} shows a reference tree and corresponding reconstructions performed using 1\%, 3\%, 10\%, and 33\% resolution hereditary stratigraph annotations.

\subsection{Phylometrics}

A wide range of metrics exists for quantifying the topology of a phylogeny.
Tucker et al. showed that these metrics can be classified into the following three dimensions: richness, divergence, and regularity \citep{tuckerGuidePhylogeneticMetrics2017}.
Richness metrics quantify the amount of phylogenetic diversity/evolutionary history represented by a phylogeny.
Divergence metrics quantify how different the units of the phylogeny are from each other.
Regularity metrics quantify the variance of other properties (i.e. how consistent they are across the phylogeny).
Here, we focus on four metrics spread across these categories:

\textbf{Sum Pairwise Distance:} This measurement sums the nodeal distance between each pair of leaf nodes.
It is a metric of phylogenetic richness \citep{tuckerGuidePhylogeneticMetrics2017}, also referred to as \textit{F}  \citep{izsakLinkEcologicalDiversity2000}.
%It is a metric of phylogenetic richness and is closely related to Faith's classic phylogenetic diversity metric \citep{faithConservationEvaluationPhylogenetic1992}.
Consequently, we would expect it to be increased by the presence of ecology or spatial structure, as both these factors increase diversity.
% TODO do we want to say more here?

\textbf{Colless-like Index:}
The original Colless Index \citep{collessReviewPhylogeneticsTheory1982}, also often referred to as $I_c$ \citep{shaoTreeBalance1990}, is a measure of tree imbalance (i.e., it gets higher as the tree gets less balanced).
In the context of Tucker et al.'s framework, it is a regularity metric.
However, the traditional Colless Index only works for strictly bifurcating trees.
As our trees have multifurcations, we instead use the Colless-like Index, which is an extension of the Colless Index to multifurcating trees \citep{mirSoundCollesslikeBalance2018}.
Tree imbalance is thought to be associated with varying ecological pressures \citep{chamberlainPhylogeneticTreeShape2014, burressEcologicalOpportunityAlters} and has also been observed to increase in the presence of spatial structure \citep{scottInferringTumorProliferative2020}.

\textbf{Mean Pairwise Distance:}
This metric is calculated by computing the shortest distance between all pairs of leaf nodes and taking the mean of these values \citep{webbExploringPhylogeneticStructure2000}.
Note that these distances are measured in terms of the number of nodes in between the pair, not in terms of branch lengths.
Mean pairwise distance is a metric of evolutionary divergence \citep{tuckerGuidePhylogeneticMetrics2017}.
Mean pairwise distance should be increased by scenarios that promote the long-term maintenance of distinct phylogenetic branches, such as ecology.
Conversely, factors that act to reduce diversity should also reduce mean pairwise distance.

\textbf{Mean Evolutionary Distinctiveness:}
Evolutionary distinctiveness is a metric that can be calculated for individual taxa to quantify how evolutionarily different that taxon is from all other taxa in the phylogeny \citep{isaacMammalsEDGEConservation2007}.
To get mean evolutionary distinctiveness, we average this value across all extant taxa in the tree.
Like mean pairwise distance, mean evolutionary distinctiveness is a metric of evolutionary divergence.
However, it is known to capture substantially different information than mean pairwise distance \citep{tuckerGuidePhylogeneticMetrics2017}.
Unlike our other metrics, evolutionary distinctiveness is heavily influenced by branch length.
We generally expect mean evolutionary distinctiveness to be increased by similar factors to mean pairwise distance.

\subsection{Effect-size Analysis}

We expect statistical tests for between treatments we respect to evolutionary dynamics of interest to serve as an important use case for phylometric analyses in digital evolution.
As such, we wish to report the capability of reported phylometrics to discern between surveyed evolutionary conditions.

Cliff's delta provides useful nonparametric means for such effect size analysis.
This statistic reports the proportion of distributional non-overlap between two distributions, ranging from -1/1 if two distributions share no overlap to 0 if they overlap entirely \citep{meissel2024using,cliff1993dominance}.
When reporting effect size, we use conventional thresholds of 0.147, 0.33, and 0.474 to distinguish between negligible, small, medium, and large effect sizes \citep{hess2004robust}.

Note that the Cliff's delta statistic tops/bottoms out entirely once two distributions become completely separable.
Although this property suits most analyses performed, it is occasionally useful to distinguish the extent of divergence between phylometric distributions past the point of complete separability.
For these purposes, we perform a simple procedure to normalize phylometrics relative baseline conditions by subtracting out the baseline mean and dividing by the baseline standard deviation.

We typically pair effect-size analysis with Mann-Whitney U testing in order to assess the extent to which differences between phylometric readings under different conditions are, or are not, evidenced by available data \citep{mann1947on}.
As a final detail, note that we typically report negated Cliff's delta values where necessary to ensure positive values correspond to larger phylometric values and vice versa.

\subsection{Software and Data Availability}

Software, configuration files, and executable notebooks for this work are available at \href{https://doi.org/10.5281/zenodo.10896667}{doi.org/10.5281/zenodo.10896667}.
Data and supplemental materials are available via the Open Science Framework \url{https://osf.io/vtxwd/} \citep{foster2017open}.
Note that materials for earlier versions of this work are also contained in these repositories \citep{moreno2023toward}.

All hereditary stratigraph annotation, reference phylogeny generation, and phylogenetic reconstruction tools used in this work are published in the \texttt{hstrat} Python package \citep{moreno2022hstrat}.
This project can be visited at \url{https://github.com/mmore500/hstrat}.

This project uses data formats and tools associated with the ALife Data Standards project \citep{lalejini2019data} and benefited from many pieces of open-source scientific software \citep{ofria2020empirical,sand2014tqdist,2020SciPy-NMeth,harris2020array,reback2020pandas,mckinney-proc-scipy-2010,sukumaran2010dendropy,cock2009biopython,dolson2024phylotrackpy,torchiano2016effsize,waskom2021seaborn,hunter2007matplotlib,moreno2024apc,moreno2024qspool,moreno2023teeplot,hagen2021gen3sis,ofria2004avida,torchiano2016effsize}.

==> bindertex-evolutionary-inference/text/body/results-and-discussion.tex <==
\section{Results and Discussion}
\label{sec:results}

\subsection{Phylometric Signatures of Evolutionary Dynamics}

\input{fig/perfect-tree-phylogenies-log}
\input{fig/perfect-tree-phylometrics}

The feasibility of harnessing phylogenetic analysis to identify evolutionary dynamics hinges on the premise that these dynamics induce detectable structure within the phylogenetic record.
Fortunately, as shown in Figure \ref{fig:perfect-tree-phylogenies-log}, dendrograms of phylogenetic histories from the different evolutionary conditions tested do indeed exhibit striking visual differences.

As a first step to characterizing the phylogenetic impact of spatial structure, ecology, and selection pressure, we tested whether surveyed evolutionary conditions exhibited detectable differences in a representative suite of four phylometrics: evolutionary distinctiveness, Colless-like index, mean pairwise distance, and sum pairwise distance.
Figure \ref{fig:perfect-tree-phylometrics} summarizes the distributions of each metric across surveyed conditions.
Statistical tests confirmed that each phylometric exhibited significant variation among surveyed evolutionary conditions for both the simple model and Avida (Kruskal-Wallis tests; all $p < 10^{-40}$; $n=50$ per condition simple model, $n=30$ Avida; Supplementary Table \ref{tab:phylostatistics-comparison-between-regimes-kwallis}).

To quantify the phylometric effects of surveyed evolutionary regimes, we performed nonparametric statistical comparisons against the ``plain'' baseline treatment.
We used a measure of distributional overlap --- Cliff's delta --- to assess effect sizes, binning into ``negligible'', ``small'' (+), ``medium'' (++), and ``large'' (+++) effects based on conventional thresholds \citep{hess2004robust}.
Significance at $\alpha = 0.05$ (*) was assessed through Mann-Whitney tests.
Figure \ref{fig:perfect-tree-phylometrics-simple-heatmap} shows nonparametric significance and effect size test results.

\noindent
\textbf{Summary of Phylometric Effects}

\noindent
Relative to the plain regime, all evolutionary regimes in the simple model depress the Colless-like index.
Reduction in this statistic indicates that all deviations from baseline conditions increased regularity in generated phylogenies.
This observation runs somewhat counter to prior results on similar tree balance metrics, in which the presence of spatial structure increased imbalance \citep{scottInferringTumorProliferative2020}.
One possible contributing factor is that taxa in our phylogenies were individuals, whereas Scott et al. used genotype-level abstraction (i.e., their trees were gene trees).
%Application of the metric to trees comprised individual-level taxa, instead of species-level taxa as is the case in most traditional phylogenetics work, may account for this result.
This possible effect of taxonomic unit is consistent with our results from the species-level phylogenies in the  Gen3sis system (Figure \ref{fig:perfect-tree-phylometrics-gen3sis}), in which ecological and spatial conditions elevated Colless imbalance.
Avida individual-level phylogenies were more consistent with the simple model than with Gen3sis; Colless index was significantly depressed under ecological regimes, and weakly but insignificantly depressed under spatial structure.
However, other modes of evolution did not meaningfully affect Colless-like index of Avida phylogenies.

Colless-like index is sensitive to changes in evolutionary conditions.
However, it appears to be the least useful metric in distinguishing different drivers of evolutionary dynamics, decreasing significantly under all non-plain evolutionary conditions.

Mean evolutionary distinctiveness was significantly higher under weak selection and with spatial structure than in the plain regime.
This metric significantly decreased under strong selection and under ecological regimes, but the numerical magnitudes of these effects were relatively smaller (Figure \ref{fig:perfect-tree-phylometrics-heatmap-parametric}).
We observed similar results in Avida, except no significant effect of strong selection and weak ecology was detected on the phylometric outcome.

Mean pairwise distance was significantly depressed under all regimes except ecology and weak ecology, although again the numerical magnitude of effects on ecological regimes were relatively smaller (Figure \ref{fig:perfect-tree-phylometrics-heatmap-parametric}).
Within Avida, weak but insignificant depressing effects were observed under weak selection and spatial structure regimes.
In contrast to results from the simple model, the strongest depressing effects were observed under the weak ecology and strong ecology regimes.

Finally, sum pairwise distance was significantly increased under all regimes compared to baseline, except for the strong selection regime where it was significantly depressed.
Effect size was again strongest under spatial structure and weak selection (Figure \ref{fig:perfect-tree-phylometrics-heatmap-parametric}).
Avida gave similar results, except that no significant effect was detected from the weak ecology and strong selection treatments, with a weak but insignificant increase effect detected under strong selection.

\noindent
\textbf{Discussion of Phylometric Effects}

\noindent
Ecological dynamics have significant influence on the surveyed phylometrics.
However, the numerical magnitudes of these effects are generally weak compared to spatial structure and selection effects (Figure \ref{fig:perfect-tree-phylometrics-heatmap-parametric}).
So, it appears careful accounting for other evolutionary dynamics (i.e., selection pressure and spatial structure) will be essential to accurate detection of ecology through phylogenetic analysis.
Mean pairwise distance may play a role in identifying ecological dynamics, as ecological dynamics --- in contrast to other factors such as spatial structure and changes in selection pressure --- have weaker effects on this phylometric.
Other phylogenetic metrics may also be better suited to detecting ecological dynamics (e.g. the ecology metric in \citep{dolson2019modes}).

Phylometric outcomes within Avida generally mirror the simple fitness model, although in many cases phylometric effects are weaker or not significant.
These less pronounced effects are not unexpected --- whereas the simple model was explicitly designed for direct manipulation of evolutionary drivers, we use more subtle configurations to impose evolutionary drivers on the Avida model (particularly, with respect to selection pressure).
Notably, the strong selection treatment resulted in no significant effects on phylometric values.
Weak selection significantly increased mean evolutionary distinctiveness and sum pairwise distance, as with the simple model, but the effect size was small.
However, spatial structure's effect size on these metrics was large and agreed with the simple model.
The ecology and rich ecology treatments agreed in sign with the simple model and generally had large effect size.
However, unlike the simple model, Avida's sole phylometric outcome under weak ecology was a strong, significant decrease in mean pairwise distance.
In contrast, the simple model exhibited no effect on this metric under the weak ecology treatment.

We additionally performed a sensitivity analysis for results from the simple model over an alternate exponential mutation operator and earlier phylogeny sampling time points.
The effects of evolutionary conditions on phylometrics were generally consistent with Figure \ref{fig:perfect-tree-phylometrics-simple-heatmap} across surveyed conditions (Supplementary Figures \labelcref{fig:perfect-tree-phylometrics-sensitivity-analysis,fig:perfect-tree-phylometrics-heatmap-sensitivity-analysis}).

\subsection{Phylometric Signatures of Ecological Dynamics in Spatially Structured Populations}

\input{fig/perfect-tree-phylometrics-heatmap-parametric}

The effects of spatial structure are of particular interest, as evolution within very large populations typically entail elements of spatial structure owing to dispersal across geographic terrain.
Even within \textit{in silico} contexts, populations too large for a single processor will almost inevitably integrate spatial structure that reflects practical limitations of distributed computing hardware \citep{ackley2014indefinitely,moreno2021conduit}.
Therefore, understanding the background effects of spatial structure on the phylogenetic signatures of other evolutionary dynamics will be essential to applications of phylogenetic inference in such applications.
For this analysis, we chose to focus on ecological dynamics due to interest in how their relatively weak phylometric signatures would respond to the relatively strong influence of spatial structure (Figure \ref{fig:perfect-tree-phylometrics-heatmap-parametric}).

\noindent
\textbf{Summary of Phylometric Effects with Background Spatial Structure}

\input{fig/perfect-tree-phylometrics-with-spatial-nuisance}

\noindent
Figure \ref{fig:perfect-tree-phylometrics-with-spatial-nuisance} summarizes the distribution of surveyed phylometrics under the three surveyed ecological regimes and the control non-ecological regime, all with spatial population structure.
Statistical tests confirmed that each phylometric exhibited significant variation among these evolutionary regimes, indicating the presence of detectable structural signatures in phylogenetic structure (Kruskal-Wallis tests; all $p < 1\times10^{-8}$; $n=50$ per condition for simple model, $n=30$ Avida; Supplementary Tables \labelcref{tab:phylostatistics-comparison-between-regimes-spatial-nuisance-kwallis,tab:phylostatistics-comparison-between-regimes-spatial-nuisance-kwallis-avida}).

As in prior experiments, all ecology treatments drove significant increases in mean evolutionary distinctiveness and sum pairwise distance.
Also consistent with spatially unstructured results, rich ecology drove significant, large-effect depression of both Colless-like index and mean pairwise distance and ecology.
However, in the presence of spatial structure, the ecology treatment depressed only mean pairwise distance.
Without spatial structure, the ecology treatment depressed Colless-like index instead.
Results under weak ecology differed notably from non-spatial baseline, with all phylometrics seeing significant, large-effect increases.
Spatial-background rich ecology results from Avida agreed with the simple model.
However, significant phylometric effects were not detected from the ecology and weak ecology treatments under spatial structure conditions.

For these experiments, we again performed a sensitivity analysis over an alternate exponential mutation operator and earlier phylogeny sampling time points.
We found the effects of evolutionary conditions on phylometrics to be generally consistent across surveyed conditions (Supplementary Figure \ref{fig:perfect-tree-phylometrics-with-spatial-nuisance-sensitivity-analysis} and Supplementary Tables \labelcref{tab:phylostatistics-comparison-between-regimes-spatial-nuisance-kwallis,tab:phylostatistics-comparison-between-resolutions-allpairs-wilcox-spatial-nuisance}).

\subsection{Species-level Phylogenies from Gen3sis Model}

\input{fig/perfect-tree-phylometrics-gen3sis}
\input{fig/perfect-tree-phylometrics-heatmap-avida-genome}

%Figure \ref{fig:perfect-tree-phylometrics-gen3sis} shows phylometric effects of spatial structure and of ecology, both with and without a spatial structure background.
Significant, large-effect changes were detected across all four phylometrics in each treatment in Gen3sis (see Figure \ref{fig:perfect-tree-phylometrics-gen3sis}).
However, with the exception of sum pariwise distance, effect signs of treatments were opposite to those for individual-level phylogenies from Avida and the simple model across all phylometrics.
Tip count effects seem likely to play a role in this discrepancy.
Unlike Avida and the simple model, which held population size constant, species richness grew freely under the Gen3sis model.
It is also possible that phylometric outcomes may be sensitive to granularity level of the taxonomic unit of the phylogeny.
As noted in Section \ref{sec:methods} and shown in Figure \ref{fig:perfect-tree-phylometrics-heatmap-avida-genome}, in Avida experiments, phylogenies using genome-level tracking (as opposed to individual-level tracking) were notably different than those using individual-level tracking.
These differences also included changes in the sign of some treatment effects, lending credence to the idea that differences between Gen3sis and the individual-level phylogenies could be partially the result of Gen3sis having a more abstract taxonomic unit.

\subsection{Phylometric Bias of Reconstruction Error}
\label{sec:phylometric-bias-reconstruction-error}

Shifting from perfect phylogenetic tracking to approximate phylogenetic reconstruction will facilitate efficiency and robust digital evolution simulations at scale, but introduces a complicating factor into phylogenetic analyses: tree reconstruction error.
A clear understanding of the impact of these errors on the computed phylometrics will be necessary for informative future phylogenetic analyses.

To explore this question, we compared phylometrics computed on reconstructed trees to corresponding true reference trees under the simple model (Wilcoxon tests; $n=50$ per condition; Supplementary Table \ref{tab:phylostatistics-comparison-between-resolutions-allpairs-wilcox}).
To err towards conservatism in detecting phylometric biases, we did not correct for multiple comparisons.
Reconstructions were performed across a range of precisions, ranging from 1\% relative resolution for MRCA estimates (most precise) to 33\% relative resolution for MRCA estimates (least precise).
Precision was manipulated by adjusting the information content of underlying hereditary stratigraphic genome annotations used to perform phylogenetic reconstruction \citep{moreno2022hereditary}.
Note that important differences exist the between nature of reconstruction error under hereditary stratigraphy versus traditional biosequence-based methods, discussed further below.

\input{fig/reconstructed-tree-phylometrics-error}

\noindent
\textbf{Phylometric Sensitivites to Reconstruction Error}

\noindent
For each phylometric, we sought to determine the minimum resolution required to achieve statistical non-detection (i.e., $p > 0.05$) of bias between reconstructions and their corresponding references.
For nearly all cases, 3\% reconstruction resolution was sufficient to achieve statistical indistinguishability between reference and reconstruction.
Mean evolutionary distinctiveness and sum pairwise distance were particularly robust to reconstruction error, showing no detectable bias even at only 33\% reconstruction resolution.

Phylometric sensitivity to reconstruction error was broadly consistent across evolutionary regimes.
Figure \ref{fig:reconstructed-tree-phylometrics-error} summarizes these results.

Where detectable, estimation uncertainty bias decreased all surveyed phylometrics' numerical value.
So, when testing for expected increases in phylometric values, the potential for systematic false positives due to reconstruction error can be discounted.
Supplementary Figure \ref{fig:reconstructed-tree-phylometrics} provides a full comparison of the distribution of phylometric estimates on reference trees with the distributions of phylometric estimates for reconstructed trees across reconstruction resolutions.

The relationship between reconstruction error and phylometric bias was similar under spatially structured regimes, the alternate exponential mutation operator, at earlier phylogeny sampling time points, and in the Avida model system (Supplementary Figures \labelcref{fig:reconstructed-tree-phylometrics-error-sensitivity-analysis,fig:reconstructed-tree-phylometrics-error-spatial-nuisance,fig:reconstructed-tree-phylometrics-with-spatial-nuisance,fig:reconstructed-tree-phylometrics-avida,fig:reconstructed-tree-phylometrics-error-avida}; Supplementary Table \labelcref{tab:phylostatistics-comparison-between-resolutions-allpairs-wilcox,tab:phylostatistics-comparison-between-resolutions-allpairs-wilcox-spatial-nuisance}).
Notably, however, reconstruction bias persisted at even 1\% relative resolution in some conditions of the sensitivity analysis and Avida experiments.
Forthcoming work has found that the byte-differentia hereditary stratigraphy configuration used for this experiment tends to lump closely contemporaneous lineage splitting events into a polytomy rather than a double-branching event --- i.e., indicating uncertainty rather than introducing error.
In contrast, reconstructions on single-bit differentia contain erroneously- sequenced branching rather than artifactual polytomies.
So, future work should explore whether working with single bit differentia could lessen phylometric bias.

\noindent
\textbf{Detection of Evolutionary Drivers' Signatures in Reconstructed Phylogenies}

\noindent
Our last objective was to assess how reconstruction error might affect detection of phylometric signatures induced by treatment conditions.
That is, we sought to perform a sort of ``integration test'' for detection of treatment conditions when working with imperfect reconstructions rather than perfect phylogenies.
To this end, we compared the phylometric outcomes of strong/weak selection, spatial structure, ecology, and weak/rich ecology relative to plain conditions for phylogenies reconstructed at 1\%, 3\%, 10\%, and 33\% resolution levels.
Supplemental Figures \labelcref{fig:reconstructed-tree-phylometrics-progressive-heatmap,fig:reconstructed-tree-phylometrics-progressive-heatmap-avida} show heatmaps with sign, effect size, and significance of phylometric effects across gradations of reconstruction precision for the simple model and Avida, respectively.
In most cases, 3\% resolution sufficed to fully recover phylometric effects of treatments observed with perfectly-tracked phylogenies.


==> bindertex-evolutionary-inference/text/frontmatter.tex <==
\title{ Ecology, Spatial Structure, and Selection Pressure Induce Strong Signatures in Phylogenetic Structure }

\author[1,2,3,*]{Matthew Andres Moreno\orcidlink{0000-0003-4726-4479}}
\author[4]{Santiago Rodriguez-Papa\orcidlink{0000-0002-6028-2105}}
\author[4,5]{Emily Dolson\orcidlink{0000-0001-8616-4898}}

\affil[1]{Department of Ecology and Evolutionary Biology, University of Michigan, Ann Arbor, United States}
\affil[2]{Center for the Study of Complex Systems, University of Michigan, Ann Arbor, United States}
\affil[3]{Michigan Institute for Data Science, University of Michigan, Ann Arbor, United States}
\affil[4]{Department of Computer Science and Engineering, Michigan State University, East Lansing, United States}
\affil[5]{Program in Ecology, Evolution, and Behavior, Michigan State University, East Lansing, United States}
\affil[*]{corresponding author: \textit{morenoma@umich.edu}}

\maketitle


==> bindertex-evolutionary-inference/text/references.tex <==
\putbib


==> draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
% \usepackage{lineno}
% \linenumbers
% \renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> fig/async-ga-schematic.tex <==
\begin{figure}
  \centering
\includegraphics[width=0.8\linewidth]{binder-wse-sketches/tex-access-proposal/img/async-ga-schematic}
  \caption{%
  \textbf{Island model GA implementation for WSE.}
  Neighboring PEs exchange agent genomes (``migration''') via asynchronous send/receive operations from dedicated buffers, with on-completion callbacks setting ``ready'' flags.
  }
  \label{fig:async-ga-schematic}
  \vspace{-0.2in}
\end{figure}


==> fig/benchmarking.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=0.85\textwidth,trim={0 0 0 0.4in
  }, clip]{binder-wafer-scale/binder/teeplots/all=false+hue=implementation+orient=h+row=language+score=nanoseconds-per-op+viz=peckplot+x=nanoseconds-per-op+y=policy+y-group=outer+ext=}

\vspace{-2.5ex}

  \caption{%
    \textbf{Hereditary stratigraphy algorithm benchmarks.}
    \footnotesize
    Comparison of per-generation operation time for column- and surface-based steady and tilted retention policies, lower is better.
    Top and bottom panels show Python and Zig implementations, respectively.
    Trivial is a simple hardcoded retention decision, provided as a baseline control.
    Background hatching indicates significant outcomes (Mann-Whitney U test; $n=20$).
  }
  \label{fig:benchmarking}
  \vspace{-0.2in}
\end{figure*}


==> fig/col-vs-surf.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{binder-reconstruction-quality/binder/surf-vs-col/outplots/surf-vs-col-table}
  \caption{%
   \textbf{Comparison of reconstruction accuracies from column- and surface-based annotations.}
   \footnotesize
    Color coding represents non-parametric difference between accuracy measures, with red indicating superior surface performance and blue indicating superior column performance.
    The left column shows tilted retention policies and the right column shows steady retention policies.
    For heatmap charts, +'s indicate small, medium, and large effect sizes of the Cliff's delta statistic and *'s indicate statistical significance at $\alpha = 0.05$ via a Mann-Whitney U test.
  }
  \label{fig:col-vs-surf}
  \vspace{-0.2in}
\end{figure*}


==> fig/genome-layout.tex <==
% Define lighter colors
\definecolor{LighterBlue}{rgb}{0.84, 0.92, 0.95}
\definecolor{LighterSalmon}{rgb}{1.0, 0.81, 0.76}
\definecolor{LighterPastelGreenYellow}{rgb}{0.88, 0.96, 0.90}

% Define thick vertical lines for section dividers
\newcolumntype{q}{!{\color{white} \vrule width 2pt}}

\begin{figure*}
    \centering
\begin{minipage}[t]{\textwidth}
\centering
\footnotesize
\begin{tabular}{
c
>{\columncolor{LighterBlue}}c
>{\columncolor{LighterBlue}}c
>{\columncolor{LighterSalmon}}c
>{\columncolor{LighterSalmon}}c
q % Thick divider
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
q % Thick divider
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
>{\columncolor{LighterPastelGreenYellow}}c
}
& \multicolumn{4}{cq}{\cellcolor{white}Word 0} & \multicolumn{4}{cq}{\cellcolor{white}Word 1} & \multicolumn{4}{c}{\cellcolor{white}Word 2} \\
\cmidrule(l{1.5pt}r{1.5pt}){2-5}
\cmidrule(l{1.5pt}r{1.5pt}){6-9}
\cmidrule(l{1.5pt}r{1.5pt}){10-13}
Byte & {\cellcolor{white}0} & {\cellcolor{white}1} & {\cellcolor{white}2} & {\cellcolor{white}3} & {\cellcolor{white}4} & {\cellcolor{white}5} & {\cellcolor{white}6} & {\cellcolor{white}7} & {\cellcolor{white}8} & {\cellcolor{white}9} & {\cellcolor{white}10} & {\cellcolor{white}11} \\
\cmidrule(l{1.5pt}r{1.5pt}){2-2}
\cmidrule(l{1.5pt}r{1.5pt}){3-3}
\cmidrule(l{1.5pt}r{1.5pt}){4-4}
\cmidrule(l{1.5pt}r{1.5pt}){5-5}
\cmidrule(l{1.5pt}r{1.5pt}){6-6}
\cmidrule(l{1.5pt}r{1.5pt}){7-7}
\cmidrule(l{1.5pt}r{1.5pt}){8-8}
\cmidrule(l{1.5pt}r{1.5pt}){9-9}
\cmidrule(l{1.5pt}r{1.5pt}){10-10}
\cmidrule(l{1.5pt}r{1.5pt}){11-11}
\cmidrule(l{1.5pt}r{1.5pt}){12-12}
\cmidrule(l{1.5pt}r{1.5pt}){13-13}
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 0} & \texttt{F9} & \texttt{02} & \texttt{79} & \texttt{00} & \texttt{8D} & \texttt{22} & \texttt{4F} & \texttt{F3} & \texttt{D2} & \texttt{78} & \texttt{AD} & \texttt{C7} \\
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 1} & \texttt{F9} & \texttt{02} & \texttt{75} & \texttt{00} & \texttt{8D} & \texttt{A1} & \texttt{CB} & \texttt{F2} & \texttt{D1} & \texttt{5B} & \texttt{CC} & \texttt{D4} \\
& \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{cq}{\cellcolor{white}} & \multicolumn{4}{c}{\cellcolor{white}} \\[-2ex]
\scriptsize{Genome 2} & \texttt{61} & \texttt{B6} & \texttt{65} & \texttt{00} & \texttt{66} & \texttt{29} & \texttt{B4} & \texttt{F0} & \texttt{62} & \texttt{99} & \texttt{5A} & \texttt{61} \\
{\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} &
{\cellcolor{white}\ldots} & {\cellcolor{white}\ldots} \\
\end{tabular}
\end{minipage}

\begin{minipage}[t]{\textwidth}
\caption{%
\textbf{Example genomes sampled after validation experiment completion.}
  In validation testing, genomes were composed of three 32-bit words.
  The first two bytes (blue) are fixed random markers generated at simulation start-up, indicating independent lineage originations.
  The next two bytes (salmon) are a generation counter.
  Bits within the final eight bytes are lineage checkpoint values to facilitate phylogenetic reconstruction, arranged according to a tilted hereditary stratigraphic algorithm.
  Note that this genome does not include any content affecting agent traits or fitness --- neutral selection was used for this validation experiment.
}
\label{fig:genome-layout}
\end{minipage}
\end{figure*}


==> fig/surf-algorithms.tex <==
\begin{figure*}
  \centering
\begin{subfigure}[b]{0.43\linewidth}
\centering
\textbf{steady retention policy}
\end{subfigure}
\begin{subfigure}[b]{0.43\linewidth}
\centering
\textbf{tilted retention policy}
\end{subfigure}

\vspace{-1.5ex}

  \begin{subfigure}[b]{0.5\linewidth}
    \centering
  \includegraphics[width=0.88\linewidth,trim={0 0 2.4cm 0},clip]{binder-surface-concept/teeplots/10/cnorm=log+num-generations=4096+surface-size=256+viz=site-deposition-depth-by-rank-heatmap+ynorm=linear+ext=}

    % \vspace{-1.5ex}

    % \caption{\footnotesize 256 bit steady surface site age plot}
    % \label{fig:steady-age-plot}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
  \includegraphics[width=0.88\linewidth, trim={2.4cm 0 0 0},clip]{binder-surface-concept/teeplots/21/cnorm=log+num-generations=4096+surface-size=256+viz=site-deposition-depth-by-rank-heatmap+ynorm=linear+ext=}

  % \vspace{-1.5ex}

  %   \caption{\footnotesize 256 bit tilted surface site age plot}
    % \label{fig:tilted-age-plot}
  \end{subfigure}

\vspace{-1ex}

\begin{subfigure}[b]{0.5\linewidth}
  \flushleft
\includegraphics[height=0.85in, trim={0 0 0 0},clip]{binder-surface-concept/teeplots/10/num-generations=262144+surface-size=64+viz=stratum-persistence-dripplot+ext=}

  % \centering
  % \vspace{-1.5ex}

  % \caption{\footnotesize 64 bit steady surface time retention plot}
  \label{fig:steady-retention-plot}
\end{subfigure}%
\begin{subfigure}[b]{0.5\linewidth}
  \centering
\includegraphics[height=0.85in, trim={1.65cm 0 0 0},clip]{binder-surface-concept/teeplots/21/num-generations=262144+surface-size=64+viz=stratum-persistence-dripplot+ext=}

  % \centering
  % \vspace{-1.5ex}

  % \caption{\footnotesize 64 bit tilted surface time retention plot}
  % \label{fig:tilted-retention-plot}
\end{subfigure}

\vspace{-2.5ex}

\caption{%
  \textbf{Surface-based hereditary stratigraphy implementations.}
  \footnotesize
  Visualizations of steady (left) and tilted (right) surface site selection policies.
  Top-row heatmaps show evolution of time-since-last-deposition for each site on a 256-bit field over the course of 4,096 time steps.
  The bottom row shows retention spans for 3,000 ingested time points.
  Vertical lines span durations between ingestion and elimination for differentia appended at successive time points.
  Time points previously eliminated are marked in red.
  Time elapses from bottom to top in both visualizations.
  }
\label{fig:surf-algorithms}
\vspace{-0.2in}

\end{figure*}


==> fig/surf-vs-column-schematic.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{img/surf-vs-column-schematic}

  \vspace{-1.5ex}

  \caption{
  \textbf{Column vs. surface-based hereditary stratigraphy.}
  \footnotesize
  Contrast of existing sorted-order ``column''-based stratum retention framework with proposed explicitly addressed ``surface''-based approach.}
  \label{fig:surf-vs-column-schematic}
  \vspace{-0.2in}
\end{figure}


==> fig/tagged.tex <==
\begin{figure}

\begin{subfigure}[c]{\linewidth} \centering
\begin{minipage}[c]{0.08\linewidth} \flushright
    \caption{\rotatebox[origin=c]{90}{25 cycles}}
    \label{fig:tagged_25}
  \end{minipage}%
  \begin{minipage}[c]{0.92\linewidth}
    \includegraphics[width=\textwidth,height=0.6in,trim={0 0.81cm 0 0},clip]{binder-wse-sketches/binder/teeplots/genome=hsurftiltedsticky_tagged+replicate=e4ea2071-8228-42de-af8c-879cedff9ba7+viz=draw-biopython-tree+ext=}
  \end{minipage}%
\end{subfigure}

\vspace{-1ex}

\begin{subfigure}[c]{\linewidth} \centering
\begin{minipage}[c]{0.08\linewidth} \flushright
    \caption{\rotatebox[origin=c]{90}{50 cycles}}
    \label{fig:tagged_50}
  \end{minipage}%
  \begin{minipage}[c]{0.92\linewidth}
    \includegraphics[width=\textwidth,height=0.6in,trim={0 0.81cm 0 0},clip]{binder-wse-sketches/binder/teeplots/genome=hsurftiltedsticky_tagged+replicate=3d55af5f-7714-45da-9276-e860f46b4d94+viz=draw-biopython-tree+ext=}
  \end{minipage}%
\end{subfigure}

\vspace{-1ex}

\begin{subfigure}[c]{\linewidth} \centering
  \begin{minipage}[c]{0.08\linewidth} \flushright
    \caption{\rotatebox[origin=c]{90}{100 cycles}}
    \label{fig:tagged_100}
  \end{minipage}%
  \begin{minipage}[c]{0.92\linewidth}
    \includegraphics[width=\textwidth,height=0.6in,trim={0 0.81cm 0 0},clip]{binder-wse-sketches/binder/teeplots/genome=hsurftiltedsticky_tagged+replicate=932aa302-becb-47e8-9712-7f550b02364c+viz=draw-biopython-tree+ext=}
  \end{minipage}%
\end{subfigure}

\vspace{-1ex}

\begin{subfigure}[c]{\linewidth} \centering
  \begin{minipage}[c]{0.08\linewidth} \flushright
    \caption{\rotatebox[origin=c]{90}{250 cycles}}
    \label{fig:tagged_250}
  \end{minipage}%
  \begin{minipage}[c]{0.92\linewidth}
    \includegraphics[width=\textwidth,height=0.8in]{binder-wse-sketches/binder/teeplots/genome=hsurftiltedsticky_tagged+replicate=42dbcbb3-b803-41a4-9285-4a450bfad6ed+viz=draw-biopython-tree+ext=}
  \end{minipage}%
\end{subfigure}

\vspace{-1.5ex}

\caption{%
\textbf{Clade Reconstruction Trial.}
\footnotesize
Example phylogenies reconstructed from runs of increasing duration on a virtual grid of nine hardware-simulated PEs.
Founding genomes were tagged with random 16-byte identifier values, which were held constant throughout simulation (Supplementary Figure \ref{fig:genome-layout}).
Color-coding indicates each sampled taxon's founding ancestor according to this identifier value.
Simulation performed under drift conditions.
}
\label{fig:tagged}
\vspace{-0.2in}
\end{figure}


==> fig/wse-phylogenies.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{\textwidth}
    \centering
    Generations Ago (approx.)
  \end{minipage}
  \begin{minipage}{\textwidth}
    \hspace{0.02\linewidth}
    \rotatebox{30}{\makebox[0.1\linewidth][c]{200,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{50,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{10,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{2,000}}
    \hfill
    \rotatebox{30}{\makebox[0.1\linewidth][c]{30}}
    \rotatebox{90}{\makebox[0.04\linewidth][c]{0}}
  \end{minipage}
  \begin{subfigure}[t]{\linewidth}
    \centering
  \includegraphics[width=\linewidth,height=0.3\linewidth]{bindertex-evolutionary-inference/img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=22/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=4+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=22+_generation=262144+_index=22+scale=log+ext=}
    \caption{%
    Tournament size 2.
    STAND-IN IMAGE.
    }
    \label{fig:wse-phylogenies-tsize2}
  \end{subfigure}

  \begin{subfigure}[t]{\linewidth}
    \centering
\includegraphics[width=\linewidth,height=0.3\linewidth]{bindertex-evolutionary-inference/img/perfect-tree-phylogenies-log/epoch=7+resolution=3+treatment=6/a=collapsed-phylogeny+epoch=00007+mut_distn=np.random.standard_normal+num_generations=32768+num_islands=1024+num_niches=1+p_island_migration=0.01+p_niche_invasion=3.0517578125e-08+population_size=3276.../8+replicate=0+tournament_size=2+treatment=6+_generation=262144+_index=6+scale=log+ext=}
    \caption{%
      Tournament size 8.
      STAND-IN IMAGE.
    }
    \label{fig:wse-phylogenies-tsize8}
  \end{subfigure}

\caption{%
\textbf{Phylogenies from on-hardware experiment.}
\footnotesize
Subfigures \ref{fig:wse-phylogenies-tsize2} and \ref{fig:wse-phylogenies-tsize8} contrast phylogenies from experiments with lower and higher selection pressure, respectively.
Note the recognizable decrease in phylogenetic richness under high selection pressure.
Each phylogeny subsampled to 131,072 taxa.
}
\label{fig:wse-phylogenies}

\end{figure*}


==> lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
asdf
}


==> lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> text/body/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

Computing hardware with transformative capabilities is coming to market right now.
This fact presents an immediate opportunity to bring orders-of-magnitude greater simulation scale to bear on grand challenges in artificial life.
It is not unreasonable to anticipate possibility that with such resources some aspects of these open questions will be revealed to harbor more-is-different dispositions, in which larger scales demonstrate qualitativey different dynamics \citep{anderson1972more}.
Riding the coattails of AI-workload-driven hardware development, itself largely driven by profound more-is-different payoffs in deep learning, provides perhaps the most immediate means toward this possibility.

Such an endeavor is a community-level challenge that will require extensive collaborative effort and pursuit of outside resources.
Work presented here is an early step in methods and wide-ranging infrastructure development necessary to scale up what's possible in digital evolution research.
We have demonstrated new algorithms and software for phylogeny-enabled agent-based evolution on a next-generation HPC accelerator hardware platform.
Microbenchmarking results show that proposed instrumentation algorithms achieve several-fold improvement in computational efficiency.
Related work shows new algorithms to improve reconstruction quality in some cases, too \citep{moreno2024guide}.
Benchmarks confirm that, including tracking operations, simple models at wafer scale can achieve quintillions of replications per day.

Special characteristics set agent-based digital evolution apart from many other HPC application domains and position it as a potentially valuable testbed for innovation and leadership.
Among these factors are challenging workload heterogeneity (varying within a population and over evolutionary time), resiliency of global state to local perturbations, and perhaps unparalleled freedom to recompose underlying simulation semantics to accommodate hardware capabilities.
Indeed, artificial life and digital evolution have played host to notable boundary-pushing approaches to computing at the frontiers of computing modalities such as best-effort computing, reservoir computing, globe-spanning time-available computing, and modular tile-based computing in addition to more traditional cluster and GPU-oriented approaches \citep{moreno2021conduit,ackley2020best,ackley2023robust,heinemann2008artificial,miikkulainen2024evolving}.
Work done to scale up digital evolution simulation should be done with an eye for contributions back to broader HPC constituencies.

In this vein, presented ``surface'' indexing algorithms stand to benefit larger classes of stream curation problems, situations in which a rolling feed of sequenced observations must be dynamically downsampled to ensure retention of elements representative across observed history \citep{moreno2024algorithms}.
In particular, to further benefit observable agent-based modeling, we are interested in exploring applications that sample time-series activity at simulation sites or distill coarsened agent histories (e.g., position over time).

The immediate goal of our presented work, however, is to build means for progress toward existing research agendas held across the realms of digital evolution and artificial life.
To this end, our work has prioritized production of reusable CSL and Python software tools ready to be harnessed by the broader research community.
In particular, CSL code implementing the presented island-model GA is defined in a modularized and extensible manner to support drop-in customization to instantiate any fixed-length genome content and fitness criteria corresponding to research interests within the community.
We look forward to collaboration in broader tandem efforts to harness the Cerebras platform, and other emerging hardware, in follow-on work.

